Z(3) Interfaces in Lattice Gauge Theory

A study is made of properties of the Z(3) interface which forms between the different ordered phases of pure SU(3) gauge theory above a critical temperature. The theory is simulated on a (2+1)-D lattice at various temperatures above this critical point. At high temperatures, the interface tension is shown to agree well with the prediction of perturbation theory. Near the critical temperature, the interface behaviour is characterised by various displacement moments, and modelled by an interacting scalar field theory. This thesis is provided for reference, as it gives full details of the computational and statistical methods outlined only briefly in preprints hep-lat/9605040 and hep-lat/9607005.

==> app_a.tex <==
\appendix{A}{Table of Values for $F(2r,3)$}

\bigskip\centerline{\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan3\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr \tableedge\tablerule\tablelines
&&#3&&#4&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height0pt&\omit&height0pt&\omit&height0pt\cr}
\def\tableedge{\omit&height2pt&\multispan3&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan3\cr}
\halign to10cm{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & 
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\ITo}{Values of $F(2r,3)$ for $r\leq 30$}
{$r$}{$F(2r,3)$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&1&&2.9257441147538591e-02&\cr
\tablelines\tablerule\tablelines
&&2&&2.8588133947184931e-03&\cr
\tablelines\tablerule\tablelines
&&3&&7.7625872330950078e-04&\cr
\tablelines\tablerule\tablelines
&&4&&3.1782999811761687e-04&\cr
\tablelines\tablerule\tablelines
&&5&&1.5992165454570213e-04&\cr
\tablelines\tablerule\tablelines
&&6&&9.1150725927608572e-05&\cr
\tablelines\tablerule\tablelines
&&7&&5.6469174319874464e-05&\cr
\tablelines\tablerule\tablelines
&&8&&3.7115784724567322e-05&\cr
\tablelines\tablerule\tablelines
&&9&&2.5484489828066094e-05&\cr
\tablelines\tablerule\tablelines
&&10&&1.8087564731975696e-05&\cr
\tablelines\tablerule\tablelines
&&11&&1.3170447587156097e-05&\cr
\tablelines\tablerule\tablelines
&&12&&9.7840479099121027e-06&\cr
\tablelines\tablerule\tablelines
&&13&&7.3840421441212328e-06&\cr
\tablelines\tablerule\tablelines
&&14&&5.6428031018154392e-06&\cr
\tablelines\tablerule\tablelines
&&15&&4.3549604790025167e-06&\cr
\tablelines\tablerule\tablelines
&&16&&3.3872387617351618e-06&\cr
\tablelines\tablerule\tablelines
&&17&&2.6505179822474595e-06&\cr
\tablelines\tablerule\tablelines
&&18&&2.0836256901432198e-06&\cr
\tablelines\tablerule\tablelines
&&19&&1.6435963519300661e-06&\cr
\tablelines\tablerule\tablelines
&&20&&1.2996333087139130e-06&\cr
\tablelines\tablerule\tablelines
&&21&&1.0292617591260539e-06&\cr
\tablelines\tablerule\tablelines
&&22&&8.1581683728676361e-07&\cr
\tablelines\tablerule\tablelines
&&23&&6.4676674563294586e-07&\cr
\tablelines\tablerule\tablelines
&&24&&5.1257056950486260e-07&\cr
\tablelines\tablerule\tablelines
&&25&&4.0588577520678718e-07&\cr
\tablelines\tablerule\tablelines
&&26&&3.2100885546335727e-07&\cr
\tablelines\tablerule\tablelines
&&27&&2.5347419875900234e-07&\cr
\tablelines\tablerule\tablelines
&&28&&1.9976210969186481e-07&\cr
\tablelines\tablerule\tablelines
&&29&&1.5708328861159867e-07&\cr
\tablelines\tablerule\tablelines
&&30&&1.2321764912912764e-07&\cr
\tablelines\tablerule}}\global\advance\tableno by1}}\bigskip
%Numbers generated by command: grep '^f\[' bessels.c | sed
%"s/f\[/\&\&/g" | sed "s/\]=/\&\&/g" | sed "s/;/\&\\cr/g"

\vfill\supereject\blankpagetrue\vbox to \vsize{}

==> app_b.tex <==
\appendix{B}{Fluctuation Moment Results}

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTi\xdef\BTi{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^2>$ from Raw Binned Data, Lower (25\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$5.63^{+0.08}_{-0.05}$&&$7.50^{+0.04}_{-0.01}$&&$10.9^{+0.1}_{-0.1}$&&$13.5^{+0.1}_{-0.1}$&&$16.6^{+0.1}_{-0.1}$&&$19.7^{+0.1}_{-0.2}$&&$21.7^{+0.2}_{-0.1}$&&${}_{ 1.30\pm 0.02}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$4.61^{+0.11}_{-0.01}$&&$6.32^{+0.05}_{-0.04}$&&$8.67^{+0.08}_{-0.04}$&&$10.6^{+0.1}_{-0.1}$&&$12.4^{+0.1}_{-0.1}$&&$15.5^{+0.1}_{-0.1}$&&$17.2^{+0.1}_{-0.1}$&&${}_{ 1.22\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$3.82^{+0.02}_{-0.03}$&&$5.00^{+0.03}_{-0.03}$&&$6.85^{+0.05}_{-0.05}$&&$8.63^{+0.08}_{-0.05}$&&$9.57^{+0.08}_{-0.06}$&&$11.5^{+0.1}_{-0.0}$&&$13.1^{+0.1}_{-0.1}$&&${}_{ 1.13\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$3.04^{+0.02}_{-0.02}$&&$4.11^{+0.03}_{-0.03}$&&$5.21^{+0.04}_{-0.03}$&&$6.21^{+0.04}_{-0.03}$&&$7.46^{+0.05}_{-0.04}$&&$8.63^{+0.07}_{-0.04}$&&$9.34^{+0.07}_{-0.06}$&&${}_{ 1.04\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$2.61^{+0.01}_{-0.02}$&&$3.43^{+0.02}_{-0.02}$&&$4.34^{+0.03}_{-0.02}$&&$5.21^{+0.03}_{-0.03}$&&$6.19^{+0.05}_{-0.04}$&&$7.27^{+0.05}_{-0.05}$&&$7.77^{+0.04}_{-0.05}$&&${}_{ 1.02\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.33\pm 0.02}$&&${}_{-0.32\pm 0.02}$&&${}_{-0.39\pm 0.02}$&&${}_{-0.40\pm 0.03}$&&${}_{-0.41\pm 0.01}$&&${}_{-0.42\pm 0.02}$&&${}_{-0.44\pm 0.03}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTii\xdef\BTii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^2>$ from Raw Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$6.87^{+0.22}_{-0.14}$&&$8.27^{+0.12}_{-0.03}$&&$12.3^{+0.2}_{-0.2}$&&$14.4^{+0.1}_{-0.1}$&&$17.8^{+0.1}_{-0.1}$&&$20.8^{+0.1}_{-0.2}$&&$23.1^{+0.2}_{-0.1}$&&${}_{ 1.20\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$5.02^{+0.20}_{-0.01}$&&$6.71^{+0.05}_{-0.05}$&&$9.14^{+0.09}_{-0.05}$&&$11.4^{+0.1}_{-0.1}$&&$13.4^{+0.1}_{-0.1}$&&$16.5^{+0.1}_{-0.1}$&&$18.2^{+0.1}_{-0.1}$&&${}_{ 1.21\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$3.93^{+0.03}_{-0.03}$&&$5.19^{+0.03}_{-0.04}$&&$7.17^{+0.05}_{-0.05}$&&$8.89^{+0.07}_{-0.05}$&&$10.0^{+0.1}_{-0.1}$&&$11.9^{+0.1}_{-0.1}$&&$13.8^{+0.1}_{-0.1}$&&${}_{ 1.15\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$3.07^{+0.02}_{-0.02}$&&$4.21^{+0.03}_{-0.03}$&&$5.32^{+0.04}_{-0.03}$&&$6.34^{+0.05}_{-0.04}$&&$7.63^{+0.06}_{-0.05}$&&$8.85^{+0.07}_{-0.05}$&&$9.57^{+0.06}_{-0.06}$&&${}_{ 1.05\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$2.62^{+0.01}_{-0.02}$&&$3.44^{+0.02}_{-0.02}$&&$4.38^{+0.03}_{-0.02}$&&$5.27^{+0.03}_{-0.03}$&&$6.29^{+0.05}_{-0.03}$&&$7.37^{+0.05}_{-0.05}$&&$7.89^{+0.04}_{-0.06}$&&${}_{ 1.03\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.41\pm 0.01}$&&${}_{-0.37\pm 0.02}$&&${}_{-0.44\pm 0.02}$&&${}_{-0.43\pm 0.03}$&&${}_{-0.44\pm 0.02}$&&${}_{-0.45\pm 0.03}$&&${}_{-0.46\pm 0.04}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTiii\xdef\BTiii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^2>$ from Raw Binned Data, Higher (75\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$9.21^{+0.50}_{-0.30}$&&$9.63^{+0.48}_{-0.08}$&&$13.4^{+0.4}_{-0.3}$&&$14.6^{+0.1}_{-0.1}$&&$17.6^{+0.1}_{-0.1}$&&$20.1^{+0.1}_{-0.1}$&&$22.0^{+0.2}_{-0.1}$&&${}_{ 0.91\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$6.19^{+0.36}_{-0.04}$&&$7.31^{+0.04}_{-0.05}$&&$9.71^{+0.06}_{-0.04}$&&$11.9^{+0.1}_{-0.1}$&&$13.9^{+0.1}_{-0.1}$&&$16.5^{+0.1}_{-0.1}$&&$18.0^{+0.1}_{-0.1}$&&${}_{ 1.08\pm 0.02}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$4.44^{+0.02}_{-0.02}$&&$5.96^{+0.03}_{-0.04}$&&$7.86^{+0.04}_{-0.05}$&&$9.48^{+0.06}_{-0.05}$&&$10.6^{+0.1}_{-0.1}$&&$12.3^{+0.1}_{-0.1}$&&$14.1^{+0.1}_{-0.1}$&&${}_{ 1.04\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$3.65^{+0.02}_{-0.02}$&&$4.88^{+0.03}_{-0.03}$&&$5.96^{+0.04}_{-0.02}$&&$6.94^{+0.04}_{-0.03}$&&$8.17^{+0.05}_{-0.05}$&&$9.29^{+0.06}_{-0.04}$&&$9.98^{+0.06}_{-0.05}$&&${}_{ 0.92\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$3.17^{+0.01}_{-0.02}$&&$4.04^{+0.02}_{-0.02}$&&$4.94^{+0.03}_{-0.02}$&&$5.79^{+0.03}_{-0.03}$&&$6.77^{+0.04}_{-0.03}$&&$7.75^{+0.05}_{-0.05}$&&$8.30^{+0.04}_{-0.05}$&&${}_{ 0.89\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.41\pm 0.03}$&&${}_{-0.37\pm 0.02}$&&${}_{-0.42\pm 0.02}$&&${}_{-0.39\pm 0.03}$&&${}_{-0.40\pm 0.02}$&&${}_{-0.41\pm 0.03}$&&${}_{-0.42\pm 0.04}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTiv\xdef\BTiv{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^4>_{Ws}$ from Raw Binned Data, Lower (25\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$1150^{+240}_{-10}$&&$251^{+81}_{+12}$&&$441^{+54}_{-33}$&&$331^{+15}_{-7}$&&$414^{+23}_{-16}$&&$568^{+14}_{-14}$&&$642^{+26}_{-10}$&&${}_{ 0.27\pm 0.25}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$438^{+891}_{-11}$&&$55.5^{+1.9}_{-1.4}$&&$102^{+5}_{-2}$&&$144^{+5}_{-4}$&&$166^{+5}_{-5}$&&$313^{+17}_{-12}$&&$286^{+9}_{-7}$&&${}_{ 1.84\pm 0.47}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$18.3^{+0.6}_{-0.5}$&&$26.7^{+0.8}_{-0.8}$&&$54.6^{+2.0}_{-1.6}$&&$79.5^{+6.3}_{-1.6}$&&$85.0^{+3.0}_{-2.3}$&&$121^{+1}_{+0.}$&&$160^{+8}_{-4}$&&${}_{ 1.99\pm 0.05}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$9.48^{+0.29}_{-0.26}$&&$16.1^{+0.6}_{-0.4}$&&$22.0^{+0.8}_{-0.4}$&&$30.3^{+1.2}_{-0.6}$&&$41.2^{+1.6}_{-1.1}$&&$49.2^{+2.3}_{-1.2}$&&$49.2^{+1.9}_{-1.5}$&&${}_{ 1.58\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$6.29^{+0.17}_{-0.18}$&&$8.88^{+0.25}_{-0.19}$&&$13.4^{+0.5}_{-0.2}$&&$17.2^{+0.6}_{-0.5}$&&$23.8^{+0.9}_{-0.6}$&&$29.2^{+1.4}_{-1.0}$&&$28.7^{+1.3}_{-0.9}$&&${}_{ 1.51\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-2.00\pm 0.43}$&&${}_{-1.25\pm 0.10}$&&${}_{-1.40\pm 0.06}$&&${}_{-1.23\pm 0.08}$&&${}_{-1.19\pm 0.04}$&&${}_{-1.24\pm 0.10}$&&${}_{-1.29\pm 0.11}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\vskip 0.5in

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTv\xdef\BTv{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^4>_{Ws}$ from Raw Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$2270^{+480}_{-180}$&&$334^{+125}_{-1.}$&&$967^{+343}_{-86}$&&$463^{+141}_{-21}$&&$492^{+58}_{-24}$&&$585^{+16}_{-13}$&&$690^{+31}_{-10}$&&${}_{-0.54\pm 0.27}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$775^{+349}_{-12}$&&$63.1^{+2.4}_{-1.9}$&&$111^{+5}_{-2}$&&$166^{+6}_{-5}$&&$199^{+6}_{-6}$&&$344^{+24}_{-14}$&&$299^{+11}_{-8}$&&${}_{ 1.31\pm 0.49}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$19.5^{+0.7}_{-0.6}$&&$28.3^{+0.9}_{-0.8}$&&$59.7^{+2.1}_{-1.7}$&&$82.5^{+3.3}_{-1.6}$&&$88.0^{+3.2}_{-2.6}$&&$126^{+8}_{-1}$&&$163^{+7}_{-4}$&&${}_{ 1.95\pm 0.05}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$9.92^{+0.30}_{-0.27}$&&$16.7^{+0.7}_{-0.5}$&&$22.3^{+0.8}_{-0.6}$&&$30.3^{+1.2}_{-0.7}$&&$43.2^{+1.9}_{-1.5}$&&$48.6^{+2.4}_{-1.3}$&&$49.5^{+2.1}_{-1.5}$&&${}_{ 1.54\pm 0.04}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$5.85^{+0.14}_{-0.17}$&&$8.80^{+0.27}_{-0.23}$&&$13.1^{+0.5}_{-0.3}$&&$15.6^{+0.6}_{-0.4}$&&$23.3^{+0.9}_{-0.6}$&&$28.6^{+1.2}_{-0.9}$&&$28.6^{+1.4}_{-1.0}$&&${}_{ 1.54\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-2.40\pm 0.44}$&&${}_{-1.33\pm 0.12}$&&${}_{-1.53\pm 0.17}$&&${}_{-1.47\pm 0.08}$&&${}_{-1.29\pm 0.05}$&&${}_{-1.26\pm 0.12}$&&${}_{-1.32\pm 0.11}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\vskip 0.5in

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTvi\xdef\BTvi{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^4>_{Ws}$ from Raw Binned Data, Higher (75\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$3820^{+540}_{-300}$&&$838^{+246}_{-22}$&&$1370^{+200}_{-100}$&&$483^{+29}_{-11}$&&$516^{+25}_{-16}$&&$705^{+19}_{-17}$&&$908^{+55}_{-20}$&&${}_{-1.01\pm 0.24}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$1750^{+340}_{-30}$&&$89.2^{+2.1}_{-1.9}$&&$139^{+3}_{-2}$&&$210^{+6}_{-5}$&&$268^{+6}_{-7}$&&$375^{+13}_{-1}$&&$371^{+11}_{-7}$&&${}_{ 0.88\pm 0.54}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$30.8^{+0.6}_{-0.5}$&&$53.4^{+2.7}_{-1.6}$&&$80.7^{+1.6}_{-1.6}$&&$114^{+2}_{-2}$&&$117^{+4}_{-3}$&&$153^{+6}_{-1}$&&$191^{+6}_{-4}$&&${}_{ 1.62\pm 0.04}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$18.5^{+0.4}_{-0.4}$&&$30.1^{+0.7}_{-0.5}$&&$38.7^{+0.8}_{-0.7}$&&$48.9^{+1.0}_{-0.7}$&&$64.4^{+2.0}_{-1.5}$&&$71.8^{+1.8}_{-1.1}$&&$76.8^{+2.2}_{-1.7}$&&${}_{ 1.32\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$12.3^{+0.2}_{-0.3}$&&$18.0^{+0.3}_{-0.3}$&&$23.8^{+0.7}_{-0.3}$&&$27.8^{+0.6}_{-0.6}$&&$39.0^{+1.0}_{-0.6}$&&$45.2^{+1.2}_{-0.9}$&&$47.1^{+1.3}_{-1.1}$&&${}_{ 1.28\pm 0.02}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-2.33\pm 0.52}$&&${}_{-1.20\pm 0.25}$&&${}_{-1.33\pm 0.24}$&&${}_{-1.21\pm 0.07}$&&${}_{-1.11\pm 0.05}$&&${}_{-1.18\pm 0.07}$&&${}_{-1.26\pm 0.06}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTvii\xdef\BTvii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^6>_{Ws}$ from Raw Binned Data, Lower (25\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$3450000$&&$540000$&&$654000$&&$84100$&&$49200$&&$34500$&&$43000$&&${}_{-4.38\pm 0.24}$&\cr
&& &&${}^{+730000}_{-310000}$&&${}^{+699000}_{+105000}$&&${}^{+166000}_{-91000}$&&${}^{+94600}_{-3900}$&&${}^{+5100}_{-2900}$&&${}^{+7200}_{-3500}$&&${}^{+7900}_{-2900}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$1370000$&&$1580$&&$3400$&&$3760$&&$3210$&&$19200$&&$1700$&&${}_{ 0.04\pm 1.18}$&\cr
&& &&${}^{+7100000}_{-20000}$&&${}^{+420}_{-160}$&&${}^{+1050}_{-300}$&&${}^{+600}_{-470}$&&${}^{+660}_{-640}$&&${}^{+6700}_{-900}$&&${}^{+1580}_{-880}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$278^{+52}_{-29}$&&$335^{+48}_{-39}$&&$1090^{+230}_{-140}$&&$2550^{+4340}_{-330}$&&$971^{+407}_{-204}$&&$1310^{+1590}_{+470}$&&$715^{+539}_{-377}$&&${}_{ 1.60\pm 0.29}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$75.2^{+11.1}_{-7.7}$&&$135^{+48}_{-18}$&&$70.9^{+30.3}_{-13.6}$&&$101^{+151}_{-47}$&&$191^{+98}_{-56}$&&$-37.5^{+156.6}_{-60.7}$&&$-637^{+111}_{-95}$&&${}_{ 0.73\pm 0.17}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$39.6^{+5.4}_{-4.5}$&&$34.2^{+6.8}_{-5.9}$&&$33.4^{+12.6}_{-9.1}$&&$19.6^{+27.8}_{-18.1}$&&$-64.2^{+25.5}_{-23.8}$&&$-157^{+56}_{-41}$&&$-149^{+48}_{-39}$&&${}_{-0.52\pm 0.11}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-4.99\pm 1.05}$&&${}_{-3.49\pm 0.57}$&&${}_{-4.08\pm 0.37}$&&${}_{-3.11\pm 0.38}$&&${}_{-2.75\pm 0.12}$&&${}_{-1.98\pm 0.47}$&&${}_{-3.00\pm 0.32}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTviii\xdef\BTviii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^6>_{Ws}$ from Raw Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$5720000$&&$391000$&&$1280000$&&$297000$&&$199000$&&$24900$&&$71700$&&${}_{-4.40\pm 0.39}$&\cr
&& &&${}^{+1370000}_{-510000}$&&${}^{+441000}_{+45000}$&&${}^{+720000}_{-180000}$&&${}^{+320000}_{-16000}$&&${}^{+295000}_{-23000}$&&${}^{+13600}_{-3800}$&&${}^{+112000}_{-7300}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$1880000$&&$1830$&&$3710$&&$5150$&&$6180$&&$42800$&&$2640$&&${}_{-2.87\pm 1.05}$&\cr
&& &&${}^{+970000}_{-20000}$&&${}^{+260}_{-170}$&&${}^{+640}_{-330}$&&${}^{+700}_{-560}$&&${}^{+1300}_{-980}$&&${}^{+41100}_{-2700}$&&${}^{+2570}_{-1400}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$289^{+44}_{-29}$&&$380^{+47}_{-47}$&&$1260^{+210}_{-140}$&&$2160^{+510}_{-160}$&&$939^{+312}_{-210}$&&$1660^{+880}_{+50}$&&$968^{+686}_{-399}$&&${}_{ 1.82\pm 0.26}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$109^{+15}_{-12}$&&$167^{+40}_{-24}$&&$110^{+29}_{-27}$&&$98.0^{+79.2}_{-43.7}$&&$285^{+127}_{-81}$&&$77.5^{+161.1}_{-61.2}$&&$-625^{+111}_{-94}$&&${}_{ 0.44\pm 0.25}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$27.1^{+3.7}_{-3.2}$&&$48.2^{+7.9}_{-7.9}$&&$39.4^{+15.0}_{-11.8}$&&$-19.7^{+26.3}_{-18.2}$&&$-65.2^{+34.7}_{-27.2}$&&$-213^{+44}_{-36}$&&$-125^{+67}_{-45}$&&${}_{ 1.06\pm 0.14}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-5.57\pm 0.98}$&&${}_{-3.16\pm 0.55}$&&${}_{-3.95\pm 0.47}$&&${}_{-3.33\pm 0.37}$&&${}_{-3.15\pm 0.23}$&&${}_{-2.27\pm 0.82}$&&${}_{-2.98\pm 0.29}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTix\xdef\BTix{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^6>_{Ws}$ from Raw Binned Data, Higher (75\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$7170000$&&$653000$&&$1580000$&&$257000$&&$59300$&&$73900$&&$157000$&&${}_{-4.40\pm 0.39}$&\cr
&& &&${}^{+1170000}_{-620000}$&&${}^{+821000}_{-43000}$&&${}^{+690000}_{-180000}$&&${}^{+323000}_{-12000}$&&${}^{+5600}_{-2800}$&&${}^{+9500}_{-6300}$&&${}^{+46000}_{-9000}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$3880000$&&$3750$&&$5410$&&$9560$&&$13700$&&$31000$&&$16000$&&${}_{-3.69\pm 0.99}$&\cr
&& &&${}^{+500000}_{-40000}$&&${}^{+390}_{-260}$&&${}^{+390}_{-270}$&&${}^{+1130}_{-800}$&&${}^{+1700}_{-1500}$&&${}^{+3400}_{-100}$&&${}^{+7100}_{-2300}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$749^{+55}_{-38}$&&$3930^{+26650}_{-1300}$&&$2180^{+200}_{-140}$&&$3900^{+230}_{-180}$&&$2650^{+390}_{-280}$&&$3650^{+960}_{-30}$&&$2190^{+950}_{-450}$&&${}_{ 1.54\pm 0.27}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$334^{+25}_{-22}$&&$660^{+55}_{-42}$&&$792^{+54}_{-58}$&&$935^{+65}_{-61}$&&$1070^{+170}_{-100}$&&$1020^{+110}_{-80}$&&$338^{+153}_{-134}$&&${}_{ 0.94\pm 0.26}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$173^{+13}_{-12}$&&$315^{+37}_{-27}$&&$378^{+43}_{-29}$&&$341^{+44}_{-32}$&&$536^{+77}_{-64}$&&$274^{+63}_{-46}$&&$207^{+68}_{-54}$&&${}_{ 0.60\pm 0.19}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-5.36\pm 1.01}$&&${}_{-2.22\pm 0.67}$&&${}_{-2.58\pm 0.70}$&&${}_{-2.39\pm 0.24}$&&${}_{-1.99\pm 0.07}$&&${}_{-2.36\pm 0.23}$&&${}_{-2.85\pm 0.11}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTx\xdef\BTx{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^2>$ from Smooth Binned Data, Lower (25\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$8.14^{+0.23}_{-0.13}$&&$10.1^{+0.2}_{-0.1}$&&$14.9^{+0.3}_{-0.2}$&&$17.8^{+0.2}_{-0.2}$&&$21.5^{+0.2}_{-0.2}$&&$25.6^{+0.2}_{-0.2}$&&$28.6^{+0.4}_{-0.3}$&&${}_{ 1.21\pm 0.02}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$6.02^{+0.14}_{-0.03}$&&$7.71^{+0.06}_{-0.06}$&&$10.6^{+0.1}_{-0.1}$&&$13.0^{+0.1}_{-0.1}$&&$15.0^{+0.1}_{-0.1}$&&$18.8^{+0.2}_{-0.1}$&&$20.6^{+0.1}_{-0.1}$&&${}_{ 1.16\pm 0.02}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$4.38^{+0.03}_{-0.04}$&&$5.75^{+0.04}_{-0.05}$&&$8.00^{+0.06}_{-0.06}$&&$10.1^{+0.1}_{-0.1}$&&$11.0^{+0.1}_{-0.1}$&&$13.1^{+0.1}_{-0.1}$&&$15.1^{+0.1}_{-0.1}$&&${}_{ 1.14\pm 0.02}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$3.14^{+0.03}_{-0.03}$&&$4.40^{+0.04}_{-0.04}$&&$5.67^{+0.05}_{-0.04}$&&$6.82^{+0.05}_{-0.04}$&&$8.19^{+0.06}_{-0.05}$&&$9.51^{+0.08}_{-0.05}$&&$10.3^{+0.1}_{-0.1}$&&${}_{ 1.09\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$2.54^{+0.02}_{-0.02}$&&$3.46^{+0.02}_{-0.02}$&&$4.50^{+0.04}_{-0.03}$&&$5.46^{+0.04}_{-0.04}$&&$6.54^{+0.05}_{-0.04}$&&$7.71^{+0.06}_{-0.06}$&&$8.26^{+0.05}_{-0.06}$&&${}_{ 1.10\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.51\pm 0.03}$&&${}_{-0.46\pm 0.03}$&&${}_{-0.51\pm 0.03}$&&${}_{-0.50\pm 0.03}$&&${}_{-0.50\pm 0.02}$&&${}_{-0.51\pm 0.02}$&&${}_{-0.53\pm 0.03}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\vskip 0.5in

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTxi\xdef\BTxi{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^2>$ from Smooth Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$7.90^{+0.19}_{-0.12}$&&$10.6^{+0.2}_{-0.0}$&&$15.4^{+0.3}_{-0.2}$&&$18.3^{+0.2}_{-0.1}$&&$22.5^{+0.2}_{-0.2}$&&$26.6^{+0.2}_{-0.2}$&&$30.3^{+0.4}_{-0.3}$&&${}_{ 1.26\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$5.67^{+0.05}_{-0.02}$&&$8.00^{+0.07}_{-0.07}$&&$11.0^{+0.1}_{-0.1}$&&$13.6^{+0.1}_{-0.1}$&&$15.8^{+0.1}_{-0.1}$&&$19.6^{+0.2}_{-0.1}$&&$21.5^{+0.2}_{-0.1}$&&${}_{ 1.23\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$4.36^{+0.04}_{-0.04}$&&$5.79^{+0.04}_{-0.05}$&&$8.17^{+0.07}_{-0.07}$&&$10.1^{+0.1}_{-0.1}$&&$11.4^{+0.1}_{-0.1}$&&$13.5^{+0.1}_{-0.1}$&&$15.6^{+0.1}_{-0.1}$&&${}_{ 1.17\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$3.07^{+0.03}_{-0.03}$&&$4.40^{+0.03}_{-0.04}$&&$5.65^{+0.05}_{-0.04}$&&$6.80^{+0.05}_{-0.04}$&&$8.22^{+0.06}_{-0.06}$&&$9.59^{+0.08}_{-0.05}$&&$10.3^{+0.1}_{-0.1}$&&${}_{ 1.11\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$2.47^{+0.01}_{-0.02}$&&$3.37^{+0.02}_{-0.02}$&&$4.40^{+0.04}_{-0.03}$&&$5.40^{+0.04}_{-0.04}$&&$6.52^{+0.05}_{-0.04}$&&$7.69^{+0.06}_{-0.06}$&&$8.25^{+0.05}_{-0.06}$&&${}_{ 1.13\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.50\pm 0.03}$&&${}_{-0.48\pm 0.03}$&&${}_{-0.54\pm 0.03}$&&${}_{-0.52\pm 0.04}$&&${}_{-0.52\pm 0.02}$&&${}_{-0.53\pm 0.03}$&&${}_{-0.56\pm 0.03}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\vskip 0.5in

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTxii\xdef\BTxii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^2>$ from Smooth Binned Data, Higher (75\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$8.35^{+0.15}_{-0.09}$&&$11.9^{+0.2}_{-0.0}$&&$16.1^{+0.2}_{-0.2}$&&$19.8^{+0.2}_{-0.2}$&&$24.0^{+0.2}_{-0.2}$&&$28.3^{+0.2}_{-0.2}$&&$32.1^{+0.4}_{-0.2}$&&${}_{ 1.23\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$6.88^{+0.12}_{-0.03}$&&$9.29^{+0.07}_{-0.07}$&&$12.1^{+0.1}_{-0.1}$&&$15.0^{+0.1}_{-0.1}$&&$17.5^{+0.1}_{-0.1}$&&$21.0^{+0.2}_{-0.1}$&&$22.8^{+0.1}_{-0.1}$&&${}_{ 1.12\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$5.32^{+0.03}_{-0.03}$&&$7.12^{+0.04}_{-0.05}$&&$9.50^{+0.06}_{-0.06}$&&$11.4^{+0.1}_{-0.1}$&&$12.6^{+0.1}_{-0.1}$&&$14.5^{+0.1}_{-0.1}$&&$16.6^{+0.1}_{-0.1}$&&${}_{ 1.03\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$4.07^{+0.03}_{-0.03}$&&$5.54^{+0.04}_{-0.04}$&&$6.79^{+0.05}_{-0.03}$&&$7.92^{+0.05}_{-0.04}$&&$9.35^{+0.06}_{-0.05}$&&$10.6^{+0.1}_{-0.0}$&&$11.4^{+0.1}_{-0.1}$&&${}_{ 0.94\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$3.34^{+0.01}_{-0.03}$&&$4.33^{+0.03}_{-0.02}$&&$5.40^{+0.04}_{-0.03}$&&$6.37^{+0.03}_{-0.04}$&&$7.50^{+0.05}_{-0.04}$&&$8.63^{+0.05}_{-0.06}$&&$9.23^{+0.05}_{-0.06}$&&${}_{ 0.95\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.40\pm 0.03}$&&${}_{-0.42\pm 0.03}$&&${}_{-0.47\pm 0.03}$&&${}_{-0.48\pm 0.03}$&&${}_{-0.49\pm 0.02}$&&${}_{-0.51\pm 0.02}$&&${}_{-0.54\pm 0.03}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTxiii\xdef\BTxiii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^4>_{Ws}$ from Smooth Binned Data, Lower (25\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$1730^{+220}_{-120}$&&$628^{+10}_{-20}$&&$1340^{+170}_{-100}$&&$981^{+478}_{-65}$&&$936^{+135}_{-80}$&&$1050^{+80}_{-50}$&&$1130^{+360}_{-50}$&&${}_{-0.18\pm 0.15}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$729^{+57}_{-9}$&&$71.8^{+2.9}_{-2.2}$&&$132^{+9}_{-3}$&&$166^{+6}_{-5}$&&$182^{+6}_{-6}$&&$456^{+261}_{-46}$&&$291^{+11}_{-8}$&&${}_{-0.11\pm 0.38}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$24.1^{+0.9}_{-0.8}$&&$31.3^{+1.3}_{-1.2}$&&$62.1^{+2.7}_{-2.1}$&&$89.2^{+15.8}_{-3.4}$&&$82.5^{+3.7}_{-3.0}$&&$112^{+11}_{+1.}$&&$148^{+7}_{-4}$&&${}_{ 1.65\pm 0.07}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$10.4^{+0.5}_{-0.4}$&&$16.1^{+0.8}_{-0.5}$&&$20.6^{+1.0}_{-0.5}$&&$26.3^{+1.6}_{-0.8}$&&$34.9^{+1.8}_{-1.2}$&&$38.2^{+2.4}_{-1.3}$&&$33.7^{+2.2}_{-1.4}$&&${}_{ 1.21\pm 0.05}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$6.04^{+0.26}_{-0.22}$&&$7.91^{+0.32}_{-0.24}$&&$11.5^{+0.5}_{-0.3}$&&$13.5^{+0.7}_{-0.5}$&&$18.7^{+0.9}_{-0.6}$&&$20.5^{+1.4}_{-1.0}$&&$18.0^{+1.3}_{-1.1}$&&${}_{ 1.19\pm 0.05}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-2.69\pm 0.34}$&&${}_{-1.63\pm 0.15}$&&${}_{-1.84\pm 0.14}$&&${}_{-1.67\pm 0.10}$&&${}_{-1.54\pm 0.06}$&&${}_{-1.65\pm 0.12}$&&${}_{-1.76\pm 0.11}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\vskip 0.5in

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTxiv\xdef\BTxiv{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^4>_{Ws}$ from Smooth Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$2230^{+270}_{-160}$&&$861^{+163}_{-12}$&&$1620^{+330}_{-140}$&&$715^{+172}_{-33}$&&$816^{+132}_{-60}$&&$912^{+55}_{-32}$&&$1300^{+340}_{-60}$&&${}_{-0.56\pm 0.17}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$497^{+28}_{-9}$&&$79.8^{+4.0}_{-3.2}$&&$132^{+7}_{-3}$&&$187^{+7}_{-7}$&&$223^{+8}_{-9}$&&$422^{+87}_{-25}$&&$300^{+16}_{-10}$&&${}_{-0.02\pm 0.31}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$24.0^{+1.1}_{-0.8}$&&$31.1^{+1.3}_{-1.2}$&&$64.4^{+2.9}_{-2.5}$&&$87.7^{+5.4}_{-2.4}$&&$82.3^{+3.9}_{-3.2}$&&$118^{+10}_{-1.}$&&$148^{+7}_{-4}$&&${}_{ 1.68\pm 0.07}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$10.3^{+0.5}_{-0.4}$&&$16.1^{+0.9}_{-0.6}$&&$20.0^{+1.0}_{-0.7}$&&$25.3^{+1.3}_{-0.8}$&&$35.9^{+2.2}_{-1.6}$&&$36.5^{+2.7}_{-1.3}$&&$32.2^{+2.0}_{-1.6}$&&${}_{ 1.17\pm 0.06}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$5.04^{+0.20}_{-0.20}$&&$7.11^{+0.34}_{-0.25}$&&$10.1^{+0.6}_{-0.3}$&&$11.0^{+0.6}_{-0.5}$&&$16.8^{+0.9}_{-0.7}$&&$19.1^{+1.3}_{-1.0}$&&$17.3^{+1.5}_{-1.0}$&&${}_{ 1.27\pm 0.05}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-2.76\pm 0.25}$&&${}_{-1.80\pm 0.17}$&&${}_{-1.88\pm 0.17}$&&${}_{-1.74\pm 0.10}$&&${}_{-1.61\pm 0.04}$&&${}_{-1.62\pm 0.13}$&&${}_{-1.82\pm 0.11}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\vskip 0.5in

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTxv\xdef\BTxv{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^4>_{Ws}$ from Smooth Binned Data, Higher (75\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$2180^{+310}_{-170}$&&$909^{+92}_{-3}$&&$1280^{+230}_{-10}$&&$967^{+57}_{-29}$&&$989^{+76}_{-44}$&&$1300^{+60}_{-40}$&&$1620^{+10}_{-40}$&&${}_{ 0.08\pm 0.16}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$1060^{+90}_{-20}$&&$138^{+5}_{-4}$&&$192^{+5}_{-3}$&&$284^{+9}_{-8}$&&$366^{+11}_{-10}$&&$522^{+24}_{-19}$&&$444^{+15}_{-11}$&&${}_{ 0.24\pm 0.33}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$43.0^{+1.2}_{-0.9}$&&$68.8^{+2.7}_{-2.0}$&&$102^{+2}_{-2}$&&$143^{+3}_{-3}$&&$131^{+5}_{-3}$&&$169^{+8}_{-1}$&&$196^{+7}_{-4}$&&${}_{ 1.36\pm 0.05}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$24.3^{+0.5}_{-0.5}$&&$37.7^{+1.0}_{-0.8}$&&$45.9^{+1.1}_{-1.0}$&&$56.0^{+1.2}_{-0.9}$&&$71.5^{+2.7}_{-1.8}$&&$74.5^{+2.0}_{-1.2}$&&$74.0^{+2.1}_{-2.0}$&&${}_{ 1.06\pm 0.04}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$15.4^{+0.4}_{-0.4}$&&$21.6^{+0.5}_{-0.5}$&&$27.1^{+0.9}_{-0.5}$&&$30.0^{+0.8}_{-0.7}$&&$41.4^{+1.1}_{-0.8}$&&$43.6^{+1.3}_{-0.9}$&&$45.0^{+1.7}_{-1.2}$&&${}_{ 1.02\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-2.28\pm 0.34}$&&${}_{-1.44\pm 0.13}$&&${}_{-1.38\pm 0.15}$&&${}_{-1.43\pm 0.05}$&&${}_{-1.34\pm 0.04}$&&${}_{-1.45\pm 0.06}$&&${}_{-1.50\pm 0.02}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTxvi\xdef\BTxvi{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^6>_{Ws}$ from Smooth Binned Data, Lower (25\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$3450000$&&$540000$&&$654000$&&$84100$&&$49200$&&$34500$&&$43000$&&${}_{-1.62\pm 0.20}$&\cr
&& &&${}^{+330000}_{-180000}$&&${}^{+170000}_{-54000}$&&${}^{+260000}_{-150000}$&&${}^{+507000}_{-38000}$&&${}^{+67000}_{-39000}$&&${}^{+166000}_{-57000}$&&${}^{+359000}_{-30000}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$1370000$&&$1580$&&$3400$&&$3760$&&$3210$&&$19200$&&$1700$&&${}_{-5.38\pm 1.17}$&\cr
&& &&${}^{+51000}_{-6000}$&&${}^{+630}_{-270}$&&${}^{+9720}_{-1340}$&&${}^{+820}_{-640}$&&${}^{+1130}_{-1020}$&&${}^{+606000}_{-13000}$&&${}^{+2940}_{-1650}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$562^{+83}_{-49}$&&$804^{+110}_{-90}$&&$1840^{+290}_{-190}$&&$5580^{+13520}_{-860}$&&$1760^{+500}_{-290}$&&$2020^{+1510}_{+370}$&&$1010^{+530}_{-370}$&&${}_{ 1.19\pm 0.32}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$156^{+21}_{-15}$&&$247^{+64}_{-28}$&&$222^{+54}_{-14}$&&$303^{+159}_{-61}$&&$485^{+105}_{-53}$&&$338^{+169}_{-59}$&&$-67.7^{+116.7}_{-86.0}$&&${}_{ 1.02\pm 0.09}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$67.0^{+11.0}_{-7.4}$&&$97.5^{+15.4}_{-10.8}$&&$119^{+19}_{-13}$&&$164^{+46}_{-31}$&&$121^{+34}_{-34}$&&$137^{+69}_{-48}$&&$208^{+53}_{-47}$&&${}_{ 0.90\pm 0.08}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-5.40\pm 0.94}$&&${}_{-3.30\pm 0.47}$&&${}_{-3.96\pm 0.37}$&&${}_{-3.25\pm 0.48}$&&${}_{-3.45\pm 0.33}$&&${}_{-3.47\pm 0.51}$&&${}_{-3.55\pm 0.22}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTxvii\xdef\BTxvii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^6>_{Ws}$ from Smooth Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$5720000$&&$391000$&&$1280000$&&$297000$&&$199000$&&$24900$&&$71700$&&${}_{-2.55\pm 0.24}$&\cr
&& &&${}^{+660000}_{-370000}$&&${}^{+910000}_{-80000}$&&${}^{+850000}_{-290000}$&&${}^{+452000}_{-22000}$&&${}^{+406000}_{-51000}$&&${}^{+250000}_{-40000}$&&${}^{+610000}_{-39000}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$1880000$&&$1830$&&$3710$&&$5150$&&$6180$&&$42800$&&$2640$&&${}_{-5.29\pm 1.10}$&\cr
&& &&${}^{+28000}_{-8000}$&&${}^{+560}_{-360}$&&${}^{+940}_{-500}$&&${}^{+960}_{-790}$&&${}^{+2600}_{-1900}$&&${}^{+109400}_{-5700}$&&${}^{+5970}_{-2450}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$546^{+70}_{-49}$&&$775^{+103}_{-83}$&&$1760^{+310}_{-210}$&&$4000^{+1370}_{-280}$&&$1850^{+470}_{-290}$&&$3380^{+1300}_{+90}$&&$1830^{+670}_{-400}$&&${}_{ 1.66\pm 0.22}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$207^{+38}_{-24}$&&$286^{+51}_{-37}$&&$295^{+42}_{-36}$&&$313^{+88}_{-60}$&&$574^{+147}_{-98}$&&$484^{+147}_{-53}$&&$-157^{+106}_{-97}$&&${}_{ 0.92\pm 0.08}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$49.7^{+9.0}_{-6.5}$&&$76.4^{+11.9}_{-9.5}$&&$90.2^{+21.3}_{-13.3}$&&$73.8^{+29.8}_{-19.0}$&&$53.7^{+47.2}_{-31.3}$&&$19.3^{+40.2}_{-35.5}$&&$178^{+65}_{-50}$&&${}_{{\hbox{n/a}}}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-5.78\pm 0.92}$&&${}_{-3.35\pm 0.59}$&&${}_{-3.79\pm 0.52}$&&${}_{-3.24\pm 0.32}$&&${}_{-3.39\pm 0.25}$&&${}_{{\hbox{n/a}}}$&&${}_{-3.71\pm 0.17}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTxviii\xdef\BTxviii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^6>_{Ws}$ from Smooth Binned Data, Higher (75\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$7170000$&&$653000$&&$1580000$&&$257000$&&$59300$&&$73900$&&$157000$&&${}_{-2.60\pm 0.19}$&\cr
&& &&${}^{+750000}_{-420000}$&&${}^{+710000}_{-40000}$&&${}^{+670000}_{-240000}$&&${}^{+322000}_{-26000}$&&${}^{+21000}_{-13000}$&&${}^{+57000}_{-32000}$&&${}^{+65000}_{-20000}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$3880000$&&$3750$&&$5410$&&$9560$&&$13700$&&$31000$&&$16000$&&${}_{-4.14\pm 0.86}$&\cr
&& &&${}^{+110000}_{-30000}$&&${}^{+2700}_{-1500}$&&${}^{+800}_{-600}$&&${}^{+3400}_{-2200}$&&${}^{+4800}_{-3500}$&&${}^{+10500}_{-2800}$&&${}^{+5700}_{-3200}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$1460^{+130}_{-80}$&&$3610^{+1460}_{-450}$&&$5230^{+1300}_{-440}$&&$9660^{+800}_{-510}$&&$7010^{+770}_{-560}$&&$7880^{+1360}_{-60}$&&$5700^{+1070}_{-690}$&&${}_{ 1.56\pm 0.18}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$707^{+46}_{-43}$&&$1380^{+120}_{-90}$&&$1860^{+140}_{-130}$&&$2290^{+320}_{-160}$&&$2640^{+300}_{-180}$&&$3080^{+240}_{-170}$&&$2140^{+250}_{-200}$&&${}_{ 1.21\pm 0.10}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$411^{+50}_{-36}$&&$713^{+93}_{-61}$&&$812^{+68}_{-46}$&&$1070^{+80}_{-70}$&&$1390^{+160}_{-110}$&&$1060^{+110}_{-70}$&&$1420^{+120}_{-10}$&&${}_{ 1.03\pm 0.07}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-5.25\pm 0.99}$&&${}_{-2.74\pm 0.43}$&&${}_{-2.43\pm 0.57}$&&${}_{-2.44\pm 0.22}$&&${}_{-2.29\pm 0.10}$&&${}_{-2.46\pm 0.17}$&&${}_{-2.36\pm 0.19}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip


==> conclusion.tex <==
\newsec{Conclusions}{}

\Subsec{Conclusions}
In this thesis, we have examined the properties of the $Z(3)$
interface in two very different regimes:
\vskip 0.2in

At high temperatures, we have
measured the interface tension on the lattice, and extrapolated our
results to the infinite-temperature limit, where we have found good
agreement with the prediction of an instanton calculation. This
reinforces the argument for the existence of $Z(3)$-breaking phases in
the Euclidean functional integral, although their physical existence
in the early universe remains in question, and suggests that the
predictions of perturbation theory are indeed reliable in this
regime. We have also examined the
Debye profile of the interface, but have not been able to compare our
results accurately with predictions at the temperatures concerned.

Just above the critical temperature, we have seen that it is possible
to follow the fluctuations in profile of the interface even though it
appears, at first sight, to disappear in the phase turbulence. We have
observed that the interface maintains a narrow width right down to the
critical temperature, but undergoes more and more severe fluctuations
in shape. We have characterised these fluctuations using moments, and
have seen that these diverge at the critical temperature; and we have
constructed a toy scalar field theory model which reproduces the
observed behaviour to a reasonable approximation. We have also
seen that whilst the intrinsic width of the interface increases rather
slowly near the critical point, the Debye screening width appears to
diverge logarithmically, in line with the predictions for a completely
wet interface; but we have not seen direct evidence for this
wetting. Finally, we have noted that the formation and movement of the
interface on the lattice shares many of the characteristics of
interface behaviour in condensed matter systems.
\vfill\supereject\blankpagetrue\vbox to \vsize{}

==> cover.tex <==
\def\quote#1#2{\footline={\hfil}\headline={\hfil} \centerline{\vbox{\vskip 2in\normalbaselines\halign{\hfil{\it ##}\hfil\cr #1\cr{\hfill\rm #2}\cr}}}}

{\headline={\hfil}
\Title{\vbox{\centerline{Z(3) Interfaces in}\vskip 5pt
\centerline{Lattice Gauge Theory}}}

\centerline{{\authorfont Stephen T. West}}
\centerline{St. John's College}
\bigskip
\centerline{{\it Theoretical Physics}}
\centerline{{\it Department of Physics}}
\centerline{{\it Oxford University}}
\bigskip
\def\crest{{\font\cf=oxcrest40\cf\char"01}}
% XXX: \def\crest{{\font\cf=oxcrest40\cf\char"01}}
\def\crest{Oxford University}
\vbox to 0pt{\hbox to\hsize{\hss\crest\hss}\vss}

\Date{Hilary Term 1996}}

%For single-sided, replace these three lines with a single \eject
\supereject
\footline={\hfil}\vbox to\vsize{}
\supereject 

{\headline={\hfil}
\Title{\vbox{\centerline{Z(3) Interfaces in}\vskip 5pt
\centerline{Lattice Gauge Theory}}}

\centerline{{\authorfont Stephen T. West}}
\centerline{St. John's College}
\bigskip
\centerline{{\it Theoretical Physics}}
\centerline{{\it Department of Physics}}
\centerline{{\it Oxford University}}
\bigskip
% XXX: \def\crest{{\font\cf=oxcrest40\cf\char"01}}
\def\crest{Oxford University}
\vbox to 0pt{\hbox to\hsize{\hss\crest\hss}\vss}
\vskip 1in
\centerline{ABSTRACT}
\vskip 0.4in
\centerline{\vbox{\advance\hsize by -0.8truein{
We study various properties of the $Z(3)$ interface which forms
between the different ordered phases of pure $SU(3)$ gauge theory
above a critical temperature. We simulate the theory on a
computational lattice of two space and one time dimensions, at various
temperatures above this critical point. At high temperatures, we
perform an accurate measurement of the interface tension, which shows
good agreement with the prediction of perturbation theory. Near the
critical temperature, we show that it is possible to observe the
behaviour of the interface amidst the phase turbulence near 
its collapse, and we characterise its fluctuations in terms of various
displacement moments. We show that the interface behaves like a
fluctuating string, and model its behaviour in terms of an
interacting scalar field theory. We also examine other properties of
the interface, including its intrinsic and Debye electric screening
widths, its formation and movement on the lattice, and its wetting.}}}

\Date{Hilary Term 1996}}

%For single-sided, replace these three lines with a single \eject
\supereject
\footline={\hfil}\vbox to\vsize{}
\supereject 

\quote{Finally Cutangle spoke, very slowly and carefully.\cr\cr `I look
at it like this,' he said. `Before I heard him talk, I was\cr  like
everyone else. You know what I mean? I was confused\cr and uncertain
about all the little details of life. But now,' he\cr brightened up,
`while I'm still confused and uncertain it's\cr on a much higher plane,
d'you see, and at least I know I'm\cr bewildered about the really
fundamental and important facts\cr of the universe.'\cr\cr Treatle
nodded. `I hadn't looked at it like that,' he said,\cr `but you're
absolutely right. He's really pushed back the\cr boundaries of
ignorance. There's so much about the universe\cr we don't know.'\cr\cr They
both savoured the strange warm glow of being much\cr more ignorant than
ordinary people, who were ignorant of\cr only ordinary things.\cr}{Terry
Pratchett --- ``Equal Rites'' (1987)}
\supereject

%For single-sided, comment out this line
\vbox to\vsize{}\supereject 

\hbox{}
\vskip 0.5in
\Title{To my parents}
\vskip 3.5in

\Title{Acknowledgements}

I should like to thank my supervisor, John Wheater, for his guidance
and support during my time as a graduate student. I am also grateful
to Mike Teper for the chance to examine his SU(2) simulation code, and
to both him and Amanda Michels for profitable discussions; also, to
James Carpenter for introducing me to modern statistical methods.

I should also like express my thanks to the P.P.A.R.C. for supporting
my research, to the denizens of room 1.12 and many others in
Theoretical Physics for making it a pleasant experience, and to my
parents for keeping me sane.

A short summary of this work is about to appear in the paper
``Properties of the $Z(3)$ Interface in (2+1)-D $SU(3)$ Gauge
Theory'', by S.T.~West and J.F.~Wheater, to be published in the
``Proceedings of Lattice '95'', \NP{Proc. Suppl. B}{1996}{}.
\vfill\supereject

%For single-sided, comment out this line
\vbox to\vsize{}\supereject 

% Comment out these lines until toc.tex and tof.tex exist:
\listtoc
\listtof


==> hightemp.tex <==
\newsec{Monte-Carlo Techniques \&}{Results at High Temperatures}

\Subsec{Computer Simulation (2+1 dimensions)}
In order to test the predictions of the previous chapter for the
properties of the $Z(3)$ interface, it is possible to simulate pure
gauge $SU(3)$ theory on a computational lattice. In what follows, we
have simulated the theory in $2+1$ dimensions, {\it i.e.} two space
and one Euclidean time dimensions, as in \IFiii. One would prefer to
work in the real world of $3+1$ dimensions, of course, but it should
be remembered that the interface profile is a one-dimensional object,
interpolating between one $Z(3)$ vacuum at $z=0$ and another
at $z=L_z$. All other spatial dimensions are therefore transverse,
simply specifying the dimensions of the interface itself: in $2+1$
dimensions, the interface is one-dimensional (a string), and in
$3+1$ dimensions, it is two-dimensional (a sheet). An interface in a
$(2+1)$-dimensional system, as well as being worthy of study in its
own right, may tell us much about properties in the higher dimension.
The most obvious reason to work in $2+1$ dimensions, apart from the
benefit to be had from studying the simpler, one-dimensional interface, is
that by working in three
Euclidean dimensions rather than four, we are able to considerably
reduce the computational time needed for results of a desired
accuracy.

The $SU(3)$ system with $2+1$ dimensions provides an extremely useful
testing ground, and is interesting in its own right. However, it
differs from a similar system in $3+1$ dimensions in at least one
fundamental respect: the nature of the phase transition at the
critical temperature. In $2+1$ dimensions, the transition is second
order, meaning that the Polyakov line diverges smoothly from zero in the
disordered phase, at and below
the critical temperature, to its non-zero values in the different
$Z(3)$ phases above $T_c$. Thus, an interface present in this theory
above the critical temperature would be expected to shrink
continuously to nothing as $T\rightarrow T_c$. However, the phase
transition in the pure glue theory has been
confirmed\ref\IIRoo{R.~V.~Gavai, F.~Karsch and 
B.~Petersson, \NP{B322}{1989}{738}; M.~Fukugita, M.~Okawa and
U.~Ukawa, \PRL{63}{1989}{1768}; \NP{B337}{1990}{181}; N.A.~Alves,
B.A.~Berg and S.~Sanielevici, \PRL{64}{1990}{3107}}
to be {\it first} order in $3+1$ dimensions, so that there is a
discontinuity in the Polyakov line at the critical temperature, {\it
i.e.} a jump from zero to a non-zero value as the temperature
increases through $T_c$, followed by a further smooth change away from
zero as the $T\rightarrow\infty$. Hence, while many inferences may be drawn
from results in $2+1$ dimensions, it is not clear that properties such
as those describing the collapse of the interface at $T_c$ will apply
equally to $3+1$ dimensions. It should be borne in mind, though, that a
second-order phase transition in $3+1$ dimensions {\it is} seen in an
$SU(2)$ system, and so those properties which do not carry directly
over to an $SU(3)$ system in $3+1$ dimensions may, instead, be
relevant to an $SU(2)$ system.

In the computer simulation of pure gauge $SU(3)$ theory,
the fundamental variables are simply the link variables of
\IExviiia. The variable $U_n^\mu$ is attached to the link leaving site
$n$ in the $\mu$ direction, where $\mu=0,1,2$,
corresponding to our one time and two space dimensions, and now $U \in
SU(3)$. In an obvious extension of notation, $U_n^{\mu\dagger} =
U_{n+\hat\mu}^{-\mu}$. We can construct physical observables from
these link variables, as in \IExixa, and then use Monte-Carlo
procedures to compute a statistical average over all possible
configurations of the system.
Leaving the details of Monte-Carlo
techniques used for the next section, we first deal with the
creation of an interface on the lattice.

\ifig\IIFo{The Euclidean lattice in $2+1$ dimensions: there are $N_t$
links in the time dimension, $\tau$; the longitudinal space dimension,
$z$, is considerably longer than the transverse dimension, $x$.
The shaded plaquettes indicate the position of the twist, when
present.}{\epsfxsize\hsize \epsfbox{latticetwist.eps}}

The type of lattice used is shown in \IIFo, with two space and one
(Euclidean) time dimensions. To study the phases of the system, we
construct a Polyakov line at each point in the space dimensions (the
$x-z$ plane), using \IExixb. We impose periodic boundary conditions in
all directions, and set the temperature, specified through the lattice
parameter, to be $\beta \gg \beta_c$, where $\beta_c$ corresponds to
the temperature of the deconfinement phase transition of \IExxv.
Left to its own devices, the entire system will settle into just one of the
$Z(3)$ phases, this being the configuration of lowest energy. An
example of such a configuration, as may be verified from
\IExviiib, is for all $U^\mu_n=1$. We need some way to force the
system into producing a $Z(3)$ interface, and this is achieved by
judicious use of a ``twist''\IRob.

\ifig\IIFi{The effect of the twist: part of the $\tau-z$ plane of
\IIFo\ for fixed $\tau,x$. Polakov lines to the left of the shaded
(twisted) plaquette show a different $Z(3)$ phase from those to the
right.}{\epsfxsize\hsgraph \epsfbox{twist.eps}} 

The twist is introduced by modifying the action \IExviiib\ so that
every plaquette in the $\tau-z$ plane at some particular value of
$\tau$ and $z$ is to be premultiplied by an element, $\vz^{-1}$, of the centre group when it appears in the action. This is illustrated in \IIFo,
with the twisted plaquettes shaded. The action becomes
$${S_W = {6\over g^2}\bigg (
\sum_{shaded\ {\hbox{\tenmsbm P}}} (1 - {\textstyle{1\over 3}}\Real(\vz^{-1}\Tr
U_{\hbox{\tenmsbm P}})) +
\sum_{other\ {\hbox{\tenmsbm P}}} (1 - {\textstyle{1\over 3}}\Real\Tr
U_{\hbox{\tenmsbm P}})\bigg ),}$$
where {\tenmsbm P} represents a plaquette ($U_{\hbox{\tenmsbm P}}$ is
the product of fields around a plaquette, as in \IExviiiaa), and $\vz$ is a member of the
centre group: $\vz\in Z(3)$. Whereas the original action favours
all $U=1$ at high temperatures, so that $U_{\hbox{\tenmsbm P}}=1$, the
twisted part now
favours $U_{\hbox{\tenmsbm P}}=\vz$ to compensate for the
pre-factor. This means that if we order the 
system so that all $U=1$ to the left of the twist, giving
Polyakov lines in the ${\hbox{\tenmsbm Z}}(3)$ phase given by $<L>=1$,
then the twist 
will cause the link variables around the 
twisted plaquettes to behave as in \IIFi, with the right-hand
time-like link given by $U=\vz$. All equivalent time-like links to the
right of the shaded plaquette at the same $\tau$ will also take this
value, so that so that $U_{\hbox{\tenmsbm P}}=1$ again, making $<L>=\vz$
to the right of the twist. No extra energy is associated with the
twist itself; it merely acts as a change of variables,
transforming one 
$Z(3)$ vacuum into another. However, the periodic boundary conditions
force the appearance of a real physical $Z(3)$ interface somewhere else in
the $z$ direction, where the Polyakov lines interpolate from $\vz$
back to $1$. Thus, we have forced the creation of two $Z(3)$ domains
on the lattice, with one $Z(3)$ interface between them. We shall
place the twist at the boundary in our simulations, so that the
left-hand end of the system is in one phase and the right-hand end in another.

One might ask why the interface should form along the $z$ direction
rather than the $\tau$. In our simulation, the fact that $N_t=2$
precludes the formation of an interface in the $\tau$ direction; the
dimension is simply not long enough for any interpolation to
occur. Thus, thermodynamics favour an interface in the $z$
direction, as long as $\beta_T\ll L_z$.

We thus set the initial
conditions of our simulation to be that all link variables are unity
except those in $\{\tau=0\ ,\ 0\leq z\leq L_z/2\ ,\ x\}$, where
they are $e^{2\pi i/3}$. The system is then allowed to
equilibrate before measurements start, using the Monte-Carlo
techniques described below.

\subsec{Monte-Carlo Techniques}
The object of Monte-Carlo methods
\IRxi\ is to evaluate the expectation value
of a quantity not by means of a path integral of high dimension,
$$<\CO>=\frac{\int\CD U \CO e^{-S}}{\int\CD U
e^{-S}},$$
but by a statistical average over gauge configurations $\{U\}_i$,
generated according to the Boltmann distribution $e^{-S}$:
\eqn\IIEi
{<\CO>=\frac{1}{i_{max}}\sum_{i=1}^{i_{max}}\CO(\{U\}_i).}
Each
$\{U\}_i$ represents a set of link variables, $U$, on all links of
the lattice. This technique is one of ``importance sampling'', where
the effort has shifted from the evaluation of the path integral, with
many configurations contributing little, to the generation of
$\{U\}_i$ with the Boltzmann weight. The statistical fluctuations in
the mean value for $\CO$ fall as $1/\sqrt{i_{max}}$ as
$i_{max}\rightarrow\infty$. In practice, many tens of thousands of
configurations are generally needed for a good estimate.

In the ``heat-bath'' algorithm, one starts with a
configuration $\{U\}$, and then changes one of the link variables to
generate a new configuration $\{U'\}$. This new configuration replaces
the old if the rules of the algorithm are satisfied. One ``sweep'' of
the lattice is accomplished by applying this procedure to each link in
turn. The object of the exercise is to generate, first of all, a
configuration at thermal equilibrium: $\{U\}_1$, a member of the Boltzmann
distribution. One then sweeps the lattice again until a new,
statistically independent member of the Boltzmann distribution
is generated: $\{U\}_2$. Repeating this procedure many times, and
calculating $\CO(\{U\})$ for each, one obtains $<\CO>$ through \IIEi.

The heat-bath algorithm
works by touching a heat bath to each link
variable in turn. Consider a particular link $l$ with link variable
$U$: all the links which
interact with $l$ have fixed $U$ matrices, providing a background. On
$l$, one chooses $U'$ from the gauge group $\CG$ with a
probability density proportional to the Boltzmann factor:
\eqn\IIEii
{dP(U')=e^{-\beta S(U')} dU'.}
This algorithm satisfies detailed
balance, ensuring that any ensemble will be brought to equilibrium
eventually. Moreover, since any other algorithm which varies one link
at a time will simulate the heat bath after repeated application,
this method must be the fastest to attain equilibrium in terms of the
number of iterations.
The challenge, therefore, is to ensure that the computational time necessary for a
heat-bath iteration is on a par with that of alternative algorithms.

A suitably fast algorithm for $SU(2)$ was originally suggested by
Creutz\ref\IIRi{M.~Creutz, \PR{D21}{1980}{2308}}, and then an alternative by
Kennedy and Pendleton\ref\IIRii{A.~D.~Kennedy and B.~J.~Pendleton,
\PL{156B}{1985}{393}}.
One can write the Wilson action \IExviiib\ in the form
\eqn\IIEiii
{\beta S_W(U)=\hbox{(constant)} - \beta'\Real\Tr(\Sigma h),}
with
$\beta'=\beta/3$, $\Sigma$ a complex $2\times 2$ matrix equal to
the sum of products of link variables neighbouring $l$, and $h$ the
$SU(2)$ matrix (link
variable) associated with the link $l$ to be updated. Thus, from
\IIEii, the problem reduces to the generation of an $SU(2)$ matrix
obeying the distribution $$Q(h)(dh) \propto e^{\beta'\Real\Tr(\Sigma
h)}(dh),$$ where $(dh)$ is the group-invariant Haar measure.
We can parametrise all $2\times 2$ matrices in terms of the $2\times 2$ unit
matrix, ${\hbox{\tenmsbm I}}$, and the vector of Pauli spin matrices,
${\bf\sigma}$:
$$a=a_0{\hbox{\tenmsbm I}} + i{\bf
a}\cdot{\bf\sigma},\qquad(a_\mu\in{\hbox{\tenmsbm R}}, \quad a^2=a_0^2 +
{\bf a}\cdot{\bf a}=1).$$
In fact, we define $a=uh$ and
$(u_0=\xi^{-1}\Real\Sigma_0,\ {\bf u}=\xi^{-1}\Real{\bf\Sigma})$,
where $a,u \in SU(2)$. In this notation, $\Real\Tr(\Sigma h) =
\xi\Tr a$. Furthermore, the Haar measure takes a simple form, which
can be rewritten in Polar coordinates:
$$(da)=\delta(1-a^2)d^4a=\half\sqrt{1-a_0^2}\
\delta(r-\sqrt{1-a_0^2})\ 
\sin\theta da_0 dr d\theta d\phi.$$
Thus, we need to generate
$a_0$ with the (normalised) probability distribution
$$P(a_0)da_0 = \frac{\alpha}{\pi I_1(\alpha)} \sqrt{1-a_0^2}\
e^{\alpha a_0} da_0,$$
where $\alpha=2\beta' \xi$, the factor of two coming from
$\Tr{\hbox{\tenmsbm I}},$ and $I_1(\alpha)$ is a modified Bessel
function. We then generate $a_i$ uniformly on a
two-sphere of radius $\sqrt{1-a_0^2}$.

The algorithm of Creutz generates such $a_0$ values with an
exponential distribution, and then imposes the square-root factor by
means of an accept/reject procedure. However, for our purposes,
$\alpha$ is generally large, so that the normalisation pre-factor is
small; this leads to a high rate of rejection. The Kennedy-Pendleton
algorithm improves on this by working in terms of a new variable
$\delta=\sqrt{1-a_0}$, so that
$$P'(\delta)d\delta \propto \sqrt{1-\half\delta^2}\ \delta^2
e^{-\alpha\delta^2} d\delta, \qquad (0\leq\delta\leq\sqrt2).$$
This algorithm is faster than that of Creutz for $\alpha\geq 1.7$.
It can be implemented as follows \IIRii:
\item{$\bullet$} Generate four uniformly distributed pseudo-random
numbers in the unit interval: $R, R', R'', R'''$;
\item{$\bullet$} Set $X=-\frac{1}{\alpha}\ln R,\quad
X'=-\frac{1}{\alpha}\ln R',\quad C=\cos^2(2\pi R'')$; 
\item{$\bullet$} Set $\bar\delta=X'+XC$;
\item{$\bullet$} If $R'''^2 > 1-\half\bar\delta$, start again;\ 
otherwise, set $a_0=1-\bar\delta$.
\bigskip

The extension of this algorithm to produce $N\times N$ unitary
matrices with distribution \IIEii\ becomes more and more complicated as $N$
increases, reducing the speed of the procedure, and favouring
alternative algorithms to the heat bath, such as the Metropolis
method\ref\IIRiii{N.~Metropolis, A.~W.~Rosenbluth, M.~N.~Rosenbluth, 
A.~H.~Teller and E.~Teller, \JCP{21}{1953}{1087}}. However, Cabibbo
and Marinari\ref\IIRiv{N.~Cabibbo and E.~Marinari,
\PL{119B}{1982}{387}} proposed 
a faster algorithm for $SU(N)$ based on updating $SU(2)$ subgroups. Their
method consists of first selecting a set $\{F: SU(2)_k,\quad
k=1,\ldots,N-1\}$ of $SU(2)$ subgroups of
$SU(N)$
such that there is no left ideal, {\it i.e.} only the whole $SU(N)$
group is invariant under left multiplication by $F$. The choice of $F$
that we use has elements of the form
$$a_k=\pmatrix{1&&&&&&\cr&\ddots&&&&&\cr&&1&&&&\cr&&&\alpha_k&&&\cr&&&&1&&\cr&&&&&\ddots&\cr&&&&&&1\cr},$$
where $\alpha_k$ is an $SU(2)$ matrix located at the $k$th and
$(k+1)$th rows and columns. 
In each step of the iteration, the new link variable is obtained by
premultiplying the previous value by one matrix from each of the $N-1$
subgroups:
$$U'=a_{N-1} a_{N-2} \ldots a_1 U, \qquad a_k \in SU(2)_k, \qquad (k=1,\ldots,N-1).$$
We obtain the matrices $a_k$ by using the Kennedy-Pendleton algorithm
to choose the appropriate $\alpha_k$. It was shown in \IIRiii\ that
$U'$ emerges with a Boltzmann distribution if $U$ has one; thus, the
procedure is ergodic.

The Monte-Carlo study of lattice gauge theory often suffers from slow
evolution of physical variables, owing to large correlations between
configurations separated only by a few sweeps. Near a second-order
phase transition, ``critical slowing down'' means that the
autocorrelation time of the Monte-Carlo evolution diverges as the
critical point is approached and physical correlation lengths increase.
One way of circumventing this problem is to use ``over-relaxation'' to
accelerate the heat-bath evolution.

This use of over-relaxation was first suggested by
Adler\ref\IIRv{S.~L.~Adler, \PR{D23}{1981}{2901}} for fields with
quadratic coupling in the action. Brown \& Woch\ref\IIRvi{F.~R.~Brown
and T.~J.~Woch,
\PRL{58}{1987}{2394}} and Creutz\ref\IIRvii{M.~Creutz, \PR{D36}{1987}{515}}
extended the procedure to more general theories. The idea is to pick a
trial change for a link variable so that the system goes to an area of
phase space as far as possible from that of the original value without
increasing the energy by a large amount. This is done by finding
roughly the
locus of minimum energy for the variable, and then picking a trial
value on the ``opposite'' side of this minimum. Consider a trial
change of link variable $h\rightarrow h'$. If a group
element $h_0$, independent of $h$, minimises the system energy, then
we wish $h'$ to be on the ``opposite side'' of $h_0$ to $h$, for
instance
$$h'=h_0 h^{-1} h_0.$$
One can use a Metropolis algorithm to accept the new value if the
configuration energy is unchanged or reduced by the change
$h\rightarrow h'$, and accept it with probability $e^{-\Delta S}$ if
it is increased.

For an action of the form \IIEiii, a natural choice for $h_0$ is the
inverse of the group element obtained by projecting $\Sigma$ onto the
group $SU(2)$. For $SU(2)$, $\Sigma$ is always
proportional to a group element, $\tilde\Sigma$. The energy of the new
configuration will be the same as that of the old for $SU(2)$,
so the Metropolis algorithm will always accept this change; the
algorithm is deterministic and microcanonical. To apply this to our
$SU(3)$ system, we again use the $SU(2)$ subgroup procedure of Cabibbo
and Marinari, over-relaxing each of the subgroups of our $SU(3)$
matrices in turn. A previous study\ref\IIRviii{K.~Akemi {\it et al.},
\NP{B (Proc. Suppl.) 30}{1993}{253}}
suggested that for $SU(3)$ gauge theory in $3+1$ dimensions below the
critical temperature, a mixture of seven Brown-Woch over-relaxation steps
followed by one heat-bath step appeared optimal for reducing the
autocorrelation time. Above the critical temperature, their results
did not indicate any particular optimal ratio. For our simulations,
therefore, there appears to be no particular optimal ratio to choose;
we use seven Brown-Woch steps for every one heat bath, after many initial
heat-bath sweeps to equilibrate the system. The link matrices are
renormalised after each sweep, to ensure that rounding errors do not
cause violation of their unitarity. Measurements of
physical operators take place only every four sweeps, to reduce the
correlations caused by adjacent configurations.

\ifig\IIFia{The real (top) and imaginary (bottom) parts of Polyakov lines
on a $2\times 24\times 96$ lattice with twist. The
interface can clearly be seen between the $<L>\approx e^{2\pi i/3}$ domain on
the left and the $<L>\approx 1$ domain on the right. The twist is at
the boundary between $z=0$ and $z=L_z$, and should not be confused with
the position of the interface. The temperature is fairly high
($\beta=50$), resulting in a high suppression of the fluctuations in phase.}
{\epsfxsize\hsgraph \epsfbox{real_imag.ps}}

\ifig\IIFib{The real (top) and imaginary (bottom) parts of Polyakov lines
on a $2\times 24\times 96$ lattice without twist, also with
$\beta=50$.}{\epsfxsize\hsgraph \epsfbox{real_imag2.ps}}

\subsec{The Wandering Interface}
We can see in \IIFia\ an interface on a $2\times 24 \times 96$ lattice
($N_t \times N_x \times N_z$). The longitudinal direction goes across
the page, and the transverse direction into it. The ``height'' in each
case is determined by the value of the Polyakov line, and has nothing
to do with the time dimension, which has been integrated over to form
the Polyakov line.
The twist has been placed at the
boundary of the $z$ direction, as mentioned before, so the left-hand
end of the lattice is in one $Z(3)$ phase with $<L>\approx e^{2\pi
i/3}$, and the right-hand end in another with $<L>\approx 1$. The
temperature is fairly high: $\beta =50 \gg \beta_c$. Thus, the
interface is fairly well-defined and stable, since its free energy
is correspondingly high, suppressing the formation of fluctuations in
phase. In \IIFib, the same system is seen {\it without} a twist.

In this picture, the
interface is roughly in the centre of the lattice. However, the
interface is actually translation invariant; there is nothing in the
action to specify that it should be located at any particular value of
$z$. We shall always start the interface in the centre of the
lattice, as mentioned in section 2.1, but for this chapter, we shall
allow it to
wander freely along the lattice. We can keep track of the interface
most easily by examining a transverse-averaged profile of the Polyakov
lines.

\ifig\IIFii{Profiles of the Polyakov lines on a $2\times 16\times 48$
lattice for $\beta=50$, averaged across the transverse direction. The
real (solid)
and imaginary (dotted) parts of the Polyakov lines are shown. The
first picture shows the initial configuration before Monte-Carlo
evolution begins; the second, the configuration after 20k heat-bath
sweeps; subsequent ones, 40k sweeps apart.}
{\epsfxsize\hsize \epsfbox{walkprofile.ps}}

We can see the interface walking along the lattice in \IIFii. 
Placed at the centre of the lattice before Monte-Carlo evolution
begins (first picture), the interface has taken up its shape of least
energy after twenty thousand (``20k'')
equilibration sweeps (second picture). It has also moved along the
lattice, and continues to do so in subsequent pictures, which are 40k
sweeps apart. In particular,
the interface often approaches the twist. In the 200k
picture, the interface is passing through the twist, and in the 240k
picture, the system has tunnelled into a different $Z(3)$
vacuum: now, $<L>=e^{2\pi i/3}$ on the left and
$<L>=e^{-2\pi i/3}$ on the right. After 260k sweeps, the system has
tunnelled again.

\ifig\IIFiii{The movement of the interface with computer `time', for a
$2\times 24\times 96$ lattice and various $\beta$.}
{\epsfxsize\hsize \epsfbox{randomwalk.ps}}

The movement of the centre of the interface as 
proceeds is shown in \IIFiii, a plot of the square of the position of
the interface centre against the iteration number. To make this
particular measurement, we allow the interface to move each sweep, but
then slide the whole gauge configuration along 
the lattice so that the interface is put back in the middle of the $z$
axis; essentially, we have put the interface on a
treadmill, so that it is allowed to move, without really
going anywhere. This technique will be used throughout the next
chapter, and will be described in more detail there. It is used here simply
to cure problems that would arise in identifying the interface as it
passed through the twist.

In a random walk with step size $a$, the lattice spacing in our case,
the probability that at time $t$
the object will be
at position $z$ is $$P(z,t)=\frac{1}{2}\sqrt\frac{2}{\pi cat}
e^{-z^2/2cat} 2a,$$
implying that $$<z^2(t)>=ca^2 t,$$
where the speed of movement is given by $c$.
The interface, from \IIFiii, clearly obeys this linear relation for
all the values of $\beta$ measured,
demonstrating that it is indeed executing a random walk, in accordance
with translation invariance. As the temperature decreases, the speed
of the walk is seen to increase slightly. This is also expected, as
the energy penalty suppressing fluctuations in phase will decrease as
the temperature drops, allowing the interface to move more swiftly by
combining with, and budding off, fluctuations nearby. We shall look
again at the random walk of the interface in the next chapter, at much
lower temperatures.

\subsec{The Surface Tension}
The free energy of a system is $F=-T\ln Z$, as in \IEiaaa, so $${\del\over
\del \beta} \bigg( {F \over T} \bigg) = {1 \over \beta} <S(U)>.$$
This gives us the behaviour of the free energy in terms of the average
plaquette action. We can perform simulations for the same lattice with
and without twisted plaquettes, {\it i.e.} with and without a $Z(3)$
interface, and the difference in free energy
between the two gives us the free energy of the interface itself, from
which we can measure its surface tension:
$$F_{interface} = F_{twisted} - F_{untwisted} = \alpha A,$$
where $\alpha$ is the surface tension, and $A$ is the `area' of the
interface (in our case, the transverse size of the lattice).
Thus, $${\del\over\del \beta}\bigg( {\alpha A \over T} \bigg) = {1
\over \beta} <\Delta S(U)>.$$
Therefore, recalling \IExvia\ and substituting $A=L_x a$,
\eqn\IIEiv
{\frac{\Delta S}{\beta}\quad=\quad\frac{\del}{\del\beta} \bigg (\frac{\alpha_0
T^{2.5}}{g} \frac{L_x a}{T} \bigg
)\quad=\quad\frac{L_x}{2\sqrt{6\beta}\ 
N_t^{1.5}}\ \alpha_0,}
where we have used \IExviii\ and \IExix\ to substitute for $T$ and
$g$.

The prediction \IExxi\ that $\alpha_0=9.82$ for a system with $N_t=2$
was made in the infinite-temperature limit. Hence, to test this prediction
it is necessary to estimate $\alpha_0$ in this limit. The best way to
do this is to carry out a survey of $\alpha_0$ for various values of
$\beta$, and then to extrapolate the results to the infinite limit.

To estimate $\alpha_0$ for a particular $\beta$, we
need to measure the
difference in total plaquette action between two simulations which
are
identical except for the presence or absence of a twist.
Several tens of thousands of heat-bath sweeps were used to ensure complete
equilibration of the lattice before measurements began. ``Main
sweep'' refers to a sweep after equilibration is complete. As
mentioned in section 3.2, the ratio
of over-relaxed to heat-bath sweeps was seven to one, and measurements of
physical quantities were taken every four sweeps.
A DEC 2100 A500MP machine was used for most of the computation, and
the simulation details are listed in the following table. The CPU time
listed was needed for runs with or without twist, and therefore needs
to be doubled to
give the total time required for an estimate of $\alpha_0$.

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan7\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr \tableedge\tablerule\tablelines
&&#3&&#4&&#5&&#6&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan7&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan7\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\IITi}{Simulation Details}{$\beta$}{Lattice Size}{Heat-Bath
+ Main Sweeps (000's)}{CPU Time (hrs)}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&16&&$2\times 12\times 30$&&15 + 400&&40&\cr
\tablelines\tablerule\tablelines
&&28.125&&$2\times 12\times 36$&&20 + 400&&60&\cr
\tablelines\tablerule\tablelines
&&50&&$2\times 16\times 48$&&20 + 400&&130&\cr
\tablelines\tablerule\tablelines
&&112.5&&$2\times 24\times 72$&&40 + 400&&400&\cr
\tablelines\tablerule\tablelines
&&200&&$2\times 32\times 96$&&40 + 400&&800&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

For each of these runs, with and without twist, we now list the
results for the average action for a single plaquette,
$<S^{\hbox{\tenmsbm P}}>$. This
 has to be multiplied by the total
number of plaquettes ($3\times N_t \times N_z \times N_x$) to give
the total action of the configuration. The difference between the two
values is then used in \IIEiv\ to obtain the
measurements of $\alpha_0$ in the last column.

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan7\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr \tableedge\tablerule\tablelines
&&#3&&#4&&#5&&#6&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan7&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan7\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\IITii}{Simulation
Results}{$\beta$}{$<S^{\hbox{\tenmsbm P}}>_{twisted}$}{$<S^{\hbox{\tenmsbm P}}>_{untwisted}$}{$\alpha_0$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&16&&0.17510(1)&&0.17379(1)&&13.1(1)&\cr
\tablelines\tablerule\tablelines
&&28.125&&0.097575(6)&&0.096832(6)&&11.79(13)&\cr
\tablelines\tablerule\tablelines
&&50&&0.054310(3)&&0.053916(3)&&11.12(12)&\cr
\tablelines\tablerule\tablelines
&&112.5&&0.0239740(7)&&0.0238074(7)&&10.58(6)&\cr
\tablelines\tablerule\tablelines
&&200&&0.0134549(5)&&0.0133644(5)&&10.21(8)&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

One would not expect the finite size of the lattices used to have a
great effect on the untwisted results, as the whole lattice will be in
one phase, but it is less clear how great the effect would be in the
presence of the twist. The shape of the interface may not
flatten out completely at opposite ends of the longitudinal dimension if
the lattice is too short, skewing our measurement
of the total interface free energy. The lattice sizes above were
chosen to be large
enough for the finite-size effects to be negligible, by studying
results for $\beta=50$ on various sizes of lattice and scaling the
spatial dimensions with the interface width, which is proportional to
$\sqrt\beta$, as we saw at the end of section 2.1, and which we choose
as our measure of physical correlation lengths. The only exception to
this was the measurement for $\beta=16$, for which the
lattice could not be safely made any smaller.
The results are given in the following table, each
from 2+20k sweeps. Similar runs without twist gave a 
result of $<S^{\hbox{\tenmsbm P}}>_{untwisted} \approx
0.05390(1)$, and this value was assumed for each lattice in the
calculation of $\alpha_0$:

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan5\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr \tableedge\tablerule\tablelines
&&#3&&#4&&#5&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan5&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan5\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\IITiii}{Finite-Size Survey: $\beta=50$}
{Lattice Size}{$<S^{\hbox{\tenmsbm P}}>_{twisted}$}{$\alpha_0$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&$2\times 16\times 32$&&0.05449(1)&&11.1(3)&\cr
\tablelines\tablerule\tablelines
&&$2\times 16\times 40$&&0.05438(1)&&11.3(3)&\cr
\tablelines\tablerule\tablelines
&&$2\times 16\times 48$&&0.05432(1)&&11.9(3)&\cr
\tablelines\tablerule\tablelines
&&$2\times 16\times 64$&&0.05422(1)&&12.0(3)&\cr
\tablelines\tablerule\tablelines
&&$2\times 24\times 48$&&0.05432(1)&&11.9(3)&\cr
\tablelines\tablerule\tablelines
&&$2\times 24\times 60$&&0.05423(1)&&11.6(3)&\cr
\tablelines\tablerule\tablelines
&&$2\times 24\times 72$&&0.05418(1)&&11.9(3)&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

This suggested, given the errors, that a lattice size of $2\times
16\times 48$ was adequate for $\beta=50$.

Now, as mentioned above, the prediction of \IExxi\ is only valid in the limit
$\beta\rightarrow\infty$, so the question arises of how to extrapolate
our results to test this prediction. This is really a question of
calculating infra-red divergences.
In $3+1$ dimensions, one would
expect the one-loop correction to \IExxi\ to go like $1/\beta$ in
this limit, since it was seen in \IExxib\ that the Debye mass, $m\sim
T$. However, in
$2+1$ dimensions, it is conceivable that a dependence on $\ln\beta$
would need to be taken into account, as this appears in the infra-red
correction for the Debye mass in this case \IExxii. For this reason,
it is difficult to predict the form of the $\beta$-dependence. In any
case, it would be
quite possible for the logarithmic dependence to masquerade as a power
law over a restricted range of $\beta$.

\ifig\IIFivo{Extrapolations of $\alpha_0$ are shown as
$\beta\rightarrow\infty$ for various powers of $\beta$. For each
power, the same five data points are plotted with a particular symbol, and
the accompanying line of extrapolation is marked with a corresponding
label for the x-axis.}{\epsfxsize\hsize \epsfbox{hightemps2.ps}} 

\ifig\IIFiv{Extrapolation of $\alpha_0$ for preferred power of
$1/\beta$ as
$\beta\rightarrow\infty$.}{\epsfxsize\hsize \epsfbox{hightemp1.ps}} 

In the absence of a definite prediction for the form of the
finite-$\beta$ correction, we perform the extrapolation using a best
fit to a power of $1/\beta$. A computer-generated fit to the data,
using the {\it IDL} package and its ``COMFIT'' function
and leaving the power as a free parameter, suggests a
power of $0.85$ with $\chi^2=2.39$. This gives a $\beta=\infty$ limit of
$\alpha_0=9.91(1)$, as extrapolated in \IIFiv. {\it IDL} fits for various
imposed powers
give a lowest $\chi^2$ of $2.34$ for a power of $0.80$, with
$\alpha_0=9.83(1)$. However,
$\chi^2\leq 2.6$ for powers between $0.75$ and $0.90$. Therefore, in
the absence of a definite prediction for the power of $1/\beta$, we
allow for a reasonable error in the fit, and use $0.85(10)$, the range
for which extrapolations are illustrated in \IIFivo.
Thus, our infinite-temperature extrapolation for the interface tension
is
$$\alpha_0=9.91(1)(14),$$ in very good agreement with the instanton
calculation result of \IExxi. The first error is associated with the
fit for $1/\beta^{0.85}$, and the second with the uncertainty in that
value for the power.

It has been argued\IRoe\ 
that the different $Z(3)$ vacua distinguished by different values of
the Polyakov line actually correspond to one and the same physical
state. This claim comes from considering the r\^ole of infra-red
divergences in the calculation of the surface tension, and, if true,
would imply that the surface tension is actually zero (since no
physical interface can exist). The agreement of our results for
$\alpha_0$ with perturbation theory tends to disprove this
argument. It is, of course, conceivable that our measurements for
$\alpha_0$ would dramatically fall towards zero if we went to higher
and higher $\beta$, meaning that our extrapolation is simply an
artefact for the range of $\beta$ that we have considered. However,
our highest value is $\beta\approx 25\beta_c$, a temperature well
above the critical point, and it seems unlikely that any dramatically
different behaviour
will set in at a temperature higher than this. A sceptic could
also argue that a lattice with $N_t=2$ could show behaviour quite
distinct from that in the continuum; but quite apart from the agreement with
the lattice prediction of $\alpha_0$ for this value of $N_t$, a
similar survey carried out for $SU(2)$ gauge theory for a range of
$N_t\leq 5$ has found similar agreement with perturbation
theory\ref\IIRx{C.P.~Korthals~Altes, A.~Michels, M.~Stephanov and
M.~Teper, \NP{B (Proc. Suppl.) 42}{1995}{517}}.

\subsec{The Debye Mass}
To measure the Debye mass on the computer, we need to study the
correlations of fluctuations in the gauge fields. The behaviour of
these correlations will give us information about the Debye screening
of sources, as in \IEix. We need to find a ``good''
operator, {\it viz.} one whose correlator rapidly converges to a decaying
exponential of only the lowest mass state. This will allow us to obtain,
in a straightforward manner, an estimate for this lowest mass. A simple
plaquette correlator does not fit our requirements, as it depends on
flux loops between the plaquettes being considered, and thus has to be
considered over a long range of separation before a single exponential
dominates. However, a good operator turns out to be given by a
transverse average of Polakov lines, as shown in \IIFii.

\ifig\IIFiva{Estimation of the Debye mass from $\mu(z)$ for untwisted
data at $\beta=200$.}{\epsfxsize\hsize \epsfbox{debye_2oon.ps}} 

We measure the correlation function of this operator along the
untwisted lattice, as it happens to be easier to obtain accurate
results from this system than from the twisted lattice, where the
$Z(3)$ interface acts as a dominating source term and the Debye mass can be
estimated from the shape of its tail. Owing to the periodic boundary
conditions in the
space directions, we expect a fluctuation at one value of $z$ to
influence another point further along the lattice by correlations
going in the $+z$ {\it and} $-z$ direction. This gives correlations,
at long distances, proportional to $e^{-2mz}$ (as in section 2.4) {\it
and} $e^{-2m(L_z-z)}$.
Therefore, we estimate $2m$ by a cosh fit, an improvement on the following
function which fits simply to a decaying exponential:
$$\mu(z)=\ln\bigg(\frac{<L^\dagger(z-1)L(0)>-<\bar
L>^2}{<L^\dagger(z)L(0)>-<\bar L>^2}\bigg),$$
where each $<L(z)>$ represents an average of $L(z)$ over all configurations
(sweeps), and $<\bar L>$ is a further average over all $z$. From the
definition of the Debye mass, we expect
$$\mu(z\rightarrow\infty)\rightarrow 2m.$$

In \IIFiva, a typical set of data is shown for $\mu(z)$ at high
$\beta$. For each similar set of data, we extracted a value of
$\mu(z)$ corresponding to the level at which the function flattened
out before errors began to increase wildly. These values are given in
the following table for the simulations listed in \IITi, in units of
the inverse lattice spacing.

\bigskip\centerline{\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan3\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr \tableedge\tablerule\tablelines
&&#3&&#4&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan3&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan3\cr}
\halign to10cm{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & 
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\IITiv}{Debye (Electric) Mass (units of $a^{-1}$)}
{$\beta$}{Twice Debye mass, $\mu=2m$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&16&&0.80(1)&\cr
\tablelines\tablerule\tablelines
&&28.125&&0.690(5)&\cr
\tablelines\tablerule\tablelines
&&50&&0.555(5)&\cr
\tablelines\tablerule\tablelines
&&112.5&&0.410(5)&\cr
\tablelines\tablerule\tablelines
&&200&&0.332(4)&\cr
\tablelines\tablerule}}\global\advance\tableno by1}}\bigskip

\ifig\IIFv{Results for the Debye mass. The prediction of \IExxiv\ is
plotted to leading-order only (dashes, C.F. \IFiv); with an
additional correction of $\ln(\ln(\beta/12))$ (dots); and with an
alternative additional correction of\break
$0.14\ln(\ln(\beta/12))+0.94$ (dot-dashes).}
{\epsfxsize\hsize \epsfbox{mass.ps}}

The values are plotted in \IIFv,
together with the theoretical prediction from \IFiv\ (dashed line),
which is expected to be
valid in the high-temperature continuum limit.
The results show some qualitative agreement with the leading-order
prediction of \IExxii\ and \IExxiv, as plotted previously in
\IFiv. However, although the shape of the rise of the mass with
temperature looks correct, the results differ from the prediction by a
factor of two or so. The reason for this becomes clearer when we
consider the size of the $O\bigg[\ln(\ln(\beta/12))\bigg]$ correction
compared to the leading-order $\frac{3}{4\pi}\ln(\beta/12)$ that we
plot: for our range $16<\beta<200$, the leading-order term is between
$0.1$ and $0.7$, but the correction is $O(-1.2)$ to $O(1.0)$! Thus, we
shall find it very difficult to draw any firm conclusions from the
data to support or deny the prediction.

To show the effect of the correction, the dotted curve in
\IIFv\ is $\frac{3}{4\pi}\ln(\beta/12)+\ln(\ln(\beta/12))$. Our
data certainly look more reasonable when this correction is included,
but, of course, this estimate is only of the order of the correction,
not of an exact expression. A free fit to a correction of the form
``$c_1\ln(\ln(\beta/12)) + c_2$'' gives the dot-dashed line in the
\IIFv, with $c_1\approx 0.14$ and $c_2\approx 0.94$, which shows
extremely good agreement with our data. Although we have two free
parameters and only five data points, the fit is strikingly good, and
this gives us some reason to hope that our data is consistent with the
theoretical prediction. Of course, no firm conclusions can be drawn
without a more explicit expression for the
$O\bigg[\ln(\ln(\beta/12))\bigg]$ correction. However, the ratio of
coefficients of the free fit does at least confirm that most of the
temperature dependence is contained within the leading
$\frac{3}{4\pi}\ln(\beta/12)$ term.

\vfill\supereject

==> intro1.tex <==
\newsec{Phases in SU(3) Gauge Theory:}{Theoretical Preliminaries}

\Subsec{Prologue: Phases in Physics}
Many physical systems possess assorted phases, undergoing transitions
between the different phases under certain conditions, for instance at
a particular temperature. Obvious examples
include $H_2O$, with phases as ice, water and steam and transitions at
$0^oC$ and $100^oC$, and ferromagnets, with ferro- and paramagnetic
phases. Phase transitions in systems such as these have been studied
extensively in the past. Where different phases coexist, interfaces
can form between them, and the interfaces have also been objects of
previous study\ref\IRooo{{\it E.g.} G.~Forgacs, R.~Lipowsky and
Th.M.~Nieuwenhuizen in {\it ``Phase Transitions and Critical
Phenomena''}, vol. 14, Academic Press Ltd. (London) 1991 (ed. C.~Domb
and J.~Lebowitz), {\it and references therein}}.

Quantum chromodynamics (QCD) is now generally accepted as the theory
responsible
for the ``strong force'' of particle physics. The gluon sector of this
theory is described by the $SU(3)$ gauge theory. This gauge theory
itself exhibits several phases at finite temperatures, as will be
detailed in the following
sections. Interfaces can form between the different phases, and this
thesis is concerned with the study of several properties of one
particular type of interface, which may be of relevance to cosmology
and to the heavy ion collision experiments of nuclear physicists at
the Relativistic Heavy Ion Collider.

This chapter will begin with some fundamentals of field theories at
finite temperature, in particular $SU(3)$ gauge theory. It will then
continue with a discussion of the types of interface present in the theory,
the mathematical framework for their description,
and some of the predicted properties of one of the types. Subsequent
chapters will proceed to consider this one particular type of interface,
first at high temperatures, where it is most stable, and then at lower
temperatures, where it is close to collapse.

\subsec{Introduction: Phases in SU(3) Theory}
It has been known for some time that pure gauge theories have a
non-confining high-temperature phase\ref\IRoo{A.~Polyakov,
\PL{B72}{1978}{477}}.
This was first shown non-perturbatively, in the strong-coupling limit
of Hamiltonian lattice gauge theory\ref\IRooa{L.~Susskind,
\PR{D20}{1979}{2610}}.
In this situation, for instance, Abelian gauge
theory can be shown to reduce to the ``Villain model''. This is a well studied
statistical-mechanical system which is known to be disordered at high
``Villain temperature'', with a pair of opposite charges experiencing
a confining linear potential; and ordered at low temperature, with a normal
Coulomb potential. The Villain temperature is actually inversely
proportional to the temperature, $T$, defined in gauge theory, which is
used from now on. Therefore, any theory in a
confining phase at $T=0$ must have a phase transition at
some finite temperature, called the critical temperature ($T_c$), separating
the confining and non-confining phases. These ideas are supported by
numerical simulations\ref\IRoob{H.J.~Rothe, {\it ``Lattice Gauge
Theories''} (ch. 19---20), World Scientific (1992)}.

A consideration of QCD at finite temperatures reveals that
the pure gauge $SU(3)$ sector has the two expected
phases. At low temperatures, there is the ``disordered'' phase where the
colour charge of QCD is confined, and the vacuum is symmetric under
the group $Z(3)$, the ``centre'' of the $SU(3)$ group (as discussed
further in section 1.7). This is why no
free quarks are seen in the relatively cool universe of today.
At high temperatures, though, one finds a
 non-confining, $Z(3)$-breaking ``ordered'' phase, corresponding to
the free quark-gluon ``plasma'' believed to exist in the hot early
universe. In fact,
owing to the $Z(3)$ breaking, there exist three different
high-temperature (high-$T$) phases, namely three degenerate vacua,
corresponding to the three members of $Z(3)$, the cube roots of
unity. Fermionic matter breaks the vacuum degeneracy, albeit on a
small scale, so we consider only the pure gauge theory in what follows.

It is apparent that two different types of interface are possible
in the theory. First, there is one between the ordered and
disordered phases; this type is only stable at the critical
temperature, since only then do the temperature and pressure match
on both of its sides. Second, an interface can form between two of the
ordered phases with different $Z(3)$ vacua, and this is usually called
an ``order-order interface'', or ``$Z(3)$ interface''. All
thermodynamic quantities are the same on both sides of a $Z(3)$
interface, but they dip slightly across the object itself. Clearly,
this second type of interface can only exist above the critical
temperature, as only there does one find the ordered phases themselves.

The aim of this thesis is to study some properties of
the $Z(3)$ interfaces, by means of Monte-Carlo simulations on a
Euclidean lattice, in two very different temperature regimes: first, in
the high-$T$ limit, where analytic predictions have been made
concerning properties such as the surface tension and Debye
screening mass of the interface; and second, just above the critical
temperature, where the interfaces are in the process of collapse.

\subsec{Cosmological Implications}
Possible cosmological significance has been claimed for these
interfaces in the past, in the r\^ole of domain walls in the early
universe, which could be responsible for matter
formation\ref\IRo{V.~Dixit and M.~C.~Ogilivie,
\PL{269}{1991}{353}}\ref\IRoa{J.~Ignatius, K.~Kajantie and
R.~Rummukainen, \PRL{68}{1992}{737}}. The
suggested process is that of bubble nucleation, forming hadronic
matter during the phase transition from the high-$T$ quark-gluon
plasma to the low-$T$ hadronic phase.
It has been believed for some time\ref\IRoao{Z.~Frei and A.~Patk\'os,
\PL{B229}{1989}{102}},
and has been shown in
simulations\ref\IRob{K.~Kajantie, L.~K\"arkk\"ainen and
K.~Rummukainen, \NP{B357}{1991}{693}}\ref\IRobo{R.~Brower, S.~Huang,
J.~Potvin, C.~Rebbi and J.~Ross, \PR{D46}{1992}{4736}; B.~Grossmann,
M.~L.~Laursen, T.~Trappenberg and U.-J.~Wiese, \NP{B396}{1993}{584}},
that the interfaces of $SU(3)$ show something called ``complete
wetting''.
The meaning of this is that a $Z(3)$ interface between two ordered phases
really consists of two order-disorder interfaces stuck back to back, leaving
a very thin slice of disorder between two ordered domains. One
possible scenario for the formation of hadronic matter in the early 
universe envisages many different domains of ordered phase at high
temperature, separated by $Z(3)$ interfaces. As the temperature drops
towards the critical value, the interfaces start to widen; and when
the temperature hits the critical value, the constituent
order-disorder interfaces split apart, spreading
the slice of disordered hadronic phase outwards.

However, it has more recently been emphasised\ref\IRoba{V.~M.~Belyaev,
I.~I.~Kogan, G.~W.~Semenoff and N.~Weiss,
\PL{B277}{1992}{331}}\ref\IRoc{N.~Weiss, UBCTP93-23
(hep-ph/9311233)}\ref\IRod{I.~I.~Kogan, \PR{D49}{1994}{6799}} that the
order parameter
distinguishing the $SU(3)$ phases is fundamentally a Euclidean object,
with no counterpart in Minkowski space. Thus, whilst the $Z(3)$
symmetry exists, and hence $Z(3)$ domains and interfaces exist, in the
Euclidean path integral, it is less certain that the interfaces can exist
as physical objects in the universe. The claim has even been
made\ref\IRoe{A.~V.~Smilga, \AP{234}{1994}{1}} that only one true physical
phase exists, even in Euclidean space, at high temperatures, and we
shall address this when discussing our results later. In Minkowski
space, the interfaces have been shown\IRoc, on current understanding,
to have unphysical thermodynamic quantities when a certain number of
fermion families is considered in addition to the gauge fields,
resulting from the unusual fact that the ordered phases occur at {\it high}
temperatures. The free energy, $F$, is proportional to the fourth
power of the temperature with a {\it positive} coefficient
for many $SU(N)$ systems with varying
numbers of fermion families present: $F=|\gamma| T^4$. Thus, the pressure,
$P=-|\gamma|T^4$; the internal energy, $E=-3|\gamma|T^4$; the specific
heat, $C=-12|\gamma|T^3$; and the entropy, $S=-4|\gamma|T^3$. 

As pointed out in \IRod, no physical systems of this type can exist
with positive temperature, but metastable states can exist with
inverse population, {\it i.e. negative} temperature, flipping the sign
of the specific heat and entropy as desired, and forming a type of
quark-gluon ``laser''.
The problem may be assuaged by embedding the interface within a system
whose positive entropy exceeds the negative entropy of the interface
itself, and such a system has recently been
postulated\ref\IRii{C.~P.~Korthals~Altes, {\it private
communication}}, 
with the interface contained within a larger volume of metastable vacuum in
the early universe. However, it is noted in \IRod\ that any
statistical description of a
system containing even a subsystem of negative entropy must fail,
since no states are available to the subsystem. For
instance, the standard electroweak model well above the QCD phase
transition has negative free energy density\IRo\IRoa, thanks to the
contributions of the leptons, Higgs and weak gauge bosons; but if we
consider the case where the quark-gluon subsystem has $F_{qg}=|\gamma|
T^4$, then the weak coupling of the other particles cannot rectify
the situation.
Even setting this problem aside, the problem of interpretation of the
interface remains, as the order parameter is non-local in Euclidean
time, corresponding to an imaginary time-like gauge field in Minkowski
space, and thus an imaginary chemical potential for the colour
charge\ref\IRof{A.~Roberge and N.~Weiss, \NP{B275}{1986}{734}}. {\it
Adhuc sub judice lis est...} In any event,
by virtue of their contribution to the partition function
and to expectation values calculated using the Euclidean path
integral, the interfaces must be included in a non-perturbative
analysis of the thermodynamics of QCD, if only (like the instanton) as a
calculational device without physical form in our universe.

In order to make analytical predictions about the interfaces, a
mathematical description of them is necessary. For this reason, the next
sections introduce some elements of quantum field theory at finite
temperatures which will be of use in future chapters.

\subsec{The Partition Function and Thermodynamics}
One now introduces a Schr\"odinger field operator at time $t$,
$\hat\phi(\vx, t)$, and its conjugate momentum operator,
$\hat\pi(\vx, t)$\ref\IRiv{C.~Bernard, \PR{D9}{1974}{3312}; for a more recent
exposition, see {\it e.g.} J.~I.~Kapusta, {\it ``Finite-Temperature Field
Theory''}, CUP, Cambridge (1989)}.
For convenience, one labels the eigenstates
of the field operator at $t=0$ as $|\phi>$, satisfying
$$\hat\phi(\vx, 0) |\phi> = \phi(\vx)|\phi>,$$ with eigenvalue
$\phi(\vx)$. The amplitude for a transition from initial state
$|\phi_i>$ at $t=t_i$ to final state $|\phi_f>$ at $t=t_f$ is then given,
as usual, by the
following functional integral in $(d-1)$ space and one time ($d$ or
``$(d-1)+1$'') dimensions:
\eqn\IEi
{<\phi_f|e^{-iH(t_f-t_i)}|\phi_i>=\int\CD\pi\CD\phi
\ e^{i\int^{t_f}_{t_i} dt \int d^{d-1}x (\pi\dot\phi -
\CH(\pi,\phi))}.}
The integral over $\pi$ is without restriction, but the integral over
$\phi$ is constrained by the requirements that $\phi(t=t_i)=\phi_i$ and
$\phi(t=t_f)=\phi_f$. $H$ is the Hamiltonian, and $\CH$ the Hamiltonian
density.

Now, the partition function of a statistical mechanical system in
thermodynamic equilibrium is given by
\eqn\IEiaa
{Z=\Tr\ e^{-{\beta_T} H}=\int d\phi <\phi|e^{-{\beta_T} H}|\phi>,}
where ${\beta_T}$ is the inverse temperature,
$T^{-1}$, and the integral sums over all states. From
$Z$, all thermodynamic properties can be calculated:
\eqn\IEiaaa
{F=-{1\over{\beta_T}} \ln Z \qquad P=-{\del F\over\del V}\bigg |_T \qquad
S=-{\del F\over\del T}\bigg |_V \qquad etc...}
Also, the expectation value of any operator is simply given by:
\eqn\IEiaab
{<\hat\CO>=\frac{1}{Z}\Tr\big (\hat\CO e^{-{\beta_T} H}\big ).}

We now generalise \IEi\ and \IEiaa\ to the logical conclusion of a
path integral over gauge fields, before turning to consider how to
distinguish between the different phases of a gauge theory
at finite temperatures.

\subsec{Finite-Temperature Field Theory} 
One can make \IEi\ look more suggestive for $Z$ by introducing an
imaginary time coordinate $\tau=it$ and putting $t_i=0$ and $it_f={\beta_T}$,
giving $$<\phi_f|e^{-{\beta_T} H}|\phi_i>=\int\CD\pi\CD\phi
\ e^{\int^{\beta_T}_0 d\tau \int d^{d-1}x (i\pi\dot\phi -
\CH(\pi,\phi))},$$ where previous functions of $t$ are now functions
of $\tau$, and $\dot\phi\equiv{\del\phi\over\del\tau}$. This enables
one to write $$Z=\int\CD\pi\int_{\rm
periodic}{\hskip-2em\relax}\CD\phi
\ e^{\int^{\beta_T}_0 d\tau \int d^{d-1}x (i\pi\dot\phi -
\CH(\pi,\phi))},$$ where the periodic boundary conditions on $\phi$
are that $\phi(\vx,0)=\phi(\vx,{\beta_T})$, arising from the trace in
\IEiaa. This periodicity restricts the energy
values associated with the fields to a set of discrete values.

For a general renormalisable scalar field Hamiltonian,
$$\CH=\pi^2-\CL(\phi, \del_\mu\phi),$$ with $\CL$ being the
Lagrangian. One can perform the integration over $\pi$ to give
$$Z=\int_{\rm periodic}{\hskip-2em\relax}\CD\phi
\ e^{\int^{\beta_T}_0 d\tau \int d^{d-1}x \CL(\phi,\del_\mu\phi)},$$
where the (irrelevant) normalisation constant has been discarded, and
the Lagrangian is Euclidean.

This technique can be extended straightforwardly to gauge
fields. When applied to quantum electrodynamics (QED), for instance,
one obtains the following functional integral for the electromagnetic
field alone, given for an arbitrary
gauge specified by $\CF=0$, where $\CF$ is a general function of the
vector potential, $A^\mu$, and its derivatives:
$$Z=\int_{\rm periodic}{\hskip-2em\relax}\CD A^\mu \delta(\CF)
\det\bigg ({\del \CF\over\del\alpha}\bigg )\ e^{\int^{\beta_T}_0 d\tau \int
d^{d-1}x (-\frac{1}{4}F_{\mu\nu}F^{\mu\nu})}.$$
The electromagnetic field tensor $F^{\mu\nu}=\del^\mu A^\nu -
\del^\nu A^\mu$, no colour indices being contained within $A^\mu$ for QED,
and $\alpha(\vx, t)$ specifies possible gauge transformations.

For a general gauge group $\CG$, with generators $T^a$ and structure
constants $f_{abc}$, the usual vector potential acquires a colour
index, $A^\mu_a$, and thence the field strength becomes
$$F^{\mu\nu}_a=\del^\mu A^\nu_a - \del^\nu A^\mu_a - gf_{abc}A^\mu_b
A^\nu_c,$$ introducing dimensionless coupling $g$. For a general gauge
group $SU(N)$, $a$ runs from $1$ to $N^2-1$. In a convenient shorthand,
we shall later write the product over colour indices as $A^\mu={\bf
A^\mu}\cdot{\bf T}$. The infinitesimal gauge transformations are now given by
$\alpha_a(\vx,t)$, and there are $N^2-1$ gauge-fixing functions
specified by $\CF^a$, so
\eqn\IEia
{Z=\int_{\rm periodic}{\hskip-2em\relax}\CD A^\mu_a \delta(\CF^b)
\det\bigg ({\del \CF^c\over\del\alpha^d}\bigg )\ e^{\int^{\beta_T}_0 d\tau \int
d^{d-1}x (-\frac{1}{4}F_{\mu\nu}^a F^{\mu\nu}_a)}.}
To work in a physical gauge, one can simply choose $\delta(\CF^b)$ to
pick such a gauge within the generating functional above. 
However, it is often more convenient to work in an unphysical gauge
such as the covariant gauge, where ghost fields $\eta_a, \bar\eta_a$
are introduced to give
$$Z=\int_{\rm periodic}{\hskip-2em\relax}\CD A^\mu_a \CD \bar\eta_a
\CD \eta_a\ e^{\int^{\beta_T}_0 d\tau \int
d^{d-1}x (-\frac{1}{4}F_{\mu\nu}^a F^{\mu\nu}_a -
\frac{1}{2\xi}(\del_\mu A_a^\mu)^2 + gf^{abc}\bar\eta_a
\del_\mu A^\mu_b \eta_c + \del_\mu\bar\eta_a\del^\mu\eta_a)}.$$

\subsec{The Polyakov Line and Confinement}
The phases of a thermal gauge theory are characterised by the free
energies of static configurations of quarks and
antiquarks\ref\IRv{L.~D.~McLerran and B.~Svetitsky, \PR{D24}{1981}{450}}.
To calculate such free energies, one needs to consider
creation and annihilation operators,
$\psi^\dagger_a(\vx_i,t)$ and $\psi_a(\vx_i,t)$, for static quarks
with colour $a$ at position $\vx_i$ and time $t$, together with
charge conjugates, $\psi^{\dagger c}_a$ and $\psi^c_a$, for
antiquarks. All equal-time anticommutators of these fields vanish with
the exception of
\eqn\IEii
{\{\psi_a(\vx_i,t),\psi^\dagger_b(\vx_j,t)\}=\delta_{ij}\delta_{ab}}
and its charge conjugate.

For the general gauge group $\CG$ of the previous section, using the
shorthand defined there for $A^\mu$, the quark fields obey the static
time-evolution equation $$\bigg (-i\frac{\del}{\del \tau} - 
gA^0(\vx_i,\tau)\bigg )\psi(\vx_i,\tau)=0,$$
whence integration yields
\eqn\IEiii
{\psi(\vx_i,\tau)=\CT \big ( e^{ig\int_0^\tau d\tau' A^0(\vx_i,\tau')}\big ) \psi(\vx_i,0).}
Consider states $|\Psi>$ containing heavy quarks at
$\vx_1,\ldots,\vx_{N_q}$ and antiquarks at $\vx_1',\ldots,\vx_{N_{\bar
q}}'$. The free energy of a collection of $N_q$ quarks and $N_{\bar q}$
antiquarks is given by a sum over all such states, from \IEiaa\
and \IEiaaa:
\eqn\IEiiia
{e^{-{\beta_T} F(\vx_1,\ldots,\vx_{N_q},\vx_1',\ldots,\vx_{N_{\bar
q}}')} \sim \sum_{|\Psi>} <\Psi|e^{-{\beta_T} H}|\Psi>.}
Using the quark field operators, one can rewrite this
expression in terms of new states $|\tilde \Psi>$ without heavy quarks:
\eqnmulti\IEiv
{e^{-{\beta_T} F_{N_q N_{\bar q}}} &\sim \sum_{|\tilde \Psi>} \bigg <\tilde
\Psi\ \bigg |
\sum_{\{a,b\}} 
\Psi_{a_1}(\vx_1,0)\ldots\psi_{a_{N_q}}(\vx_{N_q},0)\psi^c_{b_1}(\vx_1',0)
\ldots\psi^c_{b_{N_{\bar q}}}(\vx_{N_{\bar q}}',0)} 
{&\qquad\times e^{-{\beta_T} 
H}\psi^\dagger_{a_1}(\vx_1,0)\ldots\psi^\dagger_{a_{N_q}} 
(\vx_{N_q},0)\psi^{\dagger c}_{b_1}(\vx_1',0)
\ldots\psi^{\dagger c}_{b_{N_{\bar q}}}(\vx_{N_{\bar q}}',0)\ \bigg |\ \tilde
\Psi\bigg >.}
Remembering that $e^{-{\beta_T} H}$ will evolve an operator $\hat O(\tau)$ in
Euclidean time ($\hat O(\tau+{\beta_T}) = e^{{\beta_T} H} \hat O(\tau) e^{-{\beta_T}
H}$), one now introduces pairs of exponentials $e^{-{\beta_T} H}
e^{{\beta_T} H}$ to the left of each destruction operator in
\IEiv. Evolving these operators to time $\beta_T$ and using the
anticommutation properties to group operators into pairs at the same
location, one obtains
\eqnmulti\IEv
{e^{-{\beta_T} F_{N_q N_{\bar q}}} \sim \sum_{|\tilde \Psi>} \bigg <\tilde
\Psi\ \bigg |
\sum_{\{a,b\}} 
e^{-{\beta_T} H}\psi_{a_1}(\vx_1,{\beta_T})\psi^\dagger_{a_1}(\vx_1,0)\ldots\psi_{a_{N_q}}(\vx_{N_q},{\beta_T})
\psi^\dagger_{a_{N_q}}(\vx_{N_q},0)} 
{\qquad\times\psi^c_{b_1}(\vx_1',{\beta_T})\psi^{\dagger c}_{b_1} 
(\vx_1',0)\ldots\psi^c_{b_{N_{\bar q}}}(\vx_{N_{\bar q}}',{\beta_T})
\psi^{\dagger c}_{b_{N_{\bar q}}}(\vx_{N_{\bar q}}',0)\ \bigg |\ \tilde
\Psi\bigg >.}
Using \IEii\ and \IEiii, one can finally write
\eqn\IEvi
{e^{-{\beta_T} F_{N_q N_{\bar
q}}} = \Tr \big ( e^{-{\beta_T} H} L(\vx^q_1) \ldots
L(\vx^q_{N_q}) L^\dagger(\vx^{\bar q}_1) \ldots L^\dagger(
\vx^{\bar q}_{N_{\bar q}})\big ),}
where the trace is taken over states of the pure gluon theory, and
$L(\vx)$ is the ``Polyakov line'', sometimes called the ``Wilson
line'' ($\CT$ denotes time ordering):
\eqn\IEvia
{L(\vx)=\Tr\Omega(\vx), \qquad \hbox{with} \qquad
\Omega(\vx)\sim\CT e^{ig\int_0^{\beta_T} d\tau A^0(\vx_i,\tau)}}
In particular, the normalisation in \IEiiia\ for gauge group $SU(N)$
is $\frac{1}{N^{N_q+N_{\bar{q}}}}$, and $$\Omega(\vx)=\frac{1}{N}\CT
e^{ig\int_0^{\beta_T} d\tau A^0(\vx_i,\tau)}.$$
Recalling \IEiaab, one divides \IEvi\ by the vacuum, {\it viz.} the
equivalent with $N_q=N_{\bar q}=0$, to give
$$e^{-{\beta_T} \Delta F_{N_q N_{\bar
q}}} = < L(\vx^q_1) \ldots
L(\vx^q_{N_q}) L^\dagger(\vx^{\bar q}_1) \ldots L^\dagger(
\vx^{\bar q}_{N_{\bar q}})>,$$
where $\Delta F = F_{N_q N_{\bar q}} - F_{00}$.

In particular, the expectation value of a single Polyakov line
gives the
self-energy of a single quark in the gluon medium ($F_q\equiv\Delta
F_{10}$):
$$e^{-{\beta_T} F_q}
= <L(\vx)>.$$ Since these quarks are static and infinitely
heavy, $F_q$ is meaningless in itself. However, the
correlation function of two Polyakov lines, $\Gamma$, gives the static
quark-antiquark free energy ($F_{q\bar q}\equiv\Delta F_{11}$):
$$e^{-{\beta_T} F_{q \bar q}(\vx - \vy)} =
<L(\vx) L^\dagger(\vy)> = \Gamma(\vy -\vx).$$
Static quarks will be confined if this correlation function vanishes
as $|\vx - \vy| \rightarrow \infty$, but
cluster decomposition
demands that $$\Gamma(\vx) = <L(0) L^\dagger(\vx)>
\mathrel{\mathop{\longrightarrow}\limits_{|\vx| \rightarrow
\infty}} <L(0)><L^\dagger(\vx)> = |\!<L(0)>\!|^2$$
so that $F_{q \bar q}(\vx)
\mathrel{\mathop{\longrightarrow}\limits_{|\vx| \rightarrow
\infty}} 2F_q$, and so this condition is equivalent to $<L(\vx)>=0$,
showing that the insertion of a single quark requires infinite
energy, {\it i.e.} the theory is in a confining phase. In contrast, if
$<L(\vx)>\neq 0$ then $F_{q\bar q}(\vx)$ will be finite and the colour
charge deconfined. Thus, the Polyakov line gives an effective test for
confinement.

\subsec{The Centre Symmetry and its Breaking}
Turning again to the expression for the generating functional in \IEia, one
is now led to consider the symmetries of the Euclidean action, 
$$\CS_E=\int d\tau d^{d-1}x F^a_{\mu\nu}F_a^{\mu\nu},$$ and the behaviour
of the Polyakov line under the symmetry-related transformations.

Returning to the shorthand notation of section 1.5, one sees that under a
general non-Abelian gauge transformation
\eqn\IEvii
{A^\mu \rightarrow UA^\mu
U^{-1} + iU\del^\mu U^{-1},\qquad U(\vx,t) \in SU(N)}
the Polyakov line will transform in the following manner:
\eqn\IEviii
{L(\vx) \rightarrow \Tr \big ( U(\vx,0) \Omega(\vx)
U^\dagger(\vx,{\beta_T})\big ).}
This means that $L$ is invariant if $U$ is periodic in time. However,
$\CS_E$ is actually invariant under a larger
group than merely the periodic gauge transformations; the only
physical restraint is that the gauge potentials remain periodic in
time. Let $U(\vx,t+{\beta_T})=zU(\vx,t)$ in \IEvii; since $A^i$ must be
single-valued,
this tells one that $z$ must be independent of $\vx$,
satisfying $z^{-1}A^iz=A^i$. This almost always implies that $z$ is
an element of $\CC$, the ``centre'' of the gauge group (the set of
elements which commute with all members of the group): $\CC =
\{ z \in G | zgz^{-1} = g$ for all $g \in G \}$. This global symmetry
is an invariance under gauge transformations which are only periodic
up to an element of the centre; it leaves local observables unchanged, and
it remains after all gauge fixing. However, \IEviii\ reveals that the
topologically non-trivial
Polyakov line, which wraps around the periodic boundary condition in
the time direction, is not invariant under these transformations, but rather
is rotated by an element of the centre: $$L(\vx) \rightarrow zL(\vx).$$

For the $SU(N)$ groups, the centre is $Z(N)$, whose elements are the
$N$th roots of unity, $e^{2\pi iq/N}$ ($q=0,1,\ldots,N-1$). This
$Z(N)$ symmetry may not be dynamically realised, however: if it is
impossible to interpolate from one $Z(N)$ vacuum to another through
field configurations of finite energy and measure, the
symmetry will be spontaneously broken. In the absence of such
breaking, $<L(\vx)>$ must vanish, corresponding
to $F_q=\infty$. This will lead
to an exponential decay of the correlation function at large
distances: $$\Gamma(\vx) \sim e^{-\sigma |\vx| /T}.$$ From the
expression for the free energy of a quark-antiquark pair given
earlier, we obtain a linear potential with string tension
$\sigma(T)$: a confining phase. However, the symmetry could be broken
at some finite temperature, with $N$ possible
broken-symmetry ground states (vacua) for the pure gauge system.

How can the symmetry be broken at high temperatures? Consider the
continuum generating functional again, for a moment, absorbing the
dimensionless coupling through $g A^\mu \rightarrow A^\mu$:
\eqn\IEixa
{Z=\int_{\rm periodic}{\hskip-2em\relax} \CD A^\mu
e^{-{1 \over g^2}\int_0^{\beta_T} d\tau \int d^{d-1}x {1\over 4}\Tr
F^2_{\mu\nu}}.}
If one rescales $\tau \rightarrow {\beta_T} \tau, A^0 \rightarrow
A^0/{\beta_T}$, this can be rewritten as
\eqn\IEx
{\int \CD A^\mu
e^{-{1 \over g^2T}\int_0^1 d\tau \int d^{d-1}x {1\over 2}\Tr
(T^2 {\bf E}^2 + {\bf B}^2)}, \qquad \hbox{with} \qquad
A^0(\tau=1)=A^0(\tau=0),}
where the electromagnetic tensor has been written explicitly in
terms of its electric and magnetic components. As $T \rightarrow
\infty$, the only non-zero contributions will come from field
configurations with ${\bf E} = 0$, implying that $A^i$, the spatial
components of the gauge potential, must be static up to a gauge
transformation. This, together with the boundary conditions on $A^0$,
implies that $\Omega(\vx)$ must be an element of the centre
group\ref\IRvii{B.~Svetitsky and L.~G.~Yaffe,
\NP{B210[FS6]}{1982}{423}}. 
Thus, as $L(\vx) = \Tr \Omega(\vx)$, one sees that
\eqn\IExi
{<\!L\!> = e^{2\pi iq/N} \neq 0, \qquad (q=0,1,\ldots,N-1),}
drawing the conclusion that the global centre symmetry is broken at
high temperatures, corresponding to a deconfined phase, with the $N$
degenerate vacua being
labelled by the $N$ possible distinct expectation values of
$L$, $<L>=e^{2\pi iq/N}L_0$. This spontaneous breaking of the discrete
global centre symmetry ($<\!L\!> \neq 0 \Rightarrow F_q$ finite)
will lead\ref\IRvi{B.~Svetitsky, \PRep{132}{1986}{1}} to a correlator
\eqn\IEix
{\Gamma(\vx) \sim |\!<\!L\!>\!|^2 (1+{\beta_T} e^2
e^{-\mu |\vx|} / |\vx|^p),}
giving a short-range static
potential $F_{q \bar q} \sim -e^2 e^{-\mu |\vx|} / |\vx|^p$: the
Debye screening of an electric plasma.

The point to emphasise
is that $<L(\vx)>$ is acting as an order parameter for the centre
symmetry, distinguishing between broken and unbroken phases, and
between the different broken phases. This has been seen
perturbatively\ref\IRviioa{N.~Weiss,
\PR{D24}{1981}{475}}\ref\IRx{T.~Bhattacharya, A.~Gocksch, C.P.~Korthals~Altes
and R.~D.~Pisarski, \NP{B383}{1992}{497}} and by simulation\IRv.

It should also be noted, from \IEx, that this high-$T$ behaviour of a
theory in $d$
dimensions, with bare coupling $g^2$, is equivalent to that of a $T=0$
theory (where the electric
field component of the action will also vanish) in ($d-1$) dimensions
(because of the static configurations) with
effective coupling $g^2 T$. This effective
coupling will become infinitely strong as $T \rightarrow \infty$,
leading to strong-coupling behaviour. Thus, the Wilson loops mentioned
in the next chapter show confining behaviour at all temperatures, and
do not provide a valid test for confinement.

\subsec{The Background Field Method}
When we move beyond the classical level and seek to include quantum
corrections, the manifest gauge invariance of a gauge field theory is
usually broken by the gauge-fixing procedure. The ``background
field''\ref\IRviia{B.~DeWitt,
\PR{162}{1967}{1195}}\ref\IRviii{L.~F.~Abbott, \NP{B185}{1981}{189}}
quantises the field theory in the presence of a background field whose
transformation properties are chosen to restore certain symmetries of
the generating functional, and we shall rely on this method in the
next chapter.

The procedure is to write the gauge field from the
classical action as $A^\mu = A_B^\mu + a^\mu$, where $
A_B^\mu$ is the background field and $a^\mu$ the quantum field over
which the functional integral is taken. The ``background field
gauge'' is then used, breaking the gauge invariance of $a^\mu$, but
retaining that of $A_B^\mu$. External sources are coupled only to
$a^\mu$, thus allowing quantum calculations without losing explicit
gauge invariance.

First, conventional quantisation: adding a source $J$ in the
conventional fashion to the expression for the
generating functional in \IEia, and writing $x=(\tau,\vx)$ so that
$d^dx\equiv d\tau d\vx\equiv d\tau d^{d-1}x$, we have
\eqn\IExii
{Z[J]=\int_{\rm periodic}{\hskip-2em\relax}\CD A^\mu_a
\det\bigg ({\del \CF^c(A)\over\del\alpha^d}\bigg )\ e^{\int d^{d}x\ (\CL(A) -
\frac{1}{2\xi}(\CF_a(A))^2 - J_\mu^a A^\mu_a)}.}
Here, $$\CL(A)=-\frac{1}{4}F_{\mu\nu}^a F^{\mu\nu}_a
\qquad\hbox{and}\qquad \CF_a(A)=\del_\mu A_a^\mu
\qquad\hbox{(covariant gauge)},$$
and $({\del \CF^c(A)\over\del\alpha^d})$ is the derivative
under the infinitesimal transformation
\eqn\IExiia
{\delta A^\mu(x)=-D^\mu \alpha(x),}
where we define covariant derivatives for the standard and background fields
as
\eqn\IExiib
{D^\mu=\del^\mu -ig [A^\mu,\ \ ] \qquad\hbox{and}\qquad
D_B^\mu=\del^\mu -ig [A_B^\mu,\ \ ].}
The functional
derivatives of $Z[J]$ with respect to $J$ are the disconnected Green's
functions of the theory, with the connected functions generated by
$W[J]=\ln Z[J]$. We define the effective action by the Legendre
transformation $$\Gamma[\bar A]=W[J]-\int d^{d}x\ J^\mu_a \bar A_\mu^a,
\qquad\hbox{where}\qquad \bar A_\mu^a=\frac{\delta W}{\delta
J^\mu_a},$$ and generate the one-particle-irreducible Green's
functions by taking derivatives of the effective action with respect
to $\bar A$.

Now, the background field: we define $\tilde Z, \tilde W$ and
$\tilde\Gamma$ by analogy with $Z, W$ and $\Gamma$:
\eqn\IExiii
{Z[J,A_B]=\int_{\rm periodic}{\hskip-2em\relax}\CD a^\mu_a
\det\bigg ({\del \CF^c(a,A_B)\over\del\alpha^d}\bigg )\ e^{\int
d^{d}x\ (\CL(A_B+a) - \frac{1}{2\xi}(\CF_a(a,A_B))^2 - J_\mu^a a^\mu_a)},}
$$\tilde W[J,A_B]=\ln\tilde Z[J,A_B], \qquad \tilde\Gamma[\tilde
a,A_B]=\tilde W[J,A_B]-\int d^{d}x\ J^\mu_a \tilde a^a_\mu,
\qquad \tilde a^a_\mu=\frac{\delta\tilde W}{\delta
J^\mu_a}.$$
The single transformation of $A$ in \IExiia\ now corresponds to
connected transformations of $A_B$ and $a$. Invariance of the action
under \IExiia\ implies invariance under ``quantum'' transformations,
where $\delta A^\mu_B=0$, and ``background'' transformations, where
$\delta A^\mu_B=-D^\mu_B \alpha(x)$, with $\delta a^\mu$ being
chosen to give \IExiia\ in each case. To maintain explicit gauge
invariance of the action with respect to the background
transformations, we choose $\CF_a(a,A_B)$ to transform covariantly under
them, for example
\eqn\IExiiia
{\CF_a(a, A_B)=(D^\mu_B a_\mu)_a.}
Now, $({\del
\CF^c(a,A_B)\over\del\alpha^d})$ is the derivative under the quantum
transformations, for which $\delta a^\mu=-D^\mu \alpha(x)$, so a
consideration of $\CF_a(a + \delta a, A_B)$ reveals that
\eqn\IExiiib
{{\del \CF^c(a,A_B)\over\del\alpha^d}=-(D^\mu_BD_\mu)^c_d.}

By changing variables $a\rightarrow a-A_B$ in \IExiii, we
find the connection between $\tilde\Gamma$ and $\Gamma$:
$$\tilde\Gamma[\tilde a,A_B]=\Gamma[\tilde a+A_B]
\qquad\Rightarrow\qquad \tilde\Gamma[0,A_B]=\Gamma[A_B]$$
The latter is invariant under the background transformation 
$\delta A^\mu_B=-D^\mu_B \alpha(x)$, so is a gauge-invariant
functional of $A^\mu_B$.

We can now use \IExiiia\ and \IExiiib\ to rewrite \IExiii, introducing
complex Grassmann ghost fields $\eta$ in a relation of the form
$$\det\bigg ({\del \CF^c(a,A_B)\over\del\alpha^d}\bigg ) \sim
\int\CD\eta\CD\bar\eta\ e^{\int d^{d}x\ d^{d}y\ \bar\eta_c(x) ({\del
\CF^c(x)(a,A_B)\over\del\alpha^d(y)}) \eta^d(y)},$$
so that
\eqn\IExiiic
{Z[J,A_B]=\int_{\rm periodic}{\hskip-2em\relax}\CD a^\mu_a
\CD\eta\CD\bar\eta\ e^{\int
d^{d}x\ (\CL(A_B+a) - \frac{1}{2\xi}(D^\mu_B a_\mu)^2 +
\bar\eta(-D^\mu_B D_\mu)\eta - J_\mu^a a^\mu_a)}.}

\vfill\supereject


==> intro2.tex <==
\newsec{Predictions for Z(3) Interfaces}{in SU(3) Gauge Theory}

\Subsec{The Z(N) Interface}
In the deconfined phase, where the $Z(N)$ symmetry has been spontaneously
broken, we have seen that the system can exist in any one of $N$
degenerate vacua. It is possible to arrange boundary conditions
of the system so that different parts of it exist in different
vacua, {\it i.e.} different $Z(N)$ phases. The existence of these
distinct domains forces the appearance of ``domain walls'', or ``$Z(N)$
interfaces'', where they meet\ref\IRix{T.~Bhattacharya, A.~Gocksch,
C.~Korthals~Altes and R.~D.~Pisarski, \PRL{66}{1991}{998}}\IRx.
Within these interfaces, the gauge
fields interpolate between the different vacua, as does the
expectation value of the Polyakov line.

The calculation of the interface tension is clearly an instanton
problem: the field is interpolating from one $Z(3)$ vacuum to
another. An effective one-dimensional theory will describe the
interface profile. The instanton is the solution of the classical
equations of motion, with action $\sim 1/g^2$ as in \IEixa, and so we
might na\"{\i}vely expect the interface tension to have the same
behaviour. To test this guess, we can
construct an effective action from the classical piece, acting as a
kinetic term, and a quantum piece, a potential term formed by
integrating out fluctuations to one-loop order. The $Z(N)$ instanton is
the stationary point of this total action.

\ifig\IFi{A system of finite extent, with two space and one Euclidean
time dimensions.}
{\epsfxsize\hsize \epsfbox{systemsize.eps}}

In a case which will be relevant for future chapters, consider
a system of finite extent at a temperature $T$, as illustrated in \IFi. 
The Euclidean time dimension runs from $0$ to ${\beta_T}=1/T$, and let
us suppose there are two space dimensions,
one ($z$) much longer than the other ($x$), and both much longer than
the time dimension:
$L_z \gg L_x \gg {\beta_T}$. We assume that the system is in one $Z(N)$
phase at the $z=0$ end of the longitudinal dimension and another at
the $z=L_z$ end, forcing the appearance of a $Z(N)$ interface
somewhere along the $z$
direction. Where the Polyakov line was previously parametrised by the
discrete values $q=0,1,\ldots,N-1$ in \IExi, we shall now make $q$ a
continuous function of longitudinal position: $q \rightarrow q(z)$.

As we have seen, the order parameter for the $Z(N)$
symmetry is the Polyakov line, given in the fundamental representation
 by \IEvia, where the gauge coupling is now written explicitly:
\eqn\IExiv
{L(z)=\frac{1}{N}\Tr\CT e^{ig\int^{\beta_T}_0 A^0(z) d\tau}.}
We assume that the gauge fields obey strictly periodic boundary
conditions. Since the time direction is finite, states with constant
$A^0$ are inequivalent. Whilst we could work in a gauge with $A^0$ set
to zero at zero temperature, the periodic boundary conditions in the
time direction make this impossible for $T \neq 0$: were we to set
$A^0=0$ by a gauge transformation of the functional integral, 
the $A^i$ would violate the boundary conditions.
Therefore, following the method outlined in \IRix\IRx, we
choose to make a global colour rotation so that $A^\mu=(A^0,{\bf 0})$, with
$A^0$ a time-independent, diagonal $N\times N$ matrix:
\eqn\IExv
{A^0(z)=\frac{2\pi
Tq(z)}{gN}\left(\matrix{{\hbox{\tenmsbm I}_{N-1}}&{\bf 0}\cr{\bf
0}&{-(N-1)}\cr}\right) \equiv \frac{2\pi
Tq(z)}{gN}\left(\matrix{1&&&\cr&\ddots&&\cr&&1&\cr&&&{-(N-1)}\cr}\right).}
In the presence of this $A^0$ field, the Polyakov line is given by
$$L(z)=e^{2\pi iq(z)/N}\bigg (1-\frac{1}{N}[1-e^{-2\pi iq(z)}]\bigg
).$$ One can now understand the $Z(N)$ structure of the vacuum: the
$N$ degenerate vacua occur for $q(z)=0,1,\ldots,N-1$, corresponding to
$L(z)=e^{2\pi iq(z)/N}$. The ordinary perturbative vacuum has
$A^0=q(z)=0$, with $L(z)=1$. It has been shown\IRx\ that the path taken by
a gauge field when interpolating between different vacua has minimal
action for this form of $A^0(z)$, as desired.

Returning to the generating functional in \IExiiic, without
source term, and extracting the dimensionless coupling explicitly again,
the Euclidean action is given by
$$\CS_E=\int d\tau d^dx \bigg (\frac{1}{2g^2}\Tr F^2_{\mu\nu} -
\frac{1}{2\xi}(D^\mu_B a_\mu)^2 + \bar\eta(-D^\mu_B D_\mu)\eta \bigg ).$$
The first term is the (classical) kinetic part, and the second and
third terms form a potential, $V$.

For the $A^\mu\equiv A^0(z)$ field of \IExv, with transverse
space dimensions of volume $V_{trans}$, the kinetic part reduces to
$$\frac{{\beta_T}
V_{trans}}{g^2}\int \Tr (\del_z A^0(z))^2 dz = \frac{4\pi^2 T
V_{trans}(N-1)}{g^2 N} \int \bigg (\frac{dq}{dz}\bigg )^2 dz.$$

Classically, there is no potential for $A^0$, and all values of $A^0
\neq 0$ are degenerate.
However, by computing one-loop quantum
effects about the background field
\eqn\IExva
{A_B^\mu=(A^0,{\bf 0}), \qquad\hbox{where $A^0$ is as given in
\IExv,}}
we shall see that the degeneracy is broken. We treat the background
$A^0$ field as constant in $z$, justifying this later.
Expanding $V$ to quadratic order in the quantum fluctuations
$a^\mu$, we can then integrate out both these gauge fields
and the ghost fields, to give (to one-loop order):

$$V=\bigg \{\underbrace{\half\Tr\ln\bigg
[-(D_B)^2\delta_{\mu\nu} + \bigg (1-\frac{1}{\xi}\bigg )D_B^\mu
D_B^\nu\bigg ]}_{\rm from\ gauge\ fields} - \underbrace{\Tr\ln\bigg
(-(D_B)^2\bigg )}_{\rm from\ ghost\ fields} \bigg \}.$$
The potential is independent of $\xi$,
so we use the Feynman gauge, $\xi=1$, in our $d$
dimensions, to reduce the previous expression to $$V=\bigg
(\frac{d}{2}-1\bigg )\Tr\ln(-(D_B)^2).$$

Now, each matrix function $a(x)$ on which $D^\mu_B$ acts can be
written as a product of a scalar function of space-time with a
vector in an $(N^2-1)$-dimensional matrix space, where the basis
matrices are the $(N^2-1)$ generators of $SU(N)$. To find
$\Tr\ln(-(D_B)^2)$, we should diagonalise $D_B$ in function space and
then sum over its eigenvalues. A suitable basis is given by the plane
waves $e_p(x)=e^{ip_\mu x^\mu}$, with
4-momentum $p_\mu=(p_0,\bf 
p)$; the coordinates of $a(x)$ are its Fourier components $\tilde
a(p)$, and the action of $D_B$ on these comes from \IExiib:
$$D_B^\mu a(x)=\del^\mu a(x)-ig[A^\mu_B,a(x)] \qquad\Rightarrow\qquad
D^B_\mu \tilde a(p)=ip_\mu \tilde a(p)-ig[A^\mu_B,\tilde a(p)].$$
Our choice of $A_B^\mu$ earlier in \IExva\ eases the eigenvalue
calculation. For the space components, the eigenvalues of $-(D_B^i)^2$
are simply $(p^i)^2$. For the time component, the periodic boundary
conditions force $p_0=2\pi n_0/{\beta_T}=2\pi n_0T$ for integer $n_0$.
A suitable set of $SU(N)$ generators enables the eigenvalues of
$-(D_B^0)^2$ to be calculated rapidly; for instance, we can split the
$(N^2-1)$ generators into $(N-1)$ diagonal generators similar to
\IExv,
$$T_i\sim
\left(\matrix{{\hbox{\tenmsbm I}_{i-1}}&&\cr&-(N-2)&\cr&&{\hbox{\tenmsbm
I}_{N-i}}\cr}\right),\qquad(i=1,\ldots,N-1),$$
and $(N-1)!$ pairs of off-diagonal ladder
generators\ref\IRixa{V.~M.~Belyaev and V.~L.~Eletsky, \ZP{C45}{1990}{355}},
$T^\pm_{i,j}$, with all elements zero except for one, whose value is
common to the pair, at the $j$th row and $i$th column of $T^+_{i,j}$ and the
$i$th row and $j$th column of $T^-_{i,j}$ ($i=2,\ldots,N$ and
$j=1,\ldots,i-1$). When these generators are commuted with $A^0_B$,
as given by \IExva, it should be apparent that only the $(N-1)$ pairs
of generators $T^\pm_{N,j}$ will give a non-zero commutation bracket
(proportional to $\pm T^\pm_{N,j}$ respectively), with the other
$(N-2)!=\half(N-2)(N-1)$ off-diagonal pairs and $(N-1)$ diagonal
generators commuting with $A^0_B$. Thus, the eigenvalues
of $-(D_B^0)^2$ are seen to be:
$$
\eqalign{
[2\pi T(n_0\pm q)]^2&\qquad:\qquad\hbox{$(N-1)$ copies of each
(charged generators);}\cr
[2\pi Tn_0]^2&\qquad:\qquad\hbox{$(N-1)^2$ copies
(neutral generators).}}$$
The part of the trace over space-time now simply gives the
total space-time volume, $V_{tot}=\beta_T L_z V_{trans}$; however, this is
conventionally omitted from the ``potential'', so we shall ignore it
until we insert $V(q)$ into the action. Hence, putting
$V(q)=\CV(q)-\CV(0)$ so that $V(0)=0$,
$$
\eqalign{
\CV(q)=(N-1)(\tfrac{d}{2}-1)&\ T\sum_{n_0}\int\frac{d^{d-1}{\bf
p}}{(2\pi)^{d-1}}\bigg \{(N-1)\ln((2\pi Tn_0)^2 + {\bf p}^2)\cr +
&\ln((2\pi
T(n_0-q))^2 + {\bf p}^2) + \ln((2\pi T(n_0+q))^2 + {\bf p}^2)
\bigg \}.\cr}$$
Note that for finite temperatures, we
have replaced the integral over $p_0$ with a discrete sum:$$\int
\frac{d^dp}{(2\pi)^d} \rightarrow
T\sum_{n_0}\int\frac{d^{d-1}{\bf p}}{(2\pi)^{d-1}}.$$
Since $n_0$ and ${\bf p}$ run over all negative and positive
values, the $(n_0\pm q)$ terms give the same contribution, and the
subtraction of $\CV(0)$ yields
$$V(q)=2(N-1)(\tfrac{d}{2}-1)\ T
\sum_{n_0}\int\frac{d^{d-1}{\bf p}}{(2\pi)^{d-1}}[\ln((2\pi T(n_0+q))^2 +
{\bf p}^2)-\ln((2\pi Tn_0)^2 + {\bf p}^2)].$$
Now, we can use the following two integral formulae
to make progress:
$$\int_0^\infty \frac{e^{-ax}-e^{-bx}}{x}dx = \ln b - \ln a
\qquad\hbox{and}\qquad\int_{-\infty}^\infty
e^{-ax^2}=\sqrt\frac{\pi}{a}.$$ The first enables us to rewrite $V(q)$ as
$$V(q)=2(N-1)(\tfrac{d}{2}-1)\ T
\sum_{n_0}\int\frac{d^{d-1}{\bf p}}{(2\pi)^{d-1}}\int_0^\infty \frac{dt}{t}
e^{-t{\bf p}^2}[e^{(2\pi Tn_0)^2t}-e^{(2\pi T(n_0+q))^2t}],$$ before the
second gives the result of Gaussian integration over ${\bf p}$:
$$V(q)=2(N-1)(\tfrac{d}{2}-1)\ T
\sum_{n_0}\int_0^\infty \frac{dt}{t}\frac{1}{(4\pi t)^{d/2}}
[e^{(2\pi Tn_0)^2t}-e^{(2\pi T(n_0+q))^2t}].$$
A combination of the Poisson summation formula
and a standard exponential integral
leads to a useful relation:
$$\int^\infty_{-\infty}e^{-(ax^2+bx+c)}dx=\sqrt\tfrac{\pi}{a}
e^{(b^2-4ac)/4a}\quad\hbox{and}\quad
\sum^\infty_{n=-\infty}F(n)=\sum^\infty_{r=-\infty}
\bigg\{\int^\infty_{-\infty}e^{2\pi irx}F(x)dx
\bigg\}$$
$$
\Rightarrow\qquad
\sum_n e^{-a(n+b)^2} = \sum_r \sqrt\frac{\pi}{a}\ e^{-\pi(r^2/a)-2\pi
ibr}.$$
Along with a change of variable to $\hat t=4\pi T^2 t$, this leads to
$$V(q)=2(N-1)(\tfrac{d}{2}-1)\
T^{d}\sum_{r=-\infty}^\infty\int_0^\infty \frac{d\hat t}{\hat
t}{\hat t^{-d/2}}
e^{-\pi r^2/{\hat t}}(1-e^{2\pi irq}).$$
A change of variables $\hat t \rightarrow u=1/\hat t$, followed by
exponential integration over $u$,
gives the final result:
\eqn\IExvi
{V(q)=4(N-1)(\tfrac{d}{2}-1)T^{d} 
\frac{\Gamma(\tfrac{d}{2})}{\pi^{d/2}} B_{d}(q),}
where, re-expressing the sum over all $r$ as a sum over positive $r$,
$$B_{d}(q)=\sum_{r=1}^\infty \frac{1}{r^{d}}[1-\cos(2\pi rq)].$$

\ifig\IFii{The effective potential, with temperature dependence
factored out, for $d=3$ and $N=3$. This quantity is equal to
$2B_3(q)/\pi$. The solid line is the continuum version given here; the
dotted one is the lattice version for $N_t=2$, as calculated in
section 2.3.}{\epsfxsize\hsize \epsfbox{potential.ps}}

For $SU(3)$ theory in $2+1$ dimensions, $V(q)$ is illustrated in \IFii.
The potential is clearly periodic: $V(q) \equiv V(q \bmod 1)$. 
The effective potential is minimised, as mentioned before, when $q$
takes an integer value, {\it i.e.} it vanishes when $<L> \in Z(N)$,
and $<L>$ is indeed an order parameter for the $N$ degenerate vacua.

It should be noted in passing that this picture changes with the
addition of fermions, as mentioned in section 1.3. This is because a gauge
transformation of the form \IEvii\ causes the fermion wavefunction to
transform simply as $\psi\rightarrow U\psi$. Thus, whereas the gauge
fields are invariant under a $Z(N)$ transformation, the fermion
wavefunctions are generally not: $\psi\rightarrow e^{2\pi
iq/N}\psi$. This means that the boundary conditions, which should be periodic
for the gauge fields and anti-periodic for the fermions, actually
correspond to ``twisted'' conditions for the fermions:
$\psi(\beta_T)=e^{-2\pi iq/N}\psi(0)$. Thus, the $Z(N)$ symmetry is
lost, and the structure of \IFii\ changes\IRoba, with the central maximum
and minima rising as fermion families are added but the
outer maxima and $q=0$ minimum falling, the latter becoming the true
vacuum. For $N=3$ and four or more fermion families, the metastable
minima at $q=1$ and $q=2$ actually correspond to {\it positive} free
energy density of the form mentioned in section 1.3, and the peculiar
thermodynamic properties discussed there set in.

We now have an expression for the effective action in $q$, remembering
to integrate $V(q(z))$ over the total space-time volume, $V_{tot}
\rightarrow \beta_T V_{trans} \int dz$, and using
${\beta_T}=1/T$:
$$\CS_{eff}(q)=V_{trans} T \int dz \bigg \{\frac{4\pi^2(N-1)}{g^2 N}\bigg
(\frac{dq}{dz} \bigg )^2 + 4T^{d-2}(N-1) (\tfrac{d}{2}-1)
\frac{\Gamma(\tfrac{d}{2})}{\pi^{d/2}}B_{d}(q)\bigg \}.$$

For $d=3$, we convert to the dimensionless variable $z'\equiv \sqrt{NT}
gz$\ :
$$\CS_{eff}=L_x\frac{T^{1.5}}{g}\frac{4\pi^2(N-1)}{\sqrt N}\int dz' \bigg
\{ \bigg (\frac{dq}{dz'} \bigg )^2 + \frac{B_3(q)}{4\pi^3} \bigg \}.$$
Treating the integrand as a standard 
Lagrangian with ``time'' $z'$, we know that the equivalent Hamiltonian
(the energy, $\CE=(\frac{dq}{dz'})^2-\frac{B_3(q)}{4\pi^3}$) is
a constant of the 
motion. In the simplest case, we set $q=0$ at one end of the system
and $q=1$ at the other, with $\frac{dq}{dz'}=0$ at both. With these boundary
conditions, the instanton has $\CE=0$, so
$$\eqalign{
\CS_{eff}&=L_x\frac{T^{1.5}}{g}\frac{4\pi^2(N-1)}{\sqrt N}\int dz' \bigg
\{ \bigg (\frac{dq}{dz'} - \sqrt{\frac{B_3(q)}{4\pi^3}} \bigg )^2 +
\bigg (\frac{dq}{dz'} \bigg )\frac{\sqrt{B_3(q)}}{\pi^{3/2}} \bigg \}\cr
&=L_x\frac{T^{1.5}}{g}\frac{4\pi^{1/2}(N-1)}{\sqrt N}\int
dq\sqrt{B_3(q)}.\cr}$$

The interface tension, $\alpha$, is defined to be the effective action
per unit area of the interface:$$\CS_{eff}={\beta_T}
L_x\alpha.$$
This gives a prediction for the surface tension of
\eqnmulti\IExvia
{\alpha&=\frac{T^{2.5}}{g}\frac{4\pi^{1/2}(N-1)}{\sqrt N}\int
dq\sqrt{B_3(q)}} 
{&=\alpha_0\frac{T^{2.5}}{g},}
as the integral is just a number, 1.018.
Evaluating \IExvi\ for $d=3$, we see that $V(q)/T^3=(N-1) B_3(q)/\pi$,
so, in a result that we shall use again later,
\eqn\IExvib
{\alpha_0=4\pi\sqrt\frac{N-1}{N}\int dq\sqrt{V(q)/T^3}.}
For the $SU(3)$ system we shall go on to consider, this means that
\eqn\IExvii
{\alpha_0=8.33.}

It only remains to justify our original assumption that $q$ could be
treated as independent of $z$. In fact, the instanton must have width
of order $1$ in terms of the dimensionless coordinate $z'$, as there
is no length scale, and this corresponds to 
$1/g\sqrt T$ in terms of $z$. For weak coupling, this is
much larger than the natural length scale of the system,
$1/T$. Thus, the instanton field varies slowly enough in $z$ that it
can be treated as constant to leading order.

\subsec{Lattice Formalism}
Although some of the above properties can be examined in the
continuum, many calculations are performed on the
lattice\ref\IRxi{J.~B.~Kogut, \RMP{55}{1983}{775}}\ref\IRxii{Michael
Creutz (ed.), {\it ``Quantum Fields on the Computer''}, World
Scientific, Singapore (1992)}.
The advantage of this approach is that the short-distance cut-off
enters the definition of the field theory in a natural way, allowing
non-perturbative calculations to be made. In particular, lattice
theories lend themselves to strong-coupling expansions and Monte-Carlo
simulations, allowing the statistical evaluation of path integrals to
a specified accuracy. In particular, the confining and non-confining
behaviour of quarks can be seen in the lattice formalism, together
with the transition between these two regimes. Using
numerical simulations on the lattice, one can also approach the
continuum limit and compare results with analytic predictions.

\ifig\IFiii{The Euclidean lattice in two space and one time (``2+1'')
dimensions. Link variables, $U$, on the lattice are
illustrated by bold arrows, as indicated by the example to the top
left. A plaquette and a Polyakov line are shown; the Polyakov line
wraps around the boundary condition in the time direction, but this is
not shown.}{\epsfxsize\hsize \epsfbox{latticeplaq.eps}}

In the Euclidean formalism, one considers a hypercubic lattice whose sites are
separated by lattice spacing $a$. This is the only quantity on the
lattice which has dimension, and acts as an ultraviolet cut-off for
the theory on the lattice.
If we specify $N_t$ links
in the time direction, this corresponds to a temperature
\eqn\IExviii
{T=1/\beta_T=1/N_t a.}
Similarly, we have $N_z$ links in the longitudinal direction and $N_x$
in the transverse, so
$$L_z=N_z a\qquad\hbox{and}\qquad L_x=N_x a.$$
For some gauge group $\CG$, we can define a gauge field
\eqn\IExviiia
{U_n^\mu=e^{ia{\bf T}\cdot{\bf A}_{n\mu}} \in \CG,}
residing on the link leaving site $n$ in
direction $\mu$. The exponential of the field strength,
$e^{iF_{\mu\nu}}$, is now equivalent to the product of fields around a
plaquette (four connected links forming the smallest possible square,
as illustrated in \IFiii):
\eqn\IExviiiaa
{U^{\mu\nu}_n = U^\mu_n U^\nu_{n+\hat\mu} U^{\mu\dagger}_{n+\hat\nu} 
U^{\nu\dagger}_n.}
The usual procedure is now
to consider the Wilson action, which only depends on plaquette
variables ($N$ is the order of symmetry, as in section 1.5):
\eqn\IExviiib
{S_W = {2N\over g^2} 
\sum_{n\atop{\mu > \nu}} (1 - {\textstyle{1\over N}}\Real\Tr U^{\mu\nu}_n).}
The conventional bare (dimensionless) coupling, $g$, is related to the lattice
parameter $\beta$ by
\eqn\IExix
{\beta = 2N/a^{4-d}g^2}
in $d$ dimensions. For our future purposes, $d=3$ and $N=3$, so that
$\beta=6/ag^2$.

This action is, naturally, invariant under local gauge transformations,
$U^\mu_n \rightarrow V_nU^\mu_nV^\dagger_{n+\hat\mu}$, for
$V_n\in\CG$, as well as the global centre symmetry discussed in
section 1.7.
Using the gauge fields on the links, we can define ``Wilson loops'',
gauge-invariant observables given by the trace of an ordered product
around a closed curve $C$:
\eqn\IExixa
{W[C] = \Tr\prod_{n\mu \in C} U^\mu_n.}
These topologically trivial quantities are not aware of the centre
symmetry and $Z(3)$ phases.

Owing to the periodicity of the lattice in time, topologically
non-trivial loops also exist, winding around the lattice one or more
times; these cannot be shrunk to a point. The 
Polyakov line is one such, defined, as in \IExiv\ for the continuum, by
considering a path parallel to the
time axis at some spatial location $\vx$:
\eqn\IExixb
{L(\vx) = \Tr\prod^{N_t}_{n=1} U^0_{\vx + n\hat t}.}
An example of a Polyakov line is shown in \IFiii. Many of these non-trivial
quantities {\it are} aware of the $Z(3)$ phase structure, as we saw
for the Polyakov line in section 1.7. 

\subsec{The Lattice Surface Tension}
Since we shall be examining the properties of an interface in $SU(3)$
theory in $2+1$ dimensions, with $N_t=2$, it behoves us to repeat the
procedure giving the interface tension, this time on the lattice. This simply
involves replacing continuum quantities in the calculation with their
lattice equivalents, following \ref\IRxiia{C.~P.~Korthals~Altes,
A.~Michels, M.~Stephanov and M.~Teper, OUTP-96-10P}.

If we consider the space dimensions to be essentially infinite,
taking only the time dimension to be small, then the continuum momenta
are restricted as follows on the lattice:
$$\eqalign{
p_i &\rightarrow \frac{2}{a}\sin\bigg ({\frac{p_i a}{2}}\bigg ),\qquad
-\frac{\pi}{a} < p_i < \frac{\pi}{a};\cr
p_0 &\rightarrow \frac{2}{a}\sin\bigg ({\frac{p_0 a}{2}}\bigg ),\qquad
p_0=2\pi n_0T,\ 2\pi (n_0\pm q)T,\qquad n_0=0,1,\ldots,N_t-1.}$$
The techniques used are largely the same as for the continuum calculation,
but we leave the integration over the momenta until last,
as the restriction is now $-\pi<p_\mu<\pi$ (setting $a$=1 for
convenience) rather than $-\infty<p_\mu<\infty$. These integrals over
momenta give modified Bessel functions:
\eqn\IExixc{
I_n(t)=\frac{1}{2\pi}\int^\pi_{-\pi} dk\ e^{t\cos k + ink}}

The effective potential on the lattice is finally written
(C.F. \IExvi) as:
\eqn\IExx
{V_{lat}(q)=4(N-1)(\tfrac{d}{2}-1)\sum_{r=1}^\infty (1-\cos(2\pi
rq))F(rN_t,d),}
where the newly introduced function $F$ is defined in terms of the
modified Bessel functions, $I_n$:
$$F(n,d)=\int_0^\infty \frac{dt}{t} e^{-dt} I_n(t) [I_0(t)]^{d-1}.$$
For $d=3$ and $N_t=2$, the values of $F(2r,3)$ are given in Appendix
A.
For these values, the lattice quantity, $V_{lat}(q) N_t^{d}$, is plotted
in \IFii\ alongside the continuum version, $V(q)/T^{d}$.
The lattice expression for the surface tension is given by \IExvib:
$$\alpha_0=4\pi\sqrt\frac{N-1}{N}\int_0^1 dq
\sqrt{V_{lat}(q) N_t^3}.$$
For $N_t=2$ and $N=3$, this gives the prediction (C.F. \IExvii) that
\eqn\IExxi
{\alpha_0=9.82.}

To check that the correct continuum limit is recovered as
$N_t\rightarrow\infty$, we need to find 
the behaviour of $F(n,d)$ as $n\rightarrow \infty$. We use the
method of steepest descent, which determines the asymptotic
($s\rightarrow\infty$) behaviour
for an integral of the form
$$\CI(s)=\int_\CC dz g(z) e^{sf(z)},$$
as follows:

\item{$\bullet$} Find the saddle point of $f(z)$, {\it i.e.} $z_0$
such that the first derivative, $f'(z_0)=0$;
\item{$\bullet$} Expand around this point using $z=z_0 + \delta
e^{i\alpha}$, and choose $\alpha$ so that $\Real\{f(z)\}$ is a maximum,
giving the path of steepest descent;
\item{$\bullet$} Substitute into the following formula, the
approximation sought for large $s$:

$$\CI(s)\approx\frac{\sqrt{2\pi} g(z_0) e^{sf(z_0)}
e^{i\alpha}}{|sf''(z_0)|^{1/2}}.$$
From \IExixc, we can write
$$ I_n(nt)=\frac{1}{2\pi}\int^\pi_{-\pi} dk\ e^{n(t\cos k + ik)},\qquad
I_0(nt)=\frac{1}{2\pi}\int^\pi_{-\pi} dk\ e^{n(t\cos k)}$$
The forms of $I_n(nt)$ and $I_0(nt)$ enable us to find saddle points
at $k=\cos^{-1}(\frac{\sqrt{t^2+1}}{t})$ and $k=0$ respectively,
and the steepest descent in each case is for $\alpha=0$, giving
$$I_n(nt)\approx\frac{e^{n[\sqrt{t^2+1}-\sinh^{-1}(1/t)]}}{\sqrt{2\pi
nt}(1+1/t^2)^{1/4}},\qquad I_0(nt)\approx\frac{e^{nt}}{\sqrt{2\pi
nt}}.$$
Substituting into our formula for $F(n,d)$,
$$\eqalign
{F(n,d)&=\int^\infty_0 \frac{d(nt)}{nt} e^{-dnt} I_n(nt)
[I_0(nt)]^{d-1}\cr
&=\int^\infty_0 \frac{dt}{t}\frac{e^{n[t(\sqrt{1+1/t^2}-1) -
\sinh^{-1}(1/t)]}}{(2\pi nt)^{d/2} (1+1/t^2)^{1/4}}}.$$
This exponent has its stationary point at $t=+\infty$, and, since the
dominant contribution to the integral will occur around this value of
$t$, we can replace the integrand by its approximate form as
$t\rightarrow+\infty$.
A final transformation of variable, $t\rightarrow u=1/t$, then reveals
that
$$F(n,d)=\int^\infty_0 du e^{-nu^2/2} \frac{u^{d/2-1}}{(2\pi
n)^{d/2}},$$
so, by the definition of the gamma function,
$$F(n,d)\rightarrow\frac{\Gamma(d/2)}{\pi^{d/2}n^d}
\qquad\hbox{as}\qquad n\rightarrow\infty,$$
as desired from a comparison of \IExvi\ with \IExx.

\subsec{The Debye Mass}
The electric (``Debye'') mass $m$, or inverse Debye screening length,
governs gauge-invariant correlation functions of the time-like
component of the gluon field ($A_0$) at large distances and high
temperatures. The free energy of a quark-antiquark
pair, over and above the sum of their separate free energies,
vanishes as the quarks become infinitely far apart:
$$F_{q\bar
q}(\vx)-2F_q=V(|\vx|,T)\mathrel{\mathop{\longrightarrow}\limits_{|\vx|
\rightarrow \infty}}0 \qquad\hbox{for\ } T>T_c.$$
From perturbation theory, we know that quarks are screened at a
distance of the order of the inverse electric mass, so rather than
being logarithmic in $\vx$, the interaction potential takes, in the
manner of \IEix, the form
$$V(|\vx|,T)\mathrel{\mathop{\sim}\limits_{|\vx|\rightarrow \infty}}
-Ce^{-2m|\vx|} \qquad\hbox{for\ } T>T_c.$$
The factor of two arises because gauge invariance leads to an exchange of
two gluons being the lowest-order contribution in perturbation theory.
The electric mass is one of the fundamental parameters of a gauge
theory at finite temperature. One can perform a
self-consistent and gauge-invariant calculation of its value, through
the subtracted correlation function
$$\ll L(0)L^\dagger(\vx)\gg\quad\equiv\quad<L(0)L^\dagger(\vx)> -
<L(0)><L^\dagger(\vx)>,$$ and the Feynman
diagrams contributing to this correlation function have
been calculated\ref\IRxiii{E.~D'Hoker,
\NP{B200[FS4]}{1982}{517}} \ref\IRxiv{E.~D'Hoker, \NP{B201}{1982}{401}},
with the dimensional regularisation mass scale set to $m$. We shall
quote the expression found for $m^2$ later in this section, but it may
be instructive beforehand to examine screening in a simple model: a
plasma of bosons, each with mass $m_g$ and charge $\pm
g$\ref\IRxivo{{\it Following} L.~D.~Landau and E.~M.~Lifschitz, {\it
``Statistical Physics''} (Part I, Ed. 3), \S 78: {\it ``Thermodynamic
Quantities for a Classical Plasma''}}.

A positive test charge inserted into the plasma will attract (repel)
negatively (positively) charged bosons, and the net induced charge
density will result in an electrostatic potential
$\phi(r)$. The energy of a given boson in the absence of the test charge,
$E=\sqrt{p^2+m_g^2}$, will change in its presence by $\pm g\phi$, so we
can write a consistent expression for this induced charge density using the
bosonic density of states:
\eqn\IExxia{
\rho\sim -\int d^{d-1}p \bigg ( \frac{g}{e^{\beta_T(E+g\phi)}-1} +
\frac{-g}{e^{\beta_T(E-g\phi)}-1} \bigg ).}
Far away from the test charge, $\phi(r\rightarrow\infty)\rightarrow
0$, and we can expand $e^{\beta_T g\phi}\approx 1+\beta g\phi$. Changing
variables so as to pull factors of $\beta_T$ out of the resulting
integral, we find that $\rho\sim -g^2 T^2 \phi$ for $d=4$. The
inclusion of the test charge in $\rho$ gives exponential screening
with this expression for the Debye mass:
\eqn\IExxib{
\phi\sim \frac{e^{-mr}}{r},\qquad m^2\sim g^2T^2.}

For $d=3$, we find that $\rho\sim -g^2 T\phi \ln\tfrac{T}{g\phi}$, and
$\phi$ shows Gaussian rather than exponential screening.
In fact, the effective one-loop potential for small $q$ shows the
following behaviour:
$$V_{eff}\sim q^2\ln q,$$
leading to a divergence in the Debye mass. However, the full loop
calculation mentioned earlier, treating the Debye mass
self-consistently, reveals that the logarithmic divergence is halted
at an infrared cut-off, resulting in the return of exponential
screening. In our simple plasma model, this can be seen by an
approximate evaluation of \IExxia\ for non-zero mass $m_g$, putting
$e^{\beta_T E}\approx 1 + \beta_T E$ for $m_g<E<\beta_T^{-1}$:
$$
\eqalign{
\rho&\sim -g^2\beta_T\phi\bigg ( \int_{m_g}^{\beta_T^{-1}} E dE
\frac{(1+\beta_T E)}{(\beta_T E)^2} + \int_{\beta_T^{-1}}^\infty E dE
\frac{e^{\beta_T E}}{(e^{\beta_T E}-1)^2} \bigg )\cr
&\sim -g^2T\phi\ln\bigg(\frac{T}{m_g}\bigg)\qquad\hbox{to leading order}.\cr}$$
This corresponds to the return of exponential screening:
$$\phi\sim\frac{e^{-mr}}{\sqrt r},\qquad m^2\sim g^2T\ln
\bigg(\frac{T}{m_g}\bigg).$$
The prediction of the full loop calculation\IRxiii\IRxiv\ mentioned
previously is that $$V_{eff}\sim q^2m^2,$$ with a self-consistent solution
for the Debye mass:
\eqn\IExxii
{m^2=\frac{g^2NT}{4\pi}\ln(T/g^2)\quad+\quad O\bigg[g^2T\ln(\ln(T/g^2))\bigg].}
Clearly, this mass is a non-analytic function of coupling
constant and temperature. This formula is only strictly applicable for
$T/g^2\gg 1$.

\ifig\IFiv{The predicted lowest-order behaviour of the Debye mass, $m$.}
{\epsfxsize\hsize \epsfbox{masspredict.ps}}
The prediction for $m$ is shown in \IFiv. In terms of the lattice
parameter, \IExxii\ becomes 
\eqn\IExxiv
{\frac{m^2}{g^2T}=\frac{3}{4\pi}\ln(\beta/12) +
O\bigg[\ln(\ln(\beta/12))\bigg].}

Since the one-loop $V(q)\sim q^2\ln(1/q)$ rather than $q^2$ for small
$q$, we are
not able to extract an expression for the Debye mass from $\frac{\del^2
V_{lat}(q)}{\del q^2}\big |_{q=0}.$

\subsec{The Deconfinement Transition}
We can re-express the $d$-dimensional functional integral over
gauge fields, seen in section
1.6, in terms of the Polyakov line, $L$, by inserting a delta function
conforming to \IExiv, and
so construct an effective action in terms of $L$ \IRvi:
$$e^{-S_{eff}[L]} = \int \CD A_\mu e^{-S[A_\mu]} \prod_\vx \delta \bigg(
L(x) - \Tr \CT e^{i\int dt A_0(\vx,t)} \bigg).$$
Integrating out the space-like gauge fields, $A^i$, their
correlation length, $\xi$, sets the range of a set of coupling- and
temperature-dependent kernels, $S_2,
S_4, \ldots$, in
$$
\eqalign{
S_{eff}[L]=\int d\vx\ V(L(\vx))\ &+ \int d\vx\ d\vy\
L^\dagger(\vx)S_2(\vx-\vy)L(\vy)\cr &+ \int d\vx\ d\vy\ d{\bf z}\ d{\bf
w}\ L^\dagger(\vx)L^\dagger(\vy)S_4(\vx,\vy,{\bf z},{\bf w})L(z)L(w)\
+ \ldots.}$$
It can be shown\IRvi\ that $\xi$ is finite at low {\it and} high
temperatures, with space-like Wilson loops at both showing an area-law
behaviour. Assuming that this will also hold at the phase transition
itself, the kernels should be short-ranged.

The deconfinement-confinement transition now appears as a $(d-1)$-dimensional
order-disorder transition in statistical mechanics, the time dimension
having gone. Integrating
out the short-range interactions up to length $\xi$
leaves a simple Landau-Ginzburg effective action:$$S_{eff} =
\int dx \bigg( (\del_i L )^2 + V(L) \bigg).$$
$S_{eff}$ retains the invariance under the centre symmetry $L
\rightarrow zL$, so that the potential $V(L)$ must do the
same. However, we know 
little else about $V(L)$, so we need to study it in mean-field theory
(MFT), or by Monte
Carlo simulation, to find out details of the order of the phase
transition, as seen in \ref\IRxiva{M.~Gross and J.~F.~Wheater,
\NP{B240}{1984}{253}} for the strong-coupling limit.

In MFT we neglect fluctuations, so the equilibrium state of the system
is represented by the absolute minimum of $V$. If the minimum is at
$L=0$, we have the symmetric phase; at the transition, the 
transition is shown to be second order by the minimum moving away from zero
smoothly, and first by it moving discontinuously.
If the transition is continuous, renormalisation group (RG) theory
tells us that an RG fixed point will govern the critical behaviour.
Whole ``universality'' classes of theories have their critical points
mapped onto the
same fixed point, with the same exponents.
This can be very powerful: if, in the space of $(d-1)$-dimensional
theories with short-range interactions invariant under the same centre
symmetry, there is only a single fixed point, it reveals to us that a
$d$-dimensional gauge theory will have the same critical behaviour
as a $d$-dimensional spin system with the same symmetry.

MFT predicts that systems with a global $Z(3)$ symmetry should have
first-order transitions. The symmetry allows a general effective
potential depending on the cubic invariant $\Real L^3$, which we can
then expand around the origin, choosing $L$ to be real:
$$V(L)=f(|L|^2) + g(|L|^2,\Real L^3)=aL^2 + bL^3 + cL^4 + \ldots$$
A sufficiently large value of $a$ will give a unique minimum at $L=0$,
with a metastable minimum at $L\neq 0$. The true minimum will jump
to this second value when $a$ is reduced towards zero, so the
cubic term has produced a first-order transition. This argument has
been confirmed for $d\geq 4$, but is invalidated for $d=3$ by
topological excitations. For our interests, $SU(3)$ in $d=3$
dimensions should have the same critical
behaviour as the Z(3) Potts spin system, {\it viz.} a second-order
transition described by the following critical exponents:

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan7\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr \tableedge\tablerule\tablelines
&&\omit\hidewidth #3\hidewidth&&\omit\hidewidth #4\hidewidth&&
\omit\hidewidth #5\hidewidth&&\omit\hidewidth #6\hidewidth&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan7&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan7\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\ITi}{Critical Exponents}{Exponent}{Definition}{Regime}{Value}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&\it Magnetisation&&$<L(\vx)> \sim |T-T_c|^{\beta_M}$&&$T\geq
T_c$&&$\beta_M=0.11$&\cr
\tablelines\tablerule\tablelines
&&\it Susceptibility&&$\chi =\sum\Gamma(\vx) \sim
|T-T_c|^{-\gamma}$&&$T\leq T_c$&&$\gamma=1.44$&\cr
\tablelines\tablerule\tablelines
&&\it Specific heat&&$C=T\partial^2\ln Z/\partial T^2 \sim
|T-T_c|^{-\alpha}$&&$T\leq T_c$&&$\alpha=0.33$&\cr
\tablelines\tablerule\tablelines
&&\it Correlation length&&$\xi =T/\sigma \sim |T-T_c|^{-\nu}$&&$T\leq
T_c$&&$\nu=0.83$&\cr
\tablelines\tablerule\tablelines
&&\it Critical correlation&&$\Gamma(\vx) \sim
|\vx|^{-(d-2+\eta)}$&&$T=T_c$&&$\eta=0.27$&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

The critical coupling, for $SU(3)$ theory in $2+1$
dimensions, has previously been estimated\ref\IRxv{J.~Christensen,
G.~Thorleifsson, P.~H.~Damgaard and J.~F.~Wheater, \PL{276B}{1992}{472}}
as
\eqn\IExxv
{\beta_c=8.175\pm 0.002}
in the infinite-volume limit of a lattice with $N_t=2$, from
measurements of $\beta_c\approx 8.04, 8.11, 8.12$ and $8.14$ for
$L_z=L_x=20, 30, 40$ and $60$ respectively.
The coupling is related to the
temperature, as previously, by $\beta=12T/g^2$.

It has also been predicted\IRxiv\ that
$$<L>=(m^2a^2)^{(N^2-1)g^2/16\pi T_c},\qquad T\rightarrow T_c^+$$
and, leading from this, that
$$\beta_M=\frac{(N^2-1)g^2}{16\pi T_c}=\frac{6}{\pi
\beta_c}\approx 0.23\qquad\hbox{for $SU(3)$,}$$
but this is based on an approximate analytic calculation predating
universality arguments, and so cannot be treated as reliable.

\vfill\supereject\blankpagetrue\vbox to\vsize{}


==> lowtemp.tex <==
\newsec{Interface Properties}{Near the Critical Temperature}

\Subsec{Interface Behaviour Approaching Criticality}
In the previous chapter, we examined some properties of the $Z(3)$
interface at high temperatures, $\beta\gg\beta_c\approx 8.175$.
It was seen that the presence of a twist in our simulations is
sufficient to put the left- and right-hand longitudinal ends of the
lattice in different $Z(3)$ phases, with one physical $Z(3)$ interface
separating the two. At
these high temperatures, the phases are very well defined, with only
small fluctuations seen in the value of the order parameter (the
Polyakov line) across their extent. The interface is similarly well
defined, with a fairly rigid shape. Both of these aspects are due to
the suppression of fluctuations in phase resulting from the increased
energy penalty at high temperatures.

Consider, however, the phase structure at the critical temperature
itself, $\beta_c$, where the deconfinement transition occurs. At and
below this temperature, the three ordered,
$Z(3)$-broken phases cease to exist, being replaced by a single
disordered phase with symmetry restored. Obviously, therefore, no
$Z(3)$ interface can exist in this regime either. The order-disorder,
confinement-deconfinement transition itself has been studied in the
past. In \IRob, for instance, the surface tensions of
order-order and order-disorder interfaces were compared in $3+1$
dimensions near the phase
transition, and various thermodynamic properties were examined. Also,
the prediction of complete wetting,
mentioned in the introductory chapter, was tested: {\it viz.} that
an order-order
($Z(3)$) interface consists of two order-disorder ones stuck back to
back, so that $\alpha_{oo}\approx 2\alpha_{od}$.
A question that has not been addressed sufficiently in the past,
though, is that of the behaviour of the interface: how does 
this change from the rigid structure we see at high temperatures, as
we reduce the temperature towards the critical value? This chapter
aims to rectify this gap in our knowledge by
studying various properties of the $Z(3)$ interface at
temperatures just above the critical value.

So, then, what changes can we predict as the temperature drops?
To begin with, a decrease in temperature causes a corresponding
reduction in the energy penalty suppressing fluctuations in
phase. It follows that more and larger fluctuations, bubbles of
different phase, will appear
within the two main $Z(3)$ domains on the lattice, following from the
reduction in free energy of the bubble walls. Since the phase
transition at the critical point is second-order, one also expects the
expectation values of Polyakov lines in the two regions to converge
smoothly on
zero as the critical point is approached, this being the value taken in the
disordered phase below $\beta_c$. This means that the ``height'' of
the interface (the change in the real part of the Polyakov line as
one moves across it) will also decrease. These two consequences present a
double bind, with the interface decreasing in height just as the
surrounding fluctuations increase. As the interface becomes less and
less discernible amidst the phase turbulence, one might expect a detailed study
of its structure to become well nigh impossible near to the critical
temperature.

\ifig\IIIFi{Polyakov line (real part) profiles of the same $Z(3)$ interface at
different temperatures. The top left picture is identical to that of
\IIFia, with $\beta=50$ and a $2\times 24\times 96$ lattice. Going
from left to right, and then top to
bottom, the other pictures illustrate an interface between the same
phases ($<L>\approx e^{2\pi i/3}$ on
the left and the $<L>\approx 1$ on the right) for $\beta=10, 9, 8.5, 
8.3$ and $8.1$ respectively.}{\epsfxsize\hsize \epsfbox{betas.ps}}

The pictures of Polyakov lines shown in \IIIFi\ appear to confirm these
fears. One particular $Z(3)$ interface is shown at a series of
different temperatures, which drop towards the critical value. 
By the time $\beta\sim 10$, it is looking much more ragged than at the
high temperatures of the last chapter, illustrated in the first
picture. By the time $\beta<9$, the interface is difficult to spot at
all, much less study in detail. In the last picture, just below the
critical temperature, all traces of the interface have vanished, as
expected, and the Polyakov lines are fluctuating about zero.

The first question to address is that of the qualitative behaviour of
the interface as the temperature drops. Given that it must vanish at
$\beta_c$, several possibilities seem to present themselves:
\medskip

\item{1.} The interface maintains the rigid, taut structure seen at high
temperatures. It keeps its ``area'', defined as the Polyakov
``height'' multiplied by the lattice width, to a minimum,
by avoiding fluctuations in its shape. Its height shrinks
steadily until it reaches zero at the critical temperature, where the interface
consequently vanishes. Before this, though, it becomes invisible
amidst the growing fluctuations.
\medskip

\item{2.} The interface spreads out in the longitudinal direction,
following the behaviour of correlation lengths (such as the Debye
screening length)
on the lattice.
These diverge as the temperature approaches the critical
value, meaning that regions of phase separated by a large
distance on the lattice have an increasing effect on each other. The
interface thus reveals more and more disordered phase within, in
line with the prediction of complete wetting, and
as its height decreases and its width increases, talk of the interface
as a physical object becomes less and less meaningful.
\medskip

\item{3.} In addition to small bubbles of phase, many more entire
interfaces form across the lattice as the energy
penalty drops. These, together with the original interface, interact
with each other and with the fluctuating bubbles of phase, which are
also forming in increasing numbers. These interactions, collisions and
buddings off, eventually wash out all phase structure,
leaving disordered phase throughout the lattice, with the Polyakov line
averaging to zero. We would expect this behaviour to be suppressed by
increases in the transverse size of the lattice, and use a variety of
such sizes later in this chapter.
\medskip

\item{4.} The interface maintains a relatively narrow width, behaving
essentially as a one-dimensional object in the spatial dimensions ---
a string, stretching across the lattice --- but it
suffers increasingly violent transverse fluctuations, contorting its
shape and thereby increasing its
area ({\it i.e.} its length, disregarding the time dimension). The
fluctuations diverge towards the critical temperature, and
the interface eventually breaks into pieces to leave only disorder.
\medskip

As mentioned above,
it is fairly clear from \IIIFi\ that the interface has vanished by the
final picture ($\beta=8.1$), but the manner of its collapse remains
ambiguous. The fluctuations wash out the interface so much
that we cannot really rule out any of the possible behaviours at this
stage. Clearly, we need a better way to keep track of the interface
as the temperature drops, and this is the matter addressed in the next
section.

\subsec{Tracking the Interface}
One way to deal with the increase in phase fluctuations is to cut out
the highest frequency modes altogether. This can be achieved most
simply by a
``box-car'' average, where the Polyakov lines of each three-by-three
spatial array of points
are averaged over to give a new value, allocated to the central
point. Note that the periodic boundary conditions give the 
spatial dimensions the topology of a torus, so we have no edge effects
to worry about. The expectation value of the Polyakov line in a
region is unaffected by this averaging procedure.

\ifig\IIIFii{Smoothed Polyakov line profiles, produced by processing the
raw pictures of \IIIFi. As in that figure, $\beta=50, 10, 9,
8.5, 8.3$ and $8.1$ respectively.}{\epsfxsize\hsize \epsfbox{betas_smth.ps}}

The effect of smoothing out the fluctuations is shown dramatically in
the pictures of \IIIFii. These have been produced simply by applying the
box-car average to the pictures of \IIIFi.
To make things even clearer, the Polyakov lines
have first been re-binned so that the $24\times 96$ spatial dimensions
become $12\times 48$, with each two-by-two array being averaged to
one point. Now the $Z(3)$ interface can clearly be seen for all
but the last picture, {\it i.e.} for all temperatures above
$\beta_c$. The fact that the interface can still be seen for
temperatures just above the critical value gives encouragement to the belief
that a study of its structure should still be possible quite close to
the phase transition, and that the shape of the interface can be
monitored.

However, there is a drawback with this smoothing technique: it seems
less than ideal as a mechanism for
study of the interface, as it averages out a whole class of
fluctuations which may be important in the interface collapse. Thus,
we would like to find a better way to keep track of the interface. We shall,
though, use smoothing later on in conjunction with a more reliable method of
tracking the interface, and a comparison of the results will allow us
to judge how much distortion is introduced by smoothing.

A more satisfactory method is to produce a contour map from the real
part of the Polyakov lines on
the lattice. At its simplest, consider following a contour whose
height is mid-way between that of the average Polyakov line at the left-hand
end of the lattice and that at the right-hand end. This will pick out
the mid-height of the interface as it goes across the lattice, as well
as any bubbles of fluctuating phase which are large enough to cross
the contour height. The crucial point to note is that {\it only} the $Z(3)$
interface will cross the entire lattice, {\it i.e.} the only contour
that will wrap once around the lattice in the transverse direction is that
corresponding to the interface. In a sense, it has unit ``winding number'',
whereas any contour representing a bubble of phase will join up with
itself without a net crossing of any lattice boundary (winding number
zero). This gives us a way to tell the interface apart from any
fluctuations, and to identify the position of its mid-height. By
following contours at various heights between the two extremes, we can
study more of the structure of the interface. Also, the contours 
allow us to measure any fluctuations in the shape of the interface,
as well as its width in lattice units. The advantage of using contours
is that no prior processing of the Polyakov line data is
required. However, we can study contours of the box-car-averaged data
as well if we wish, as this may be useful very close to the
critical temperature.

\ifig\IIIFiii{Contour maps of raw and processed Polyakov lines for
$\beta=10$ on a $2\times 24\times 96$ lattice. These maps correspond
to the $\beta=10$ pictures of \IIIFi\ and \IIIFii\ respectively. The
contour levels are at $-0.25, 0, 0.25, 0.5$ and $0.75$, darker regions
corresponding to higher values.}
{\epsfxsize\hsize \epsfbox{contourmaps.ps}}

An example of a contour map is shown in \IIIFiii, for the same gauge
configuration as featured in the prior two diagrams for
$\beta=10$. Notice the interface in the centre of the maps,
represented by
the only contours going all the way across the lattice. The first
picture shows the raw data of \IIIFi; the second, the smoothed data of
\IIIFii, but without first re-binning into a $12\times 48$ lattice
in this case.

\subsec{Fixing the Interface Position}
The ideas behind contour following also solve another problem for us:
how to keep
the interface fixed in place. In the previous chapter, we allowed it
to execute a random walk along the lattice, as permitted by
translation invariance. This allowed the system to tunnel into
different $Z(3)$ vacua, producing a different $Z(3)$ interface each
time. However, this is unsuitable for our present purposes, as we wish
to study the profile of one particular $Z(3)$ interface without
interference from other vacua. Of course, the properties that we find
will apply equally to all the $Z(3)$ interfaces, but our measurement
techniques cope best with one particular interface. We need to stop
the interface wandering
through the twist, as this is the process by which the system tunnels.
Ideally, the interface should be held in place well away from the
twist, so that no part of it, even its wildest fluctuations, passes
through the twist.

How, then, can we pin the twist down in the longitudinal centre of the
lattice? One method might be to use a partial anti-twist, {\it i.e.}
premultiply just one or two plaquettes at $z=L/2$ by the inverse of
the factor used in the twist at $z=0$. If we inserted a full
anti-twist, it would just act as another change of variables, taking
the Polyakov lines which have been flipped by the twist back to their
original value, without physical consequence; no $Z(3)$ interface would
need to form. However, by flipping just one or two plaquettes rather
than the whole set across the lattice, we make it energetically
favourable for the Polyakov lines to flip at that position, whilst still
forcing the appearance of a physical interface because of the
untwisted state of most of the plaquettes.

The problems with this suggestion are twofold. First, an objection of
principle: this method of pinning is distinctly artificial, breaking
the translation invariance of the interface. How, then, can we be sure
that the behaviour of the interface is not be affected by the
procedure? The presence of the anti-twisted plaquettes, together with
the periodic boundary conditions in the transverse direction, fixes
the part of the interface at the boundary,
suppressing the even (cosinusoidal) fluctuations in the interface in
favour of the odd (sinusoidal) ones. Second, an objection of
practice: the anti-twist makes it energetically favourable for the
interface to form at its location, but we have already seen that
energetic considerations become less and less important as the
temperature drops towards the critical value, {\it i.e.} the penalty
for the interface to wander away from the anti-twist becomes less and
less. Thus, we need to introduce more and more anti-twisted plaquettes
as the temperature drops, in order to keep the interface pinned in
place. This causes more and more distortion in the fluctuations of
the interface. In computational trials, we found that this technique
was simply not effective at the sort of temperatures in which we were
interested.

A far more appealing approach is to
locate the position of the interface after each sweep of the
lattice, and then slide the whole gauge configuration along the
lattice until the interface is re-centred. Any link variables which
are shifted through the twist are multiplied by the appropriate
factor, so that there is no physical effect from the procedure. This
is clearly superior to using the anti-twist: there is no physical
effect and no violation of translation invariance, and it can be used
close to the critical temperature, for as long as the interface can be
located. This, therefore, is the method used in all following
simulations, unless stated otherwise.

\ifig\IIIFiv{The procedure for locating the interface, illustrated
for the $\beta=10$ configuration of previous figures, on a $2\times
24\times 96$ lattice. The raw Polyakov line profile is smoothed, and
then averaged in the transverse direction.}
{\epsfxsize\hsize \epsfbox{locator.ps}}

\subsec{Locating \& Profiling the Interface}
To find the position of the interface after each sweep of the lattice,
we construct a smoothed Polyakov profile using box-car averaging, as
above, and then average this profile in the transverse direction.
This process is illustrated in \IIIFiv. The
Polyakov line averages of this last profile are then averaged
separately at opposite ends, to give the long dotted lines marking the
top and bottom levels of the interface. Three evenly spaced contours
are then chosen between these two, as illustrated by the short
dotted lines crossing the interface. Starting from the (longitudinal)
centre of the lattice, the
algorithm searches for the nearest point to pass through the middle
contour level in the correct direction (increasing from left to
right). It is assumed that the Polyakov lines interpolate linearly
between neighbouring lattice sites. The point found is defined to be
the centre of the interface, and the
configuration is then shifted to reposition this at the centre of the
lattice. Given that this procedure is repeated after each sweep, it is
extremely unlikely that the algorithm will be misled by a large
fluctuation passing through the middle contour level; it will almost
certainly find the true interface first, as this will be closest to
the centre of the lattice.

To find a contour at a particular level, we return to the raw Polyakov
line data. For $x=0$, the algorithm follows a procedure similar to that above:
starting from the centre, $z=L_z/2$, it looks for the nearest point passing
through the contour level. Then, it considers the square of
points formed by the two neighbouring lattice sites at $x=0$ and the
corresponding sites at $x=1$.

\ifig\IIIFv{Options for the contour-following algorithm. Given a point
at the desired contour level on the lower side, the Polyakov lines at
the upper two corners determine the progress of the contour in cases
(i)-(iii). A plus (minus) sign indicates a Polyakov line value greater
(less) than
the contour level. The same corner configurations of
(iv) and (v) give two
possible contour directions; we choose between them by considering the
central average of the corner values. These pictures exhaust all
possibilities for the values of the lower corners given, but any general
configuration can be rotated and reflected into one of these.}
{\epsfxsize\hsgraph \epsfbox{contours.eps}}

\ifig\IIIFva{An interface contour is illustrated crossing the lattice:
the dashed line. The dotted line marks the average position of the
contour, at the longitudinal centre of the lattice. As the contour
twists and turns to cross some transverse lattice positions more than
once, we shall approximate it, where necessary, by the solid
contour, which crosses each transverse lattice position only once, at
the closest approach of the dashed contour to the central (dotted) line.}
{\epsfxsize\hsgraph \epsfbox{contour_approx.eps}}

The algorithm decides to which side of the square the contour should
go, as in \IIIFv. Denoting Polyakov line values which are greater or
less than the contour level by plus and minus signs respectively, the
five possible configurations illustrated determine the progress of the
contour. The last two are ambiguous, with a central average of the
four corner values used to decide which direction of the two
possibilities should be chosen, as shown. Once the destination side is
determined, the point at which the contour crosses that side is found
by extrapolating between the two relevant corners, as usual. Then,
starting with this side, the whole procedure continues. Eventually,
the contour must join up with itself. If it has wrapped across the
lattice exactly once in this process, it must be the contour
representing the interface; if not, it has merely identified a bubble
of phase, and can be discarded. Repeated application of this technique
for different contour levels determines the structure of the interface
to the desired precision. The same procedure can be applied to the
smoothed Polyakov line configurations, to obtain smoothed contour
maps.

In a tiny fraction of cases, the algorithm above may fail. For
instance, cases (iv) and (v) of \IIIFv\ cannot be distinguished with
certainty as Polyakov lines are only defined {\it on} the lattice
sites. Also, extremely close to the phase transition, the interface
may break up into several pieces, so that no contour goes all the way
across the lattice. In the event of such failure, a reserve method is
used to find the rough positions of the contours; in fact, this is the
same method as
originally used to locate the centre of the interface, but using
raw rather than smoothed Polyakov lines: for each
transverse position, $x$, the nearest point to the centre of the
lattice is found at which the Polyakov line passes through the desired
contour level in the correct direction ({\it i.e.} increasing or
decreasing with $z$, as appropriate for the interface).

Later, we shall need to define the interface just once for each transverse
lattice site, but at very low temperatures, the contour sometimes
twists and turns so much that it crosses some transverse values several
times. In these cases, we take the interface to be at that crossing point which
is closest to the average longitudinal position of the interface
across the lattice. This procedure is illustrated in \IIIFva, with the
solid contour being the approximation taken to the dashed
contour.

\subsec{Qualitative Results for Interface Behaviour}
To address the question posed in section 4.1 of how the interface
behaves near the critical temperature, we use the contour techniques
described above to follow the changes in its structure as the
temperature drops. We start by considering some results from our
simulations on a $2\times 36\times 72$ lattice. The length of the
lattice, seventy-two sites, was chosen after studies with various lengths,
to ensure that not even the wildest fluctuations of the interface would
reach as far as the twist during our full-length runs. The simulations
consisted, in each case, of 2k heat-bath sweeps and 100k main
sweeps. Since we were interested in the evolution of the interface,
contour measurements were taken after every sweep of the
lattice. Approximately 100---200 hours of CPU time on a DEC 2100 A500MP
machine were needed for each value of $\beta$, as shown in the
following table (occasionally, parts of simulations were performed on DEC 3000
machines; these times have been adjusted to compensate):

\bigskip\centerline{\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan3\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr \tableedge\tablerule\tablelines
&&#3&&#4&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan3&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan3\cr}
\halign to10cm{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & 
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\IIITi}{Simulation Times for $2\times 36\times 72$ lattice}
{$\beta$}{CPU time for 2k+100k Sweeps (hrs)}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&8.25&&96&\cr
\tablelines\tablerule\tablelines
&&8.35&&134&\cr
\tablelines\tablerule\tablelines
&&8.50&&152&\cr
\tablelines\tablerule\tablelines
&&8.75&&184&\cr
\tablelines\tablerule\tablelines
&&9.00&&197&\cr
\tablelines\tablerule}}\global\advance\tableno by1}}\bigskip


\ifigp\IIIFvi{Contour maps of the interface on a $2\times 36\times 72$
lattice, for decreasing temperature. Moving left to right, and then
top to bottom, the picture illustrates the interface structure around the
longitudinal centre of the lattice after
2k heat-bath and 60k main sweeps for $\beta=9, 8.75, 8.5, 8.35$ and $8.25$.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{contourtemps.ps}}

In \IIIFvi, a contour snapshot of the interface is shown for each
temperature studied, at the same point in each simulation: just over
halfway through. Three contours have been followed in each
case. We can see that the contours stay close together across most of
the interface, indicating that the interface remains relatively narrow
as the temperature drops. The quantitative behaviour of the interface
width will be studied more closely later in this chapter. However, the
shape of the interface appears to fluctuate rather more wildly with the
falling temperature. Again, a detailed study of the fluctuations will
be undertaken later in the chapter.

\ifig\IIIFvia{A contour map of the whole $2\times 36\times 72$ lattice for
$\beta=8.25$, corresponding to the last picture of \IIIFvi, showing
that only one interface exists.}
{\epsfxsize\hsize \epsfbox{contourtemps2.ps}}

These observations suggest a behaviour of the fourth type in section
4.1, with the interface retaining a relatively narrow width as it
approaches the critical temperature but suffering increasingly violent
fluctuations in shape. In \IIIFvi, only the central longitudinal
portion of the lattice is shown, to show the interface contours more
clearly. However, lest one wonder whether more interfaces are
appearing across the lattice further away from the one shown, 
we show in \IIIFvia\ the full structure
corresponding to the last picture of \IIIFvi. This demonstrates that
even at $\beta=8.25$, no other interfaces appear.
Only bubbles of phase form, increasing in size and occurrence as the
temperature drops and occasionally budding from the main interface or
recombining with it. As already mentioned, the interface does not
spread out noticeably in width, which we can define to be the average
difference in position
between the lowest and highest contour across the interface, and so it
appears to be relatively unaffected by the divergence of physical
correlation lengths such as the Debye screening length. Neither
does it remain in the sort of rigid shape of minimal ``area'' that we
saw at higher temperatures, following from the reduction in free
energy per unit area of the interface.

\ifigp\IIIFvii{Contour snapshots of the interface at various stages of
a $\beta=8.5$ run on a $2\times 36\times 72$ lattice, showing just the
central longitudinal portion of the lattice. Three contour levels were
chosen by the method of
\IIIFiv, with values as given in the first picture.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{contourevol.ps}}

\ifigp\IIIFviii{The same contour snapshots as in \IIIFvii, but this time
using the smoothed Polyakov lines.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{contourevol_sm.ps}}

The snapshots of \IIIFvii\ for $\beta=8.5$ give an idea of how the
interface continually changes
shape as it evolves in computer time. The initial configuration is
shown in the first picture: the lattice is set up to be in two
definite $Z(3)$ phases, with a sharp boundary between them midway
along the lattice, as
discussed in section 3.1. The configuration after the equilibration
sweeps have occurred is shown in the second picture, with the
physical $Z(3)$
interface broadening into an equilibrated shape. Pictures after this are
spaced at intervals of
20k main sweeps, showing some snapshots of the interface as it writhes
and twists. It is clear that the it maintains its narrow width,
but fluctuates
a great deal as bubbles of phase appear and disappear around it.
Note that the interface remains centred, and that the fluctuations are
not large enough to go beyond our field of view in the centre of the
lattice. This reassures us that the interface does not bump into the
twist at any time.

We also follow the interface evolution by contouring the smoothed
(box-car-averaged) configurations after each sweep, as illustrated in
\IIIFviii; the pictures shown are those from \IIIFvii, but from the
smoothed Polyakov lines rather than the raw ones.
Notice that we can identify the interface a great deal more clearly,
at the price of losing a great deal of phase structure. We continue
to monitor the smoothed configurations, as the greater clarity of the
interface may allow us to follow its behaviour closer to the critical
temperature than
the raw data alone. Later in this chapter, we shall
have the opportunity to
check how results from the smoothed data compare with those from the
raw data, and thus gauge the usefulness of this procedure. The
increase in computer time to keep track of the smoothed configurations
is extremely small.

\ifig\IIIFix{Polyakov line profile for $\beta=8.5$ on a $2\times
36\times 72$ lattice, produced by taking an average over all sweeps of
the transverse-averaged profile (see text). The
dotted line represents the best fit to a $\tanh$ function, giving the
Debye screening length (inverse mass); the value shown is actually
$(2m)^{-1}$, as discussed in section 2.4. The average interface width,
between the lowest (25\%) and highest (75\%) contours, is also shown.}
{\epsfxsize\hsize \epsfbox{domainwall.ps}}

To provide further evidence for the behaviour that we are suggesting
above, we take a transverse-averaged Polyakov profile of the lattice
after each sweep. Averaging this profile over all 100k
main sweeps, we obtain an average profile such as that of \IIIFix. Notice that
this average one-dimensional profile of the interface fits the
expected shape for an instanton interpolating between two vacua,
namely a $\tanh$ function, remarkably well. This is true even at
$\beta=8.25$, though the divergence from the $\tanh$ profile is more
noticeable at the lower temperatures; this is discussed briefly
in the next section but one.

We can determine the Debye mass of the
interface from the coefficient of the fitted $\tanh$ function, since we
expect the interface width to be of order the Debye screening length,
{\it viz.} the inverse of the Debye mass. We can also estimate the
intrinsic width of the interface, characterising the width at any
time and point of the interface, rather than the Debye screening
length, where all fluctuations are washed out to give the width of a
``fuzzy'' average interface. The intrinsic width is estimated by
taking the average distance between the
lowest contour, at 25\% of the height of the interface,
and the highest, at 75\%, all the way across the lattice, after
each sweep. The result for this case is shown in \IIIFix,
and full results for each type of width are given later in this chapter.

\subsec{Simulation Parameters}
Having established the qualitative features of the behaviour of the
interface near the critical temperature, we now proceed with a
detailed quantitative analysis of our results. Since we wish to
examine aspects of the interface behaviour as the
temperature drops to the critical value, we perform simulations for
the various values of $\beta$ mentioned previously; these are
tabulated below for easy reference. It will be seen later that it
is difficult for us to obtain reliable results closer to the critical
temperature than $\beta=8.25$.

\bigskip\centerline{\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan1\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#3&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan1&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan1\cr}
\halign to3in{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\IIITii}{Simulation Temperatures, $\beta$}
{8.25}
\tablelines\tablerule\tablelines
&&8.35&\cr
\tablelines\tablerule\tablelines
&&8.50&\cr
\tablelines\tablerule\tablelines
&&8.75&\cr
\tablelines\tablerule\tablelines
&&9.00&\cr
\tablelines\tablerule}}\global\advance\tableno by1}}\bigskip

For each value of $\beta$ in \IIITii, we carry out simulations with 2k
heat-bath and 100k main sweeps on
$2\times N_x\times 72$ lattices with a range of transverse lattice sizes,
$N_x$. This will allow us to examine the dependence of the interface
behaviour on its size, {\it i.e.} the lattice width.

\bigskip\centerline{\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan1\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#3&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan1&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan1\cr}
\halign to3in{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\IIITiii}{Simulation Lattice Widths, $L_x$}
{18}
\tablelines\tablerule\tablelines
&&24&\cr
\tablelines\tablerule\tablelines
&&30&\cr
\tablelines\tablerule\tablelines
&&36&\cr
\tablelines\tablerule\tablelines
&&42&\cr
\tablelines\tablerule\tablelines
&&48&\cr
\tablelines\tablerule\tablelines
&&54&\cr
\tablelines\tablerule}}\global\advance\tableno by1}}\bigskip

\subsec{Interface Wetting}
Before moving on, we pause briefly to consider the question of
interface wetting. As mentioned earlier, a $Z(3)$ interface is
believed to consist of two order-disorder interfaces stuck back to
back, enclosing a narrow slice of disordered (low-temperature)
phase. Evidence to support this theory has been provided by
simulations in $3+1$ dimensions\IRob, measuring the surface tension of
both types of interface at the critical temperature, and it seems
reasonable that the same behaviour should be seen in $2+1$
dimensions. As we do not measure the properties of order-disorder
interfaces in this survey, it is worth considering whether we can see
any indication of the wetting behaviour in our study of the $Z(3)$
interface alone. At the critical temperature itself, complete wetting
would suggest that the interface profile should split in two to include an
area of disordered ($<L>=0$) phase. Although average profiles akin to \IIIFix\
show slightly more divergence from the $\tanh$ form at lower $\beta$,
it is not possible to see such a splitting clearly in our system. However, we
would expect any area of disordered phase within the interface to
remain extremely small until
$\beta\approx\beta_c=8.175$\ref\IIIRii{T.~Trappenberg and U.-J.~Wiese,
\NP{B372}{1992}{703}}, and
so we cannot take this as evidence against wetting in $2+1$ dimensions.

\ifig\IIIFixa{Polyakov line profiles for $\beta=8.15$ on a $2\times
48\times 200$ lattice, produced by taking instantaneous transverse
averages at fifty-sweep intervals.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{wetting.ps}}

We cannot obtain reliable average profiles much below $\beta=8.25$
because of the difficulty of identifying the interface so close to
collapse, in order to keep it centred for the average. Another
approach to the problem which can be followed at lower $\beta$,
though, is artificially to split the interface into two by changing
the initial conditions to include a
large area of disordered phase between the two ordered domains. The
persistence, or otherwise, of this interface structure can then be
examined at various $\beta\approx\beta_c$. In
\IIIFixa, instantaneous profiles are shown at fifty-sweep intervals on
a long lattice at $\beta=8.15$ (actually just above $\beta_c$ for our
finite-sized system). Disordered phase is present only where both left-
{\it and} right-hand plots ({\it i.e.} real {\it and} imaginary
Polyakov profiles) coincide with the dotted line ($<L>=0$: disordered
phase). The disordered region given by the initial conditions is
seen not to persist, but rather quickly dissolves into many bubbles of
$Z(3)$ phase. Again, this cannot be taken as strong evidence against
complete wetting, because of the imprecise nature of the observation;
but neither does there seem anything in our observations which could
be taken as positive evidence of the wetting.

\subsec{Estimates of the Critical Coupling and the Magnetisation Exponent}
We now proceed to more concrete measurements of interface properties.
We know that the expectation values of the Polyakov lines in
the main phases to either side of the interface must tend to zero as
the temperature descends to its critical value, since the disordered
phase which exists below that temperature has the $Z(3)$ vacuum
symmetry restored: $<L>=0$. This means that by monitoring the average
values of $<L>$ at either end of the lattice, which can be read off
from graphs such as \IIIFix, one can obtain an estimate for the
critical temperature itself, and also the magnetisation exponent, $\beta_M$,
determining the fall in the Polyakov expectation:
$$<L> \sim (\beta-\beta_c)^{\beta_M},\qquad \beta\geq\beta_c.$$
Our estimates of the Polyakov line expectations at opposite ends of
the lattice are given in the following tables for each simulation
performed, along with an average value thence obtained for each value
of $\beta$:

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\IIITia\xdef\IIITia{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<L>_L$}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ \ddots\ L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Average}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&-0.15414&&-0.15975&&-0.15421&&-0.16121&&-0.16205&&-0.16053&&-0.16360&&-0.1594(37)&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&-0.18135&&-0.18355&&-0.18407&&-0.18655&&-0.18585&&-0.18511&&-0.18647&&-0.1847(19)&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&-0.20172&&-0.20304&&-0.20348&&-0.20306&&-0.20409&&-0.20379&&-0.20457&&-0.2034(9)&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&-0.22241&&-0.22277&&-0.22247&&-0.22296&&-0.22306&&-0.22286&&-0.22340&&-0.2228(3)&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&-0.23644&&-0.23666&&-0.23687&&-0.23685&&-0.23724&&-0.23715&&-0.23711&&-0.2369(3)&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\IIITib\xdef\IIITib{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<L>_R$}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ \ddots\ L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Average}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&0.33667&&0.33570&&0.32767&&0.34012&&0.33955&&0.33600&&0.33651&&0.3360(41)&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&0.37655&&0.37486&&0.37494&&0.37491&&0.37511&&0.37453&&0.37612&&0.3753(7)&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&0.40925&&0.40898&&0.40797&&0.40816&&0.40895&&0.40908&&0.40855&&0.4087(5)&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&0.44595&&0.44575&&0.44549&&0.44665&&0.44629&&0.44620&&0.44635&&0.4461(4)&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&0.47399&&0.47416&&0.47412&&0.47340&&0.47391&&0.47452&&0.47407&&0.4740(3)&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

The figures from each simulation come from the transverse-averaged
Polyakov profiles, averaging over all 100k main sweeps, and then
averaging over the six longitudinal points at each end of the lattice
($0\leq z \leq 5$ and $66\leq z \leq 71$). The errors from a given
simulation are $O(10^{-6})$, decreasing to $O(10^{-7})$ for the larger
$\beta$ values, and are not shown, being negligible compared to the
error between different simulations, which is included with the average.

\ifig\IIIFx{A three-parameter fit for the critical temperature, $\beta_c$, and
the magnetisation exponent, $\beta_M$, from the expectation value of
the Polyakov line deep in the phases at the right- and left-hand ends
of the lattice (denoted by ``R.H.'' and ``L.H.'' respectively), as
found from averaged profiles such as \IIIFix.}
{\epsfxsize\hsize \epsfbox{exponent.ps}}

\ifig\IIIFxa{A two-parameter fit for the magnetisation exponent,
$\beta_M$, using $\beta_c=8.14$.}
{\epsfxsize\hsize \epsfbox{exponent2.ps}}

An accurate fit to the form $$<L>=a(\beta-\beta_c)^{\beta_M}$$ is
difficult, since we only have five points and must fit three parameters.
Using the gradient expansion fitting of {\it IDL}'s function
``CURVEFIT'', we plot the average values from the tables in \IIIFx.
The independent estimates from each of the two $Z(3)$ phases give the
following results for the critical temperature and magnetisation exponent:

$$\beta_c = 8.170(5),$$

$$\beta_M = 0.159(3).$$

These are some distance from the values of $\beta_c\approx 8.14$ and
$\beta_M\approx 0.13$ obtained in \ref\IIIRi{J.~Christensen, G.~Thorleifsson,
P.~H.~Damgaard and J.~F.~Wheater, \NP{B374}{1992}{225}}, the estimate
for $\beta_c$ being closer to the continuum estimate of $8.175$ than
to the value of $8.14$ which broadly corresponds to our lattice sizes.
As a check, \IIIFxa\ shows our estimates for $\beta_M$ if we assume
that $\beta_c=8.14$; the estimates are little changed.

\subsec{Quantitative Results}
Having established that the interface remains as a thin, localised
object even very close to the critical temperature, we now wish to
examine its behaviour in more quantitative detail. To do this, we need
a way to quantify the fluctuations in the interface. The phase
transition is second-order, with the Polyakov lines (and the
interface) vanishing smoothly at $\beta_c$; thus, we expect the 
fluctuations to diverge as $\beta\rightarrow \beta_c$, 
and we wish to quantify this divergence.

\ifig\IIIFxi{An interface contour is illustrated crossing the lattice:
the bold line. The dotted line marks the average position of the
contour, at the longitudinal centre of the lattice. We quantify the
fluctuations in the interface shape by the displacement, $\phi(x)$, from the
average position at each point $x$ across the lattice.}
{\epsfxsize\hsgraph \epsfbox{moments.eps}}

Illustrated in \IIIFxi\ is a contour going across the lattice, with
displacements from its average position at transverse location $x$
given by $\phi(x)$. To characterise the fluctuations, we monitor the
fluctuation ``moments'', where the $n$th moment is defined to be
$<\phi(x)^n>$. We track the first six moments ($1\leq n\leq 6$) in our
simulations; higher moments are subject to unacceptably large errors.
We take a separate average for each transverse position across the
lattice, and, because of the translation invariance of the interface, we
expect the moments to be roughly constant across the lattice after a
large number of sweeps.

First of all, we need to examine the qualitative behaviour of the
fluctuation moments. As mentioned above, we expect the moments to be
essentially constant across the lattice, owing to the periodic boundary
conditions in the transverse direction and the translation invariance
of the interface. Of course, we would expect the moments to approach
constancy more closely with increasing simulation length.

\ifigp\IIIFxii{The first six moments for $\beta=8.5$ on a $2\times 36\times 72$
lattice, shown separately for each of the three contour levels
followed. These are averages over 100k sweeps for the raw Polyakov data.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{momentsample.ps}}

\ifigp\IIIFxiii{The first six moments for $\beta=8.5$ on a $2\times
36\times 72$
lattice, shown separately for each of the three contour levels
followed. These are averages over 100k sweeps for the smoothed
Polyakov data corresponding to \IIIFxii.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{momentsample_sm.ps}}

The following graphs show some moments for $\beta=8.5$, averaged
over the full 100k sweeps. Separate sets of data are shown for each of
the three contours followed, at 25\%, 50\% and 75\% of the height of the
interface respectively. The qualitative behaviour is roughly the same
for each contour. The upper and lower contours are subject to
rather more fluctuation than the middle one, as we expect since they
are closer to the outside of the interface and therefore more susceptible
to bubbles of phase forming nearby and distorting the edge of the
interface. The even moments are fairly
constant across the lattice, whilst the odd moments are very much smaller
and show more variation. Note that the first moment must average to zero
across the lattice, by definition, and we likewise expect all odd
moments to be comparatively close to zero, becoming closer with even
longer runs.

In \IIIFxiii, we show the moment data from the smoothed contours
measured in the same simulation as \IIIFii. One can see that the
behaviour is very similar to the raw data, both qualitatively and
quantitatively. Since this may indicate that the smoothed data has not
lost a significant amount of information about the fluctuations,
we shall present our data later on
for both raw and smoothed moments, in order to compare the two.

\vfill\supereject

\subsec{A Toy Model: A Scalar Field Theory with Associated Feynman Rules}
Since the interface has been shown to behave as a fluctuating, narrow
object, winding across the lattice, it may be helpful to think about
it as a one-dimensional object, {\it viz.} a string. At high
temperatures, the string
stretches tightly across the lattice, its length being equal to
the transverse size of the lattice. At low temperatures, though, if
coils and twists ever more violently, and loops form which break off and
recombine with it, representing bubbles of $Z(3)$ phase. If we take
this picture further, we can consider the possibility of describing
the string in terms of a one-dimensional field theory. The scalar
field in this case is simply the displacement of the string from
equilibrium at a position $x$ along its length: $\phi(x)$. At high
temperatures, we essentially have a free field theory; at low
temperatures, we need an interaction term to account for the breaking off
and recombination of loops of string.

To preserve the translation invariance of the interface, the
Lagrangian cannot depend directly on $\phi(x)$, but instead must depend
only on the derivative $\del_x\phi(x)$. We keep the normal kinetic
term for a scalar field theory, and add a quartic interaction term; a
cubic interaction is ruled out by ``parity'', as we expect the
interface to be invariant under $\phi\rightarrow -\phi$. Thus, we have a
Lagrangian of the form
\eqn\EIVi
{\CL=\half\gamma(\del_x\phi)^2 + \tfrac{\lambda}{4!}(\del_x\phi)^4,}
where $\gamma$ and $\lambda$ are both unknown functions of $\beta$. By
examining the dependence of the fluctuations on the temperature, we
shall be able to determine these functions. Since we expect the
fluctuations to diverge as $\beta\rightarrow\beta_c$, this implies
that $\gamma$ and $\lambda$ will both be functions of
$(\beta-\beta_c)$.

To test how well this toy model describes the actual behaviour of the
$Z(3)$ interface, we need to calculate the correlation functions of
$\phi$, which we can then compare with the behaviour seen. The
$n$-point connected vacuum correlation function at point $x$, $<\phi(x)^n>$,
corresponds to the $n$th Wick-subtracted
fluctuation moment at the same point. The Wick subtracted moments,
denoted by the subscript ``Ws'', are
given, as is well known, by the following relations:
$$\eqalign{
\hbox{2nd Moment:}\qquad<\phi^2>_{Ws}&=<\phi^2>,\cr
\hbox{4th Moment:}\qquad<\phi^4>_{Ws}&=<\phi^4>-3<\phi^2>^2,\cr
\hbox{6th Moment:}\qquad<\phi^6>_{Ws}&=<\phi^6>-15<\phi^2>^3-15<\phi^2><\phi^4>_{Ws}.}$$
For the Lagrangian above, the odd
correlation functions are zero, so we expect all the odd moments to be
zero. To calculate the even moments, we need to calculate the
appropriate vacuum diagrams.

\ifig\IIIFxiv{The vacuum diagrams corresponding to the 2nd, 4th and 6th
connected vacuum correlation functions respectively. The open circle
simply denotes point $x$, the endpoint of each external leg; the
solid circle denotes an interaction vertex, $\lambda$; and the
momentum travelling along a leg is denoted by $k$.}
{\epsfxsize\hsize \epsfbox{diags.eps}}

These diagrams are shown in \IIIFxiv, with the momenta denoted by the
$k$'s, and the four-way vertices marked by $\lambda$, corresponding to
the interaction term in the Lagrangian. The diagrams shown are the
lowest-order Wick-subtracted diagrams with two, four and six legs
respectively leaving the point $x$. To perform the calculations,
we need to derive Feynman rules for a $(\del_x\phi)^4$ theory, rather
than the usual $\phi^4$, and we do this now.

The path integral, for our one spatial dimension only, is
$$W[J]=N\int\CD\phi e^{\int dx (\CL(\phi,\del_x\phi) + J\phi)},$$
where $N$ is the normalisation and $\CL$ is given by \EIVi, written in
the form
$$\CL=\CL_0+\CL_{int}(\del_x\phi),\qquad
\CL_0=\half\gamma(\del_x\phi)^2,\qquad
\CL_{int}=\textstyle{\frac{\lambda}{4!}}(\del_x\phi)^4.$$
In the absence of the interaction,
$$W[J]=W_0[J]=Ne^{\half\int dx dy J(x)\Delta_F(x-y) J(y)},$$
with the Feynman propagator for the scalar field,
$$\Delta_F(x-y)=\int\frac{dp}{2\pi\gamma} \frac{e^{ip(x-y)}}{p^2}.$$
To include the interaction, we expand $W[J]$ as a power series in
$\lambda$:
$$\eqalign{
W[J]&=e^{dx \CL_{int} (\frac{\delta}{\delta J(x)})} W_0[J]\cr
&=\bigg[ 1 + \int dx \CL_{int}\big (\frac{\delta}{\delta J(x)}\big ) +
\ldots \bigg] W_0[J]\cr
&=W_0[J] + \frac{\lambda}{4!}\int dx \bigg(\frac{\del}{\del x}
\frac{\delta}{\delta J(x)}\bigg )^4 W_0[J] + \ldots.}$$
Now,
$$\frac{\del}{\del x} \frac{\delta W_0}{\delta J(x)} = \int dy \del_x
[\Delta_F(x-y)] J(y) W_0[J],$$
and further differentiation of this yields
$$\eqalign{
W[J]=\bigg\{ 1 + \frac{\lambda}{4!}\int dx \bigg[\ &3(\del^2_x
\Delta_F(0))^2\cr +
&6 \int dy_1 dy_2
\del^2_x[\Delta_F(0)\del_x[\Delta_F(x-y_1)\del_x[\Delta_F(x-y_2)]]]
J(y_1)J(y_2)\cr
+ &\int dy_1 dy_2 dy_3 dy_4 \del_x[\Delta_F(x-y_1)
\del_x[\Delta_F(x-y_2)\cr
&\times \del_x[\Delta_F(x-y_3)
\del_x[\Delta_F(x-y_4)]]]] J(y_1) J(y_2) J(y_3) J(y_4)\cr
+ &\ldots \bigg]
\bigg\} W_0[J].}$$

The free-field Green's functions are defined by
$$\CG^{(n)}(x_1,\ldots,x_n)=\frac{\delta^nW[J]}{\delta
J(x_1)\ldots\delta J(x_n)}\big |_{J=0},$$
giving the propagator
$$\CG^{(2)}(x_1,x_2)=\Delta_F(x_1-x_2).$$ 
The connected Green's functions are defined by
$$G^{(n)}(x_1,\ldots,x_n)=\frac{\delta^nX[J]}{\delta
J(x_1)\ldots\delta J(x_n)}\big |_{J=0},\qquad X[J]=\ln W[J],$$
giving interaction term
$$\eqalign{
G^{(4)}(x_1,x_2,x_3,x_4)&=\lambda\int dx \del_x[\Delta_F(x-x_1)
\del_x[\Delta_F(x-x_2) \del_x[\Delta_F(x-x_3) \del_x[\Delta_F(x-x_4)]]]]\cr
&=\lambda\int dx (-\del_{x_1}[\Delta_F(x-x_1)])
(-\del_{x_2}[\Delta_F(x-x_2)])\cr
&\qquad\qquad\qquad\times (-\del_{x_3}[\Delta_F(x-x_3)])
(-\del_{x_4}[\Delta_F(x-x_4)]).}$$
Converting to momentum space,
$$\eqalign{
\tilde G^{(4)}(p_1,p_2,p_3,p_4)&(2\pi)^4\delta(p_1+p_2+p_3+p_4)\cr
&=\int dx_1 dx_2 dx_3 dx_4 G^{(4)}(x_1,x_2,x_3,x_4)
e^{-i(p_1x_1+p_2x_2+p_3x_3+p_4x_4)},}$$
and, integrating by parts,
$$\int dx_1 \del_{x_1} \Delta_F(x_1-x) e^{-ip_1x_1}=ip_1\int
\Delta_F(x_1-x) e^{-ip_1x_1}.$$
Thus, each vertex picks up a factor of
$$\tilde G^{(4)}(p_1,p_2,p_3,p_4)=\lambda
p_1p_2p_3p_4.\qquad\hbox{where}\qquad p_1+p_2+p_3+p_4=0.$$

\subsec{Field Theoretic Predictions for Fluctuation Moment Behaviour}
In the continuum, therefore, the Feynman
diagrams of \IIIFxiv\ are given by the following formulae:
$$\eqalign{
<\phi(x)^2>&=\frac{1}{2\pi\gamma}\int \frac{dk}{k^2},\cr
<\phi(x)^4>_{Ws}&=\frac{\lambda}{4!}\frac{1}{(2\pi\gamma)^4}\int
\frac{dk_1}{k_1^2}\ldots\frac{dk_4}{k_4^2}
e^{-i(k_1+k_2+k_3-k_4)x}\cr
&\qquad\qquad\times 2\pi k_1k_2k_3k_4\delta(k_1+k_2+k_3-k_4),\cr
&=\frac{\lambda}{4!\gamma^4}\frac{1}{(2\pi)^3}\int
\frac{dk_1}{k_1}\frac{dk_2}{k_2}\frac{dk_3}{k_3}
\frac{1}{(k_1+k_2+k_3)},\cr
<\phi(x)^6>_{Ws}&=\frac{\lambda^2}{2!}\frac{1}{(2\pi\gamma)^7}\int
\frac{dk_1}{k_1^2}\ldots
\frac{dk_7}{k_7^2}
e^{-i(k_1-k_2-k_3+k_4+k_5-k_6)x}\cr
&\qquad\qquad\times (2\pi)^2 k_1k_2k_3k_4k_5k_6k_7^2
\delta(k_1-k_2-k_3-k_7) \delta(k_4+k_5-k_6+k_7)\cr
&=\frac{\lambda^2}{2!\gamma^7}\frac{1}{(2\pi)^5}\int
\frac{dk_2}{k_2}\frac{dk_3}{k_3}\frac{dk_4}{k_4}\frac{dk_5}{k_5}dk_7
\frac{1}{(k_2+k_3+k_7)}\frac{1}{(k_4+k_5+k_7)}.}$$

Note that there is no exponential in the first formula, as the
propagator starts and finishes at the same point, $x$. Also, the
symmetry factor in the last formula is from
$\frac{1}{2!}\times(\frac{1}{4!})^2\times (4\times 3\times 2)^2
 = \frac{1}{2!}$, from the two vertices, the four legs
per vertex, the number of legs connected to $x$, and the number
connected within the loop respectively.

Since we are working on a finite space of extent $L_x$, we have to
replace the integrals over $k$ with sums over integers $n$, putting
$k=2\pi n/L_x$:
$$\frac{1}{2\pi} \int dk \rightarrow \frac{1}{L_x}\sum_{n=1}^\infty.$$
Using the numerically-calculated results
$$\sum_n \frac{1}{n^2} = \frac{\pi^2}{6},\qquad
\sum_{n_a\ldots n_c}\textstyle{\frac{1}{n_a}\frac{1}{n_b}\frac{1}{n_c}
\frac{1}{(n_a+n_b+n_c)}}\approx 6.49(1)$$
$$\hbox{and}\qquad \sum_{n_a\ldots
n_e}\textstyle{\frac{1}{n_a}\frac{1}{n_b}\frac{1}{n_c}\frac{1}{n_d}
\frac{1}{(n_a+n_b+n_c)}\frac{1}{(n_a+n_d+n_e)}} \approx 60(1),$$
we obtain the following expressions:
$$\eqalign{
<\phi(x)^2>&=\frac{L_x}{(2\pi)^2\gamma}\sum_n
\frac{1}{n^2}=\frac{L_x}{24\gamma},\cr
<\phi(x)^4>_{Ws}&=
(6.49(1))\frac{\lambda}{4!}\frac{L_x}{(2\pi)^4\gamma^4},\cr
<\phi(x)^6>_{Ws}&=
(60(1))\frac{\lambda^2}{2!}\frac{L_x}{(2\pi)^6\gamma^7}.}$$

Note that the above expressions for the
correlation functions do not depend on the position $x$, so we now write
$\phi(x)$ simply as $\phi$. This confirms our original assertion that
the fluctuation moments should be constant across the lattice. In
future, we shall work with the average of a fluctuation moment across
the lattice.
Now, since the action, $\CS=\int \CL dx$, must be a dimensionless
quantity, and assuming $\gamma$ to be dimensionless, we find that
$\phi$ must have space dimension $\half$, and
coupling $\lambda$ dimension 1. Thus, as the only
fundamental length in our space is $L_x$, this implies that
$\lambda\sim L_x$, or $\lambda=\lambda_0 L_x$.
Substituting this dependence into the previous expressions, we obtain
the following predictions:
$$<\phi^2>\sim L_x,\qquad <\phi^4>_{Ws}\sim L_x^2
\qquad\hbox{and}\qquad <\phi^6>_{Ws}\sim L_x^3.$$
Checking the $L_x$-dependence of our results will thus help to verify
whether the scalar field theory really is a good model for the
interface fluctuations. However, the above calculations have all been
for the continuum, so we first need to calculate some corrections.

We have neglected the fact that we are
working on a lattice with site spacing $a$ and periodic boundary
conditions. To take this into account, we need to replace $k^2$ with
$4\sin^2(ak/2)$. This is equivalent to the following change in our
sums over $n$:
$$\frac{1}{k^2}=\bigg (\frac{L_x}{2\pi n}\bigg )^2\rightarrow
\frac{1}{4\sin^2(\pi na/L_x)}=\frac{1}{4\sin^2(\pi n/N_x)}.$$
We now calculate the corrections to our previous expressions which
result from this change.

First, we tackle the two-point function. To do this, we calculate the
sum from an integral, working with an expansion in the small parameter
$\xi$:
$$\int_\frac{\pi}{N_x}^\frac{(N_x-1)\pi}{N_x}\frac{1}{\sin^2 x} dx =
2\int_\frac{\pi}{N_x}^\frac{\pi}{2} \frac{1}{\sin^2 x} dx =
2\sum_{n=1}^{\frac{N_x}{2}-1}\int_0^\frac{\pi}{N_x} \frac{1}{\sin^2 (\frac{\pi
n}{N_x} + \xi)} d\xi.$$
Consider the $n=1$ term:
$$\int_0^\frac{\pi}{N_x}\frac{1}{\sin^2(\frac{\pi}{N_x}+\xi)}d\xi=\frac{\pi/N_x}{\sin^2(\pi/N_x)}
- \frac{N_x}{2\pi} + \CO[(\pi/N_x)^3].$$
Similarly, for the $n>1$ terms,
$$\eqalign{
\sum_{n=2}^{\frac{N_x}{2}-1} \int_0^\frac{\pi}{N_x} \frac{1}{\sin^2
(\frac{\pi n}{N_x} + \xi)} d\xi &= \sum_{n=2}^{\frac{N_x}{2}-1}
\int_0^\frac{\pi}{N_x} \bigg[\csc^2(\frac{\pi n}{N_x}) - 2\xi\cot(\frac{\pi
n}{N_x})\csc^2(\frac{\pi n}{N_x})\cr
&\qquad + 3\xi^2\bigg(\cot^2(\frac{\pi
n}{N_x})\csc^2(\frac{\pi n}{N_x}) + \frac{1}{3}\csc^2(\frac{\pi
n}{N_x}\bigg)+\ldots \bigg]d\xi\cr
&=\frac{\pi}{N_x}\sum_{n=2}^{\frac{N_x}{2}-1}\csc^2(\frac{\pi n}{N_x})
\quad - \quad\bigg(\frac{\pi}{N_x}\bigg )^2\sum_{n=2}^{\frac{N_x}{2}-1}
\cot(\frac{\pi n}{N_x})\csc^2(\frac{\pi n}{N_x})\cr
&\qquad +\bigg(\frac{\pi}{N_x}\bigg
)^3\sum_{n=2}^{\frac{N_x}{2}-1}\bigg(\cot^2(\frac{\pi
n}{N_x})\csc^2(\frac{\pi n}{N_x}) + \frac{1}{3}\csc^2(\frac{\pi
n}{N_x})\bigg) + \ldots\cr
&=\frac{\pi}{N_x}\sum_{n=2}^{\frac{N_x}{2}-1}\bigg(\csc^2(\frac{\pi n}{N_x})
+\frac{N_x}{\pi}(\textstyle{-\frac{1}{n^3}+\frac{1}{n^4}-\ldots})\bigg) +
\CO[(\pi/N_x)^3].}$$
Now,
$$\sum_{n=2}^{\frac{N_x}{2}-1}(-\tfrac{1}{n^3}+\tfrac{1}{n^4}-\ldots)=\sum_{n=2}^{\frac{N_x}{2}-1}\textstyle{\frac{-1}{n^2(n+1)}}=\frac{1}{2}
- (\frac{\pi^2}{6}-1) + \CO[(2/N_x)^3].$$
Thus, our result for the original integral, dropping
$\CO[(\pi/N_x)^3]$ terms and above, is
$$\frac{2\pi}{N_x}\sum_{n=1}^{\frac{N_x}{2}-1}\csc^2(\frac{\pi
n}{N_x}) - \frac{2N_x}{\pi}(\frac{\pi^2}{6}-1)
=\frac{\pi}{N_x}\sum_{n=1}^{N_x-2}\csc^2(\frac{\pi n}{N_x})
+\frac{N_x}{\pi}(3-\frac{\pi^2}{3}).$$
This series expansion in $N_x^{-1}$ must be equal to the value of the
original integral,
$$[-\cot x]^\frac{(N_x-1)\pi}{N_x}_\frac{\pi}{N_x} =
2\cot\frac{\pi}{N_x} = 2(\frac{N_x}{\pi} - \frac{\pi}{3N_x} +
\ldots),$$
so our final result is that
$$\frac{1}{N_x}\sum_{n=1}^{N_x-2} \csc^2(\frac{\pi n}{N_x}) \approx
\frac{N_x}{\pi^2}\bigg(\frac{\pi^2}{3}-1\bigg) - \frac{2}{3N_x}.$$
The correction to our original prediction, that $<\phi^2>\sim N_x$, is
negligible for our purposes (about 0.3\% for $N_x=18$). We assume that
the corrections to the higher moments are similarly negligible, as the
calculation of these lattice corrections is considerably more difficult.

\subsec{Observed Behaviour of Fluctuation Moments}
We now compare these predictions with the results that we obtain from
our computer simulations. Tables 4.6-8 list a sample set of results
for a contour halfway up the interface, using raw ({\it i.e.}
unprocessed) data. An estimate of each even moment is presented for
each value of $\beta$ and $L_x$, together with the calculated gradients
of log--log plots of the moments against $(\beta-\beta_c)$ or $L_x$
as appropriate, which give the power-law dependence of the moments on
these quantities.
To examine the behaviour of the interface more
fully, we tracked fluctuations in a total of three contours, defined
to be equally spaced between the top and bottom of the interface. For
each of these three contours, we also measured the fluctuations in the
interface after smoothing, to see whether the procedure would affect
results. Appendix B lists complete results for all three contours
used, and both raw and smoothed Polyakov data. In this chapter, tables
4.9-11 summarise the power-law dependence of the moments from each dataset on
$L_x$, while tables 4.12-14 give the equivalent dependence on $\beta-\beta_c$.

\goodbreak\pageinsert{
\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTii\xdef\BTii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^2>$ from Raw Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$6.87^{+0.22}_{-0.14}$&&$8.27^{+0.12}_{-0.03}$&&$12.3^{+0.2}_{-0.2}$&&$14.4^{+0.1}_{-0.1}$&&$17.8^{+0.1}_{-0.1}$&&$20.8^{+0.1}_{-0.2}$&&$23.1^{+0.2}_{-0.1}$&&${}_{ 1.20\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$5.02^{+0.20}_{-0.01}$&&$6.71^{+0.05}_{-0.05}$&&$9.14^{+0.09}_{-0.05}$&&$11.4^{+0.1}_{-0.1}$&&$13.4^{+0.1}_{-0.1}$&&$16.5^{+0.1}_{-0.1}$&&$18.2^{+0.1}_{-0.1}$&&${}_{ 1.21\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$3.93^{+0.03}_{-0.03}$&&$5.19^{+0.03}_{-0.04}$&&$7.17^{+0.05}_{-0.05}$&&$8.89^{+0.07}_{-0.05}$&&$10.0^{+0.1}_{-0.1}$&&$11.9^{+0.1}_{-0.1}$&&$13.8^{+0.1}_{-0.1}$&&${}_{ 1.15\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$3.07^{+0.02}_{-0.02}$&&$4.21^{+0.03}_{-0.03}$&&$5.32^{+0.04}_{-0.03}$&&$6.34^{+0.05}_{-0.04}$&&$7.63^{+0.06}_{-0.05}$&&$8.85^{+0.07}_{-0.05}$&&$9.57^{+0.06}_{-0.06}$&&${}_{ 1.05\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$2.62^{+0.01}_{-0.02}$&&$3.44^{+0.02}_{-0.02}$&&$4.38^{+0.03}_{-0.02}$&&$5.27^{+0.03}_{-0.03}$&&$6.29^{+0.05}_{-0.03}$&&$7.37^{+0.05}_{-0.05}$&&$7.89^{+0.04}_{-0.06}$&&${}_{ 1.03\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.41\pm 0.01}$&&${}_{-0.37\pm 0.02}$&&${}_{-0.44\pm 0.02}$&&${}_{-0.43\pm 0.03}$&&${}_{-0.44\pm 0.02}$&&${}_{-0.45\pm 0.03}$&&${}_{-0.46\pm 0.04}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTv\xdef\BTv{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^4>_{Ws}$ from Raw Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$2270^{+480}_{-180}$&&$334^{+125}_{-1.}$&&$967^{+343}_{-86}$&&$463^{+141}_{-21}$&&$492^{+58}_{-24}$&&$585^{+16}_{-13}$&&$690^{+31}_{-10}$&&${}_{-0.54\pm 0.27}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$775^{+349}_{-12}$&&$63.1^{+2.4}_{-1.9}$&&$111^{+5}_{-2}$&&$166^{+6}_{-5}$&&$199^{+6}_{-6}$&&$344^{+24}_{-14}$&&$299^{+11}_{-8}$&&${}_{ 1.31\pm 0.49}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$19.5^{+0.7}_{-0.6}$&&$28.3^{+0.9}_{-0.8}$&&$59.7^{+2.1}_{-1.7}$&&$82.5^{+3.3}_{-1.6}$&&$88.0^{+3.2}_{-2.6}$&&$126^{+8}_{-1}$&&$163^{+7}_{-4}$&&${}_{ 1.95\pm 0.05}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$9.92^{+0.30}_{-0.27}$&&$16.7^{+0.7}_{-0.5}$&&$22.3^{+0.8}_{-0.6}$&&$30.3^{+1.2}_{-0.7}$&&$43.2^{+1.9}_{-1.5}$&&$48.6^{+2.4}_{-1.3}$&&$49.5^{+2.1}_{-1.5}$&&${}_{ 1.54\pm 0.04}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$5.85^{+0.14}_{-0.17}$&&$8.80^{+0.27}_{-0.23}$&&$13.1^{+0.5}_{-0.3}$&&$15.6^{+0.6}_{-0.4}$&&$23.3^{+0.9}_{-0.6}$&&$28.6^{+1.2}_{-0.9}$&&$28.6^{+1.4}_{-1.0}$&&${}_{ 1.54\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-2.40\pm 0.44}$&&${}_{-1.33\pm 0.12}$&&${}_{-1.53\pm 0.17}$&&${}_{-1.47\pm 0.08}$&&${}_{-1.29\pm 0.05}$&&${}_{-1.26\pm 0.12}$&&${}_{-1.32\pm 0.11}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTviii\xdef\BTviii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^6>_{Ws}$ from Raw Binned Data, Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$5720000$&&$391000$&&$1280000$&&$297000$&&$199000$&&$24900$&&$71700$&&${}_{-4.40\pm 0.39}$&\cr
&& &&${}^{+1370000}_{-510000}$&&${}^{+441000}_{+45000}$&&${}^{+720000}_{-180000}$&&${}^{+320000}_{-16000}$&&${}^{+295000}_{-23000}$&&${}^{+13600}_{-3800}$&&${}^{+112000}_{-7300}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$1880000$&&$1830$&&$3710$&&$5150$&&$6180$&&$42800$&&$2640$&&${}_{-2.87\pm 1.05}$&\cr
&& &&${}^{+970000}_{-20000}$&&${}^{+260}_{-170}$&&${}^{+640}_{-330}$&&${}^{+700}_{-560}$&&${}^{+1300}_{-980}$&&${}^{+41100}_{-2700}$&&${}^{+2570}_{-1400}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$289^{+44}_{-29}$&&$380^{+47}_{-47}$&&$1260^{+210}_{-140}$&&$2160^{+510}_{-160}$&&$939^{+312}_{-210}$&&$1660^{+880}_{+50}$&&$968^{+686}_{-399}$&&${}_{ 1.82\pm 0.26}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$109^{+15}_{-12}$&&$167^{+40}_{-24}$&&$110^{+29}_{-27}$&&$98.0^{+79.2}_{-43.7}$&&$285^{+127}_{-81}$&&$77.5^{+161.1}_{-61.2}$&&$-625^{+111}_{-94}$&&${}_{ 0.44\pm 0.25}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$27.1^{+3.7}_{-3.2}$&&$48.2^{+7.9}_{-7.9}$&&$39.4^{+15.0}_{-11.8}$&&$-19.7^{+26.3}_{-18.2}$&&$-65.2^{+34.7}_{-27.2}$&&$-213^{+44}_{-36}$&&$-125^{+67}_{-45}$&&${}_{ 1.06\pm 0.14}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-5.57\pm 0.98}$&&${}_{-3.16\pm 0.55}$&&${}_{-3.95\pm 0.47}$&&${}_{-3.33\pm 0.37}$&&${}_{-3.15\pm 0.23}$&&${}_{-2.27\pm 0.82}$&&${}_{-2.98\pm 0.29}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip
}\endinsert

\goodbreak\pageinsert{
\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7{\DefWarn\CTi\xdef\BTi{table
\secsym\the\tableno}&&\multispan{13}\hfil {Table
\secsym\the\tableno: Power-Law Dependence of $<\phi^2>$ on $L_x$}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{13}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{13}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{Contour}{Data}{$\beta=8.25$}{$\beta=8.35$}{$\beta=8.50$}{$\beta=8.75$}{$\beta=9.00$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Lower}&&{\it Raw}&&${}_{ 1.30\pm 0.02}$&&${}_{ 1.22\pm 0.01}$&&${}_{ 1.13\pm 0.01}$&&${}_{ 1.04\pm 0.01}$&&${}_{ 1.02\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Lower}&&{\it Smooth}&&${}_{ 1.21\pm 0.02}$&&${}_{ 1.16\pm 0.02}$&&${}_{ 1.14\pm 0.02}$&&${}_{ 1.09\pm 0.01}$&&${}_{ 1.10\pm 0.01}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Middle}&&{\it Raw}&&${}_{ 1.20\pm 0.03}$&&${}_{ 1.21\pm 0.01}$&&${}_{ 1.15\pm 0.01}$&&${}_{ 1.05\pm 0.01}$&&${}_{ 1.03\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Middle}&&{\it Smooth}&&${}_{ 1.26\pm 0.01}$&&${}_{ 1.23\pm 0.01}$&&${}_{ 1.17\pm 0.01}$&&${}_{ 1.11\pm 0.01}$&&${}_{ 1.13\pm 0.01}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Higher}&&{\it Raw}&&${}_{ 0.91\pm 0.03}$&&${}_{ 1.08\pm 0.02}$&&${}_{ 1.04\pm 0.01}$&&${}_{ 0.92\pm 0.01}$&&${}_{ 0.89\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Higher}&&{\it Smooth}&&${}_{ 1.23\pm 0.01}$&&${}_{ 1.12\pm 0.01}$&&${}_{ 1.03\pm 0.01}$&&${}_{ 0.94\pm 0.01}$&&${}_{ 0.95\pm 0.01}$&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7{\DefWarn\CTii\xdef\BTii{table
\secsym\the\tableno}&&\multispan{13}\hfil {Table
\secsym\the\tableno: Power-Law Dependence of $<\phi^4>_{Ws}$ on $L_x$}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{13}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{13}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{Contour}{Data}{$\beta=8.25$}{$\beta=8.35$}{$\beta=8.50$}{$\beta=8.75$}{$\beta=9.00$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Lower}&&{\it Raw}&&${}_{ 0.27\pm 0.25}$&&${}_{ 1.84\pm 0.47}$&&${}_{ 1.99\pm 0.05}$&&${}_{ 1.58\pm 0.03}$&&${}_{ 1.51\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it Lower}&&{\it Smooth}&&${}_{-0.18\pm 0.15}$&&${}_{-0.11\pm 0.38}$&&${}_{ 1.65\pm 0.07}$&&${}_{ 1.21\pm 0.05}$&&${}_{ 1.19\pm 0.05}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Middle}&&{\it Raw}&&${}_{-0.54\pm 0.27}$&&${}_{ 1.31\pm 0.49}$&&${}_{ 1.95\pm 0.05}$&&${}_{ 1.54\pm 0.04}$&&${}_{ 1.54\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it Middle}&&{\it Smooth}&&${}_{-0.56\pm 0.17}$&&${}_{-0.02\pm 0.31}$&&${}_{ 1.68\pm 0.07}$&&${}_{ 1.17\pm 0.06}$&&${}_{ 1.27\pm 0.05}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Higher}&&{\it Raw}&&${}_{-1.01\pm 0.24}$&&${}_{ 0.88\pm 0.54}$&&${}_{ 1.62\pm 0.04}$&&${}_{ 1.32\pm 0.03}$&&${}_{ 1.28\pm 0.02}$&\cr
\tablelines\tablerule\tablelines
&&{\it Higher}&&{\it Smooth}&&${}_{ 0.08\pm 0.16}$&&${}_{ 0.24\pm 0.33}$&&${}_{ 1.36\pm 0.05}$&&${}_{ 1.06\pm 0.04}$&&${}_{ 1.02\pm 0.03}$&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7{\DefWarn\CTiii\xdef\BTiii{table
\secsym\the\tableno}&&\multispan{13}\hfil {Table
\secsym\the\tableno: Power-Law Dependence of $<\phi^6>_{Ws}$ on $L_x$}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{13}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{13}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{Contour}{Data}{$\beta=8.25$}{$\beta=8.35$}{$\beta=8.50$}{$\beta=8.75$}{$\beta=9.00$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Lower}&&{\it Raw}&&${}_{-4.38\pm 0.24}$&&${}_{ 0.04\pm 1.18}$&&${}_{ 1.60\pm 0.29}$&&${}_{ 0.73\pm 0.17}$&&${}_{-0.52\pm 0.11}$&\cr
\tablelines\tablerule\tablelines
&&{\it Lower}&&{\it Smooth}&&${}_{-1.62\pm 0.20}$&&${}_{-5.38\pm 1.17}$&&${}_{ 1.19\pm 0.32}$&&${}_{ 1.02\pm 0.09}$&&${}_{ 0.90\pm 0.08}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Middle}&&{\it Raw}&&${}_{-4.40\pm 0.39}$&&${}_{-2.87\pm 1.05}$&&${}_{ 1.82\pm 0.26}$&&${}_{ 0.44\pm 0.25}$&&${}_{ 1.06\pm 0.14}$&\cr
\tablelines\tablerule\tablelines
&&{\it Middle}&&{\it Smooth}&&${}_{-2.55\pm 0.24}$&&${}_{-5.29\pm 1.10}$&&${}_{ 1.66\pm 0.22}$&&${}_{ 0.92\pm 0.08}$&&${}_{?\pm?}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Higher}&&{\it Raw}&&${}_{-4.40\pm 0.39}$&&${}_{-3.69\pm 0.99}$&&${}_{ 1.54\pm 0.27}$&&${}_{ 0.94\pm 0.26}$&&${}_{ 0.60\pm 0.19}$&\cr
\tablelines\tablerule\tablelines
&&{\it Higher}&&{\it Smooth}&&${}_{-2.60\pm 0.19}$&&${}_{-4.14\pm 0.86}$&&${}_{ 1.56\pm 0.18}$&&${}_{ 1.21\pm 0.10}$&&${}_{ 1.03\pm 0.07}$&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip
}\endinsert

\ifig\IIIFxv{Graphs of even moments against transverse size,
$L_x$, for $\beta=8.5$. Data are shown for both raw
(unprocessed) and smoothed Polyakov configurations. For the 4th and
6th moments, the left-hand graphs are as measured initially; the
right-hand ones are Wick-subtracted.}
{\epsfxsize\hsize \epsfbox{w1.ps}}

\ifig\IIIFxvi{Log plots corresponding to the Wick-subtracted data of
\IIIFxv, with best fits to a power-law dependence on the lattice width.}
{\epsfxsize\hsize \epsfbox{w1l.ps}}

A typical set of results is shown in \IIIFxv, showing the dependence
of $<\bar{\phi(x)^n}>$ on the lattice width (interface length), $L_x$,
for a particular value of $\beta$.
Both raw and smoothed data
are shown, and these are in good qualitative agreement, though there
is a small quantitative difference between them.
In \IIIFxvi, we obtain best estimates for the power-law dependences of
the even Wick-subtracted moments on the lattice width. These are displayed
in the graphs, matching the values given in the earlier tables, and
show reasonable agreement with our theoretical predictions for the
2nd and 4th moments. The agreement is distinctly less good for the
6th, but the nature of this Wick-subtracted moment, the small difference
between two large numbers derived from powers of a fluctuation, may
go a long way towards explaining this discrepancy.
Our results are similar for the other values of $\beta$, as shown in
tables 4.12-14. Though not in perfect agreement with our predictions
for the higher moments, these measurements
encourage us to believe that our toy Lagrangian
is a reasonable model for the interface behaviour.

It should further be pointed out that some of the results at low
$\beta$ and small $L_x$ seem to suffer from anomalous large ``spikes'' in
the data, which can skew the estimates of the higher moments severely, and
with them the slopes. This problem is addressed at the end of the next
chapter, and oddities such as the negative slopes of the higher
moments against $L_x$ for small $\beta$ then disappear from the
corrected results given there.

\goodbreak\pageinsert{
\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\CTi\xdef\BTi{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Power-Law Dependence of $<\phi^2>$ on $(\beta-\beta_c)$}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{Contour}{Data}{$L_x=18$}{$L_x=24$}{$L_x=30$}{$L_x=36$}{$L_x=42$}{$L_x=48$}{$L_x=54$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Lower}&&{\it Raw}&&${}_{-0.33\pm 0.02}$&&${}_{-0.32\pm 0.02}$&&${}_{-0.39\pm 0.02}$&&${}_{-0.40\pm 0.03}$&&${}_{-0.41\pm 0.01}$&&${}_{-0.42\pm 0.02}$&&${}_{-0.44\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it Lower}&&{\it Smooth}&&${}_{-0.51\pm 0.03}$&&${}_{-0.46\pm 0.03}$&&${}_{-0.51\pm 0.03}$&&${}_{-0.50\pm 0.03}$&&${}_{-0.50\pm 0.02}$&&${}_{-0.51\pm 0.02}$&&${}_{-0.53\pm 0.03}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Middle}&&{\it Raw}&&${}_{-0.41\pm 0.01}$&&${}_{-0.37\pm 0.02}$&&${}_{-0.44\pm 0.02}$&&${}_{-0.43\pm 0.03}$&&${}_{-0.44\pm 0.02}$&&${}_{-0.45\pm 0.03}$&&${}_{-0.46\pm 0.04}$&\cr
\tablelines\tablerule\tablelines
&&{\it Middle}&&{\it Smooth}&&${}_{-0.50\pm 0.03}$&&${}_{-0.48\pm 0.03}$&&${}_{-0.54\pm 0.03}$&&${}_{-0.52\pm 0.04}$&&${}_{-0.52\pm 0.02}$&&${}_{-0.53\pm 0.03}$&&${}_{-0.56\pm 0.03}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Higher}&&{\it Raw}&&${}_{-0.41\pm 0.03}$&&${}_{-0.37\pm 0.02}$&&${}_{-0.42\pm 0.02}$&&${}_{-0.39\pm 0.03}$&&${}_{-0.40\pm 0.02}$&&${}_{-0.41\pm 0.03}$&&${}_{-0.42\pm 0.04}$&\cr
\tablelines\tablerule\tablelines
&&{\it Higher}&&{\it Smooth}&&${}_{-0.40\pm 0.03}$&&${}_{-0.42\pm 0.03}$&&${}_{-0.47\pm 0.03}$&&${}_{-0.48\pm 0.03}$&&${}_{-0.49\pm 0.02}$&&${}_{-0.51\pm 0.02}$&&${}_{-0.54\pm 0.03}$&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\CTii\xdef\BTii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Power-Law Dependence of $<\phi^4>_{Ws}$ on $(\beta-\beta_c)$}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{Contour}{Data}{$L_x=18$}{$L_x=24$}{$L_x=30$}{$L_x=36$}{$L_x=42$}{$L_x=48$}{$L_x=54$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Lower}&&{\it Raw}&&${}_{-2.00\pm 0.43}$&&${}_{-1.25\pm 0.10}$&&${}_{-1.40\pm 0.06}$&&${}_{-1.23\pm 0.08}$&&${}_{-1.19\pm 0.04}$&&${}_{-1.24\pm 0.10}$&&${}_{-1.29\pm 0.11}$&\cr
\tablelines\tablerule\tablelines
&&{\it Lower}&&{\it Smooth}&&${}_{-2.69\pm 0.34}$&&${}_{-1.63\pm 0.15}$&&${}_{-1.84\pm 0.14}$&&${}_{-1.67\pm 0.10}$&&${}_{-1.54\pm 0.06}$&&${}_{-1.65\pm 0.12}$&&${}_{-1.76\pm 0.11}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Middle}&&{\it Raw}&&${}_{-2.40\pm 0.44}$&&${}_{-1.33\pm 0.12}$&&${}_{-1.53\pm 0.17}$&&${}_{-1.47\pm 0.08}$&&${}_{-1.29\pm 0.05}$&&${}_{-1.26\pm 0.12}$&&${}_{-1.32\pm 0.11}$&\cr
\tablelines\tablerule\tablelines
&&{\it Middle}&&{\it Smooth}&&${}_{-2.76\pm 0.25}$&&${}_{-1.80\pm 0.17}$&&${}_{-1.88\pm 0.17}$&&${}_{-1.74\pm 0.10}$&&${}_{-1.61\pm 0.04}$&&${}_{-1.62\pm 0.13}$&&${}_{-1.82\pm 0.11}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Higher}&&{\it Raw}&&${}_{-2.33\pm 0.52}$&&${}_{-1.20\pm 0.25}$&&${}_{-1.33\pm 0.24}$&&${}_{-1.21\pm 0.07}$&&${}_{-1.11\pm 0.05}$&&${}_{-1.18\pm 0.07}$&&${}_{-1.26\pm 0.06}$&\cr
\tablelines\tablerule\tablelines
&&{\it Higher}&&{\it Smooth}&&${}_{-2.28\pm 0.34}$&&${}_{-1.44\pm 0.13}$&&${}_{-1.38\pm 0.15}$&&${}_{-1.43\pm 0.05}$&&${}_{-1.34\pm 0.04}$&&${}_{-1.45\pm 0.06}$&&${}_{-1.50\pm 0.02}$&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\CTiii\xdef\BTiii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Power-Law Dependence of $<\phi^6>_{Ws}$ on $(\beta-\beta_c)$}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{Contour}{Data}{$L_x=18$}{$L_x=24$}{$L_x=30$}{$L_x=36$}{$L_x=42$}{$L_x=48$}{$L_x=54$}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Lower}&&{\it Raw}&&${}_{-4.99\pm 1.05}$&&${}_{-3.49\pm 0.57}$&&${}_{-4.08\pm 0.37}$&&${}_{-3.11\pm 0.38}$&&${}_{-2.75\pm 0.12}$&&${}_{-1.98\pm 0.47}$&&${}_{-3.00\pm 0.32}$&\cr
\tablelines\tablerule\tablelines
&&{\it Lower}&&{\it Smooth}&&${}_{-5.40\pm 0.94}$&&${}_{-3.30\pm 0.47}$&&${}_{-3.96\pm 0.37}$&&${}_{-3.25\pm 0.48}$&&${}_{-3.45\pm 0.33}$&&${}_{-3.47\pm 0.51}$&&${}_{-3.55\pm 0.22}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Middle}&&{\it Raw}&&${}_{-5.57\pm 0.98}$&&${}_{-3.16\pm 0.55}$&&${}_{-3.95\pm 0.47}$&&${}_{-3.33\pm 0.37}$&&${}_{-3.15\pm 0.23}$&&${}_{-2.27\pm 0.82}$&&${}_{-2.98\pm 0.29}$&\cr
\tablelines\tablerule\tablelines
&&{\it Middle}&&{\it Smooth}&&${}_{-5.78\pm 0.92}$&&${}_{-3.35\pm 0.59}$&&${}_{-3.79\pm 0.52}$&&${}_{-3.24\pm 0.32}$&&${}_{-3.39\pm 0.25}$&&${}_{?\pm?}$&&${}_{-3.71\pm 0.17}$&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&{\it Higher}&&{\it Raw}&&${}_{-5.36\pm 1.01}$&&${}_{-2.22\pm 0.67}$&&${}_{-2.58\pm 0.70}$&&${}_{-2.39\pm 0.24}$&&${}_{-1.99\pm 0.07}$&&${}_{-2.36\pm 0.23}$&&${}_{-2.85\pm 0.11}$&\cr
\tablelines\tablerule\tablelines
&&{\it Higher}&&{\it Smooth}&&${}_{-5.25\pm 0.99}$&&${}_{-2.74\pm 0.43}$&&${}_{-2.43\pm 0.57}$&&${}_{-2.44\pm 0.22}$&&${}_{-2.29\pm 0.10}$&&${}_{-2.46\pm 0.17}$&&${}_{-2.36\pm 0.19}$&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip
}\endinsert

\ifig\IIIFxvii{Graphs of even moments against $\beta$,
for $L_x=36$. Data are shown for both raw
(unprocessed) and smoothed Polyakov configurations. For the 4th and
6th moments, the first graphs are as measured by the computer, and the
second graphs are Wick-subtracted.}
{\epsfxsize\hsize \epsfbox{l1.ps}}

Having obtained reasonable results for our model, we now turn to the
question of the unknown functions, $\gamma$ and $\lambda$. To tell
anything about these functions, we need to produce similar plots to
\IIIFxv\ and \IIIFxvi, but showing the dependence on $\beta$ instead
of $L_x$. 
In \IIIFxvii, we show the divergence of the non-Wick-subtracted even
moments as $\beta\rightarrow\beta_c$. The data shown are for lattices
with $L_x=36$. To find the degree of divergence, we need to fit this
behaviour to a power law dependence on $(\beta-\beta_c)$.

\ifig\IIIFxviii{Log plots corresponding to the Wick-subtracted data of
\IIIFxvii, with best fits to a power-law dependence on $(\beta-\beta_c)$.}
{\epsfxsize\hsize \epsfbox{l1l.ps}}

In \IIIFxviii, we fit our results to just such a power-law divergence,
taking $\beta_c=8.175$.
We obtain good fits even for the sixth moment, giving another
indication that our model is reasonable.
For the data shown in the graphs of this chapter ($L_x=36$, middle
contour, raw data), the fitted slopes for the
second, fourth and sixth moments are:
$$<\phi^2>\sim(\beta-\beta_c)^{-0.43(3)},\quad
<\phi^4>_{Ws}\sim(\beta-\beta_c)^{-1.47(8)},\quad
<\phi^6>_{Ws}\sim(\beta-\beta_c)^{-3.33(37)}.$$
Referring back to our formulae for the moments, we see that the
first two imply the following for our unknown functions of $\beta$:
$$\gamma\sim (\beta-\beta_c)^{0.43(3)},\qquad \lambda\sim
(\beta-\beta_c)^{0.25(14)}.$$ 
These two together predict, from our previous formulae, that 
$$<\phi^6>_{Ws}\sim(\beta-\beta_c)^{-2.51(21)},$$ within roughly one
standard deviation of the observed behaviour. Our other sets of data give
similar results for $\gamma$ and $\lambda$.

It can be seen from the tables that the different contours give
similar results, as hoped. For this reason, we use the middle contour,
as it should be less susceptible to the influence of nearby bubbles of
phase. Also, the results after smoothing are close to those from the
raw data, but the discrepancies increase for the higher
moments. Smoothing appears to be a useful technique for keeping track
of the interface at low $\beta$, indeed lower $\beta$ than is possible
in its absence. It appears not to alter the results significantly for
the lower moments, though the discrepancies increase fast enough for
the results to disagree somewhat with the unprocessed results over the
higher moments.

\subsec{Interface Width: Intrinsic \& Screening}
In addition to our survey of fluctuation moments, we also measure
the Debye electric screening mass and interface width for each value
of $\beta$ and $L_x$,
as illustrated in \IIIFix. As touched on previously, we can measure
the ``intrinsic'' width of the interface by taking the distance
between the lower and upper contours at every point across the
lattice, and then averaging this quantity across the lattice, and then
over all sweeps. By contrast, we obtain the screening mass by
averaging the transverse-averaged Polyakov profile of the interface,
obtained after each sweep, over all sweeps, and fitting the resulting
function to a $\tanh$ with coefficient proportional to the Debye
mass. The inverse of this mass is the Debye screening length, giving
the screening width of the interface, in contrast to the intrinsic
width mentioned before.

\ifig\IIIFxxiii{Measurements of the average
interface width in units of the lattice spacing. For reasons of
accuracy, twice the half-width (the average separation of the 25\% and
50\% contours) is plotted rather than the width (25\%---75\%).
This remains roughly constant as the width of the lattice
increases, and rises somewhat as the temperature
drops.}{\epsfxsize\hsgraph \epsfbox{wallwidths.ps}}

We can return to our picture of the interface as a string. The intrinsic
width is the width of the string itself, which should be independent
of the length of the string ($L_x$), and which we would not expect to
change much with temperature. To visualise the screening width, however,
we need to imagine letting the string fluctuate very fast while we
look at it, so that the different shapes blur into one another; at
very high temperatures, where the fluctuations are suppressed, this
blurred string should look only a little wider than the stationary
string, but as the temperature drops and the fluctuations diverge, we
expect the blurred string to appear wider and wider, also diverging in
width towards the critical temperature. Since the mean square
fluctuations (the second moments) grow like $L_x$, we might expect the
screening width of the interface to grow like $\sqrt{L_x}$.

The results for the intrinsic width, shown in \IIIFxxiii, show that
the width does indeed remain constant as $L_x$ increases, and that it
increases only moderately as $\beta\rightarrow\beta_c$. Presumably, this
increase is due to the less rigid shape of the interface as the energy
penalty drops.

\ifig\IIIFxxii{Measurements of the Debye screening length for each
value of ($\beta, L_x$), showing a roughly linear dependence on $L_x$.}
{\epsfxsize\hsgraph \epsfbox{deb_mass.ps}}

\ifig\IIIFxxiia{Measurements of the Debye screening length
for each value of ($\beta, L_x$), showing a mild divergence as
$\beta\rightarrow\beta_c$, which we fit to a curve of the form
$a+b\ln(\beta-\beta_c)$ for each $L_x$.}{\epsfxsize\hsgraph \epsfbox{deb_mass2.ps}}

Our results for the Debye screening length are shown in \IIIFxxii\ and
\IIIFxxiia. Rather surprisingly, the best fit is for a linear
dependence on $L_x$, with a constant term to which it tends at very
high temperatures when the interface is rigid. The length also appears
to diverge somewhat as $\beta\rightarrow\beta_c$, as expected. The best
fit of this divergence is to a curve of the form
$a+b\ln(\beta-\beta_c)$ for each $L_x$, as predicted for completely
wet $Z(3)$ interfaces in $3+1$ dimensions\IIIRii.

\supereject

\subsec{Critical Acceleration of the Random Walk}
As a curiosity, we can also measure the speed of the random walk of the
interface near the critical temperature if we turn off the mechanism
that constantly re-centres the interface. As the temperature drops and
more and larger bubbles of phase froth within the main phase domains,
the interface will combine with, and bud off, more and more of these
bubbles. Therefore, we would expect it to wander more and more rapidly
along the lattice, moving in bursts as it merges with bubbles in ``front''
of it or buds off bubbles ``behind'' it.

\ifig\IIIFxxiv{This shows the random wandering of the
interface, for temperatures near the critical temperature, over 40k
sweeps after an initial 400 heat-bath sweeps.}
{\epsfxsize\hsgraph \epsfbox{randomwalk2.ps}}

In \IIIFxxiv, we do indeed see an increase in speed as the
temperature drops. In fact, in common with many other parameters, the
speed appears to diverge as $\beta\rightarrow\beta_c$. Of course, it
could be argued that this is simply an artefact of the Monte-Carlo
heatbath algorithm, with no relevance to a ``real'' interface at
all. In the absence of a physical ``time'' to measure and use as a yardstick in
the Monte-Carlo procedure, the best way to test this hypothesis would
seem to be to to examine the behaviour
of the interface under another Monte-Carlo scheme, with
different autocorrelation behaviour as $\beta$ drops; we do not do
this here.

\ifig\IIIFxxv{This uses the divergence of the speed of the random walk
in \IIIFxxiv\ to estimate the critical temperature and exponent of divergence.}
{\epsfxsize\hsgraph \epsfbox{rw_exponent.ps}}

In \IIIFxxv, we fit the speed to a function of the
form
$$\frac{\del z^2}{\del t} \sim (\beta-\beta_c)^{\beta_{RW}}.$$
Our results suggest values of
$$\beta_c=8.14(3),\qquad \beta_{RW}=-0.71(6).$$
This value for $\beta_c$ is certainly consistent with our previous
estimates, and the dynamical exponent governing the critical
acceleration of the random walk is given by $\beta_{RW}$.

\subsec{Interface Equilibration}
It is interesting to note that studies of discrete
models\ref\IIIRiii{F.~Family and T.~Vicsek, \JP{A18}{1985}{L75};
F.~Family, \JP{A19}{1986}{L441}; P.~Meakin, P.~Ramanlal, L.~M.~Sander
and R.~C.~Ball, \PR{A34}{1986}{5091}; J.~M.~Kim and J.~M.~Kosterlitz,
\PRL{62}{1989}{2289}} and
continuum growth equations\ref\IIIRiv{S.~F.~Edwards and D.~R.~Wilkinson,
{\it Proc. R. Soc., London}, \vyp{A381}{1982}{17}; M.~Kardar, G.~Parisi
and Y.-C.~Zhang, \PRL{56}{1986}{889}} in condensed matter make predictions for
the behaviour of the width of an interface.
The ``width'' here is usually defined to be the square-root of our
second moment,
$$W(L_x,t)=\sqrt{\bar{\phi^2}-{\bar\phi}^2},$$
where $t$ is the time since formation of the interface (initial width
zero).

Models generally predict that for times much smaller than some
critical time, $t_X(L_x)$, determined by the interface size, an
exponent $\beta_G$ will govern the growth of the width:
$$W(t)\sim t^{\beta_G},\qquad t\ll t_X(L_x).$$
For times much larger than this, as might be expected, the width is
predicted to saturate at a value whose relationship to the interface
size is governed by $\alpha_G$, the roughness exponent:
$$W_{sat}(L_x)\sim L^{\alpha_G}.$$

\ifig\IIIFxxvi{An example of the growth in size of an interface for
$\beta=8.5, L_x=36$, and a growth profile averaged over all $L_x$ and
$\beta$. In each case, $\beta_G$ is estimated from the slope of the
dotted line.}
{\epsfxsize\hsize \epsfbox{growth.ps}}

For the $Z(3)$ interface, we have already seen behaviour corresponding
to the latter of these two, since
$$<\phi^2>\sim L_x^{1.13(1)}\Rightarrow \alpha_G=0.56(1).$$
It can be seen again in \IIIFxxvi, an example of the growth of a
$Z(3)$ interface. At high $t$, the size saturates as usual, but at low
$t$, we see growth governed by an exponent, as in the condensed matter
models. For our interface, the average profile yields
$$\beta_G=0.61(2).$$ This, again, could
be dismissed as an artefact of the simulation technique, but the
manner of formation simulated by the Monte-Carlo technique seems
eminently plausible for a ``real'' interface, and it is suggestive that
the interface shares many characteristics with more familiar
interfaces in condensed matter physics.

\vfill\supereject


==> quote1.tex <==
\def\quote#1#2{\footline={\hfil}\headline={\hfil} \centerline{\vbox{\vskip 2in\normalbaselines\halign{\hfil{\it ##}\hfil\cr #1\cr{\hfill\rm #2}\cr}}}}

{\headline={\hfil}
\quote{{\tenmsbm NESCIRE\ \ QUAEDAM\ \ MAGNA\ \ PARS\ \ SAPIENTAE\ \ EST}\cr}{Grotius}
\quote{For in much wisdom is much grief:\cr and he that increaseth
knowledge increaseth sorrow.\cr}{Ecclesiastes 1.18}
\quote{{\tenmsbm IMPOSSIBILIUM\ \ NULLA\ \ OBLIGATIO\ \ EST}\cr}{Celsus}
\supereject

%For single-sided, comment out this line
\vbox to\vsize{}\supereject 

\pageno=1
\headline={\tenrm \iftitlepage \hfil
\else \ifblankpage \hfil \folio
\else {\it Chapter \the\secno: \quad \chap} \hfil
\folio \fi \fi}
\footline={\tenrm \iftitlepage \hfil\folio\hfil
\global\titlepagefalse
\else \hfil \fi}

==> quote2.tex <==
\def\quote#1#2{\footline={\hfil}\headline={\hfil} \centerline{\vbox{\vskip 2in\normalbaselines\halign{\hfil{\it ##}\hfil\cr #1\cr{\hfill\rm #2}\cr}}}}

{\headline={\hfil}
\quote{{\tenmsbm IUCUNDI\ \ ACTI\ \ LABORES}\cr}{Cicero}
\quote{pltlh!\cr}{(Klingon saying)}
\supereject

%For single-sided, comment out this line
\vbox to\vsize{}\supereject 


==> statistics.tex <==
\newsec{Statistical Discussion:}{Bootstrap Techniques}

\Subsec{The Bootstrap}
Since it is not clear that the Wick-subtracted moments will be
normally distributed, we need a reliable method to construct
confidence intervals for them which does not rely on our knowing their
distribution at the start. A suitable method is given by the
``bootstrap'' principle\ref\RIVi{B.~Efron and R.~J.~Tibshirani, {\it
``An Introduction to the Bootstrap''}, Chapman and Hall, London
(1993); J.~R.~Carpenter, {\it ``Simulated Confidence Intervals for
Parameters in Epidemiological Models''}, D. Phil thesis,
University of Oxford (1996)},
and we now discuss some aspects of it as applied to our analysis.

Let $\vx=(x_1,x_2,\ldots,x_n)$ be a vector of samples from a normal
distribution with unknown mean and variance. Further, sample the random
variable $T$ from the t-distribution with $n-1$ degrees of freedom, and
define the quartile $t_{n-1,\alpha}$, shortened in future to
$t_\alpha$, by $\hbox{Prob}(T\leq t_\alpha)=\alpha$. If $\bar x_n$ and
$s_n^2$ are the sample mean and variance, then
$$(\bar x_n + s_nt_{0.975}\quad,\quad \bar x_n-s_nt_{0.025})$$
is the shortest unbiased exact 95\% confidence interval for the
mean. To obtain the standard deviation (a 68\% confidence interval for
the normal distribution), we simply change the subscripts on $t$ to
0.84 and 0.18.

How, then, can we construct confidence intervals for an unknown
distribution? This is where the bootstrap principle comes to our aid,
as it enables us, as its name suggests, to estimate confidence
intervals just from our observed data, with no prior knowledge of the
distribution. Let us denote the population
parameter, in our case corresponding to one of the moments, by
$\theta$. Given a random sample from the population,
$\vx$, we should like to be able to
construct an estimate, $\hat\Theta\equiv\hat\theta(\vx)$, for
$\theta$. The idea of 
the bootstrap is to learn about the relationship between $\theta$ and
$\hat\theta(\vx)$ by examining that between
$\hat\theta\equiv\hat\theta(\vx_{obs})$ 
and $\hat\theta(\vx^*)$, where $\vx^*$ is a resample with replacement
from the observed data, $\vx_{obs}$ (our results for the particular
moment). This is known as the ``nonparametric bootstrap''.

In the simplest case, we choose to consider the statistic
$W=\hat\Theta-\theta$, invoking the bootstrap principle to estimate its
quantiles by those of $W^*=\hat\Theta^*-\hat\theta$. We follow the
procedure given here: 

\item{$\bullet$} Fix $\theta$ at the value given by
$\hat\theta\equiv\hat\theta(\vx_{obs})$;

\item{$\bullet$} Sample with replacement from $\vx_{obs}$ to obtain
$\vx^*$;

\item{$\bullet$} From this, make an estimate of
$\hat\theta(\vx_{obs})$, denoted $\hat\theta^*\equiv\hat\theta(\vx^*)$;


\item{$\bullet$} Repeat the previous steps $(m-1)$ times to obtain $m$
estimates for $\hat\theta(\vx_{obs})$;

\item{$\bullet$} Sort the $\hat\theta^*$ into order, denoting the $p$th
ordered estimate by $\hat\theta^*_{(p)}$;

\item{$\bullet$} The $100(1-\alpha)$th percentile of the distribution
of $W^*$ is now consistently estimated by
$\hat\theta^*_{1-\alpha}-\hat\theta$, where we define
$\hat\theta^*_{1-\alpha} = \hat\theta^*_{(p)}$, choosing $m$ so that
$p=m(1-\alpha)$ is an integer.

\noindent It then follows
that the approximate 95\% confidence interval so obtained
is $$(2\hat\theta - \hat\theta^*_{0.975}\quad,\quad 2\hat\theta - \hat\theta^*_{0.025}).$$
There are two approximations behind this. The first is that
$\hat\theta^*_\alpha-\hat\theta$ is a consistent estimate of
$w^*_\alpha$, where $\hbox{Prob}(W^*\leq w^*_\alpha)=\alpha$, and can
be reduced as desired by increasing the number of resamplings,
$m$. The second relies on $W$ having the same distribution as $W^*$,
and will be true if the distribution of $W$ is pivotal, {\it i.e.}
depends on no unknown parameters. Unfortunately, a sizeable error may
be introduced if this is not the case.

\subsec{The Bootstrap t}
To overcome this problem, we need to make the statistic $W$ more
accurately pivotal. Such modification is suggested by considering a
sample $\vx=(x_1,\ldots,x_n)$ from normal distribution with mean
$\theta$ and variance $\sigma^2$. The
distribution of $\bar x-\theta$, our previous choice of
$W$, depends on $\sigma^2$, and is hence non-pivotal. However,
introducing the sample variance, $s^2=\frac{1}{n-1}\sum^n_{i=1} (x_i-\bar
x)^2$, we can see that the distribution of $\sqrt n(\bar x-\theta)/s$
{\it is} pivotal, following a $t$ distribution with $(n-1)$ degrees of
freedom. Thus, we ``studentise'' our previous $W$: we divide by an
estimate of the standard error of $\hat\Theta$, giving a new statistic:
$$T=\frac{\hat\Theta-\theta}{s(\hat\Theta)}.$$
Using $T$, we proceed exactly as for $W$, invoking the bootstrap
principle to estimate the quantiles by those of
$$T^*=\frac{\hat\Theta^*-\theta}{s(\hat\Theta^*)},$$
and finding the 95\% confidence interval to be
$$(\hat\theta-s(\hat\theta)\hat
t^*_{0.975}\quad,\quad\hat\theta-s(\hat\theta)\hat t^*_{0.025}).$$
The approximations are as before, but the error associated with the
pivotal quality of the statistic should be much reduced.
It has been
shown, in fact\ref\RIVii{P.~Hall, {\it ``The Bootstrap and Edgeworth
Expansion''}, Springer-Verlag, London (1992)}, that the coverage
error of the interval reduces from $O(n^{-0.5})$ to $O(n^{-1})$ for
many cases. If $T$ is
truly pivotal, the error will reduce to zero.

\subsec{The Non-Parametric Delta Method}
For our purposes, there is an added complication: whilst we can
calculate the sample variance for the second moment,
$\bar{\phi^2}$, in the usual manner, the form of the Wick subtraction
in $\bar{\phi^4_{Ws}}$ and $\bar{\phi^6_{Ws}}$ makes it impossible to
use a similar formula for them. Fortunately, a variance approximation
exists for many general statistics $T$ which can take the
representation $\theta=t(F)$. In this case, $F$ is the 
cumulative distribution function $F$ (the integral of the probability
density function) for a distribution ${\bf X}$. If the sample data is
denoted by the usual vector $\vx$, then a simple example would be the
mean of ${\bf X}$, given by $t(F)=\int x dF(x).$

The method works by applying aa Taylor expansion to $t(F)$:
$$t(G)=t(F)+\int L_t(x;F)dG(x).$$
$L_t$ gives the first derivative of $t$ at $F$ in direction $G$, and
is sometimes called the ``influence function'':
$$L_t(x;F)=\mathrel{\lim\limits_{\epsilon\rightarrow 0}}
\frac{t((1-\epsilon)F+\epsilon H_x)-t(F)}{\epsilon}=\frac{\del
t((1-\epsilon)F+\epsilon H_x)}{\del\epsilon}\bigg |_{\epsilon=0}.$$
Here, $H_x(y)$ is the Heaviside step function, stepping from 0 to 1 at
$y=x$. The empirical approximations given by the data values,
$l_i=L_t(x_i,\hat F)$, are the ``empirical influence values''.
The ``nonparametric delta method'' relies on applying this
approximation with $G=\hat F$, so that
\eqn\EIVii
{t(\hat F)=t(F)+\frac{1}{n}\sum_{i=1}^{n}L_t(x_i).}
Now, the difference, $(T-\theta)$, between $t(F)$ and $t(\hat F)$ will follow a
normal distribution, by the central limit theorem, with mean zero
and variance,
$$\nu_L(F)=\frac{1}{n}\int L_t^2(x) dF(x).$$ We approximate $\nu_L(F)$
by the sample version,
\eqn\EIViii
{\nu_L(\hat F)=\frac{1}{n^2}\sum_{i=1}^{n} l_i^2,}
the ``nonparametric delta method variance estimate''. Note that
subsitution of $\hat F$ for $F$ in \EIVii\ implies that $\sum_i l_i=0$.
For our purposes, we also note that we can use the chain rule for
statistics which are functions of others, $t(F)=\CT
\{t_1(f),\ldots,t_m(F)\},$ yielding
$$L_t(x)=\sum_{i=1}{m}\frac{\del\CT}{\del t_i}L_{t_i}(x).$$

Let us consider the three even moments, denoting the population means
of the {\it unsubtracted} moments by $\mu_2$, $\mu_4$ and $\mu_6$
respectively. First, the second moment:
$$\eqalign{
t=\bar{x^2} \Rightarrow L_t(x)&=\del_\epsilon [(1-\epsilon)\mu_2 +
\epsilon x^2]|_{\epsilon=0}\cr
&=x^2-\mu_2 \cr
\Rightarrow l(x_i)&=(x_i^2-\bar{x^2}).}$$
Similarly, the unsubtracted fourth and sixth moments are:
$$\eqalign{
t=\bar{x^4} &\Rightarrow l(x_i)=(x_i^4-\bar{x^4})\cr
t=\bar{x^6} &\Rightarrow l(x_i)=(x_i^6-\bar{x^6}).}$$
Using the chain rule then allows us to calculate the empirical
influence values for the subtracted moments:
$$\eqalign{
t&=\bar{x^4}-3{\bar{x^2}}^2\cr
&\Rightarrow l(x_i)=(x_i^4-\bar{x^4})-6\bar{x^2}(x_i^2-\bar{x^2})\cr
t&=\bar{x^6}-15{\bar{x^2}}^3-15\bar{x^2}(\bar{x^4}-3{\bar{x^2}}^2)\cr
&\Rightarrow l(x_i)=(x_i^6-\bar{x^6})+90{\bar{x^2}}^2(x_i^2-\bar{x^2})
-15\bar{x^2}(x_i^4-\bar{x^4})-15\bar{x^4}(x_i^2-\bar{x^2}).}$$
In each case, the variance is estimated by \EIViii; also, as expected,
$\sum_i l(x_i)=0$.

Finally, then, we are able to construct confidence intervals for the
subtracted moments, and this is how we obtain the standard errors for
the fluctuation moments given in tables and graphs. For a full data
vector, $\vx$, of 100,000 values, approximately 2,000 resamplings,
$\vx^*$, are necessary.

\ifig\IVFi{Variance stabilisation in numerical second-level bootstrap
procedures, illustrated for ($\beta=8.75, L_x=36$). The left-hand plots
show the second-level standard
deviations $\sigma(\hat\theta)$, against the first-level estimates for the
average moment, $\hat\theta$, together with a fit to a smooth function. The
right-hand plots show $g(\hat\theta)$, the integral of the function
$\sigma(\hat\theta)^{-1}$. In this case, 200 second-level bootstraps are used,
though only 25---50 are needed for sufficiently accurate results.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{var_stab.ps}}

\subsec{Variance Stabilisation}
A check on the standard errors obtained in this way is provided by
using a numerical approach rather than \EIViii. To do this, we perform
a second-level bootstrap analysis on each resampled vector, $\vx^*$,
resampling each vector itself ($\ll 2,000$ times) to obtain
$\vx^{**}$. The sample variance of the second-level estimates of the
mean of the subtracted moment gives the standard deviation for the
``parent'' first-level estimate. To check for any correlation
between the mean and deviation of the first-level estimates, which
might skew the confidence intervals, we then
plot one against the other. If a trend is seen, we introduce
``variance stabilisation''\ref\RIViia{A.~C.~Davison and D.~V.~Hinkley,
{\it ``Bootstrap Methods''}, CUP, Cambridge (1996)},
as follows. A smooth curve is
fitted to the data, denoted by $\sigma(\hat\theta)$. We then construct a
compensating function by numerically integrating the inverse:
$$g(\hat\theta)=\int^{\hat\theta} \frac{1}{\sigma(y)} dy,$$
as illustrated in \IVFi\ for data from a $(\beta=8.75, L_x=36)$ run.
We rescale $g(\hat\theta)$ so that its mean and variance are the same as that
of the original data vector $\vx$, order it, and plot it against the
estimates $\hat\theta$. Then, we simply read off the values for
$\hat\theta$ which correspond to the desired percentiles in
$g(\hat\theta)$, giving the desired confidence interval (quoted for
95\%): $$(2\hat\theta-\hat\theta^*_{0.975}\quad,\quad
2\hat\theta-\hat\theta^*_{0.025}).$$

\ifig\IVFia{Q-Q plots comparing the different methods for obtaining
confidence intervals, using data for ($\beta=8.75,
L_x=36$). Horizontally, the plots refer to the second, fourth and sixth moments
respectively. Vertically, the upper plots are for the basic bootstrap,
the central ones for the bootstrap $t$, and the lower ones for
variance stabilisation. The dotted lines are those which would be
obtained for normally distributed data.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{qq_plots.ps}}

The best way to compare the validity of the different methods is to
construct ``Q-Q plots'', where the ordered bootstrap vectors are
plotted against quantiles of the standard normal distribution, as
illustrated in \IVFia. The dotted lines on these graphs show what
would be obtained by a normal distribution with mean and standard
deviation given by the relevant bootstrap vector. Thus, the most
reliable data is that which most closely matches the dotted line
over the desired confidence interval. The upper three and middle three
sets of plots show respectively that the bootstrap and bootstrap $t$
distributions are close to, but not quite, normal. The variance
stabilisation technique is designed to transform to a scale where the
variance is constant relative to the mean, and will therefore
compensate for any divergence from normality
in the bootstrap $t$ distribution; the lower three
plots are included merely to show that it does indeed produce
curves which compensate for the deviations from normality of the
bootstrap $t$ curves above.

As just mentioned, the intervals from variance
stabilisation are the most reliable, being produced from accurately
normal bootstrap $t$ distributions, but they differ little from
the bootstrap $t$ estimates for our data. As an example of this, the
following table lists the 95\% and 1-$\sigma$ confidence intervals for
$\beta=8.75$ and $L_x=36$, matching the data of \IVFia. Since the
variance stabilisation technique requires computationally intensive
second-level bootstrap analysis, we therefore use straight bootstrap $t$
intervals for our results.

\bigskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8{\DefWarn#1\xdef#1{table
\secsym\the\tableno}&&\multispan{11}\hfil {Table
\secsym\the\tableno: #2}\hfil&\cr \tableedge\tablerule\tablelines
&&\omit\hidewidth #3\hidewidth&&\omit\hidewidth #4\hidewidth&&
\omit\hidewidth #5\hidewidth&&\omit\hidewidth
#6\hidewidth&&\omit\hidewidth #7\hidewidth&&\omit\hidewidth #8\hidewidth&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{11}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{11}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=1em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{\VTi}{Estimates of Confidence Intervals}{Moment}{Technique}{95\%
(Lower)}{$\sigma$ (Lower)}{$\sigma$ (Upper)}{95\% (Upper)}
\tablelines\tablerule\tablegap\tablerule\tablelines
&&2nd&&Bootstrap&&6.269&&6.313&&6.396&&6.436&\cr
\tablelines\tablerule\tablelines
&&2nd&&Bootstrap $t$&&6.276&&6.314&&6.397&&6.442&\cr
\tablelines\tablerule\tablelines
&&2nd&&V. Stabilisation&&6.270&&6.316&&6.395&&6.437&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&4th&&Bootstrap&&28.43&&29.38&&31.30&&32.32&\cr
\tablelines\tablerule\tablelines
&&4th&&Bootstrap $t$&&28.47&&29.43&&31.34&&32.44&\cr
\tablelines\tablerule\tablelines
&&4th&&V. Stabilisation&&28.63&&29.46&&31.44&&32.38&\cr
\tablelines\tablerule\tablegap\tablerule\tablelines
&&6th&&Bootstrap&&-5.3&&42.1&&155.2&&214.5&\cr
\tablelines\tablerule\tablelines
&&6th&&Bootstrap $t$&&12.4&&48.8&&171.6&&257.8&\cr
\tablelines\tablerule\tablelines
&&6th&&V. Stabilisation&&15.7&&51.1&&167.1&&251.3&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\bigskip

\vfill\supereject

\ifig\IVFii{Correlations are given between interface contour shapes
separated by a certain number of sweeps, for $L_x=36$. A particular
correlation is
shown on the right, whilst approximately 4,000 such graphs are
averaged on the left, for four values of $\beta$. It is clear that the
correlation function drops to one half within approximately ten
sweeps, as illustrated on the left.}
{\epsfxsize\hsize \epsfbox{autoco.ps}}

\ifig\IVFiii{The bootstrap errors, both studentised (``bootstrap $t$'')
and non-studentised, are shown here for ($\beta=8.75, L_x=36$). On the
left, the $\pm\sigma$ bounds (68\% confidence intervals) are shown for
different binnings of the data; on the right, a logarithmic plot of
interval sizes against number of bins shows a linear dependence for
large numbers of bins, whose gradient gives the corresponding
power-law behaviour.}
{\epsfxsize\hsize \epsfysize\vsgraph \epsfbox{booterrors.ps}}

\subsec{Correlations and Data Bins}
In our simulations, we record the full 100k measurements for each raw, even
moment of the central (50\%) contour, but bin all data from other
contours, and all smoothed data, in groups of one thousand. Thus, we must
consider how to ensure that the standard errors are not distorted by
the binning used. In \IVFii, the correlation between two interface
contour shapes is given as a function of the number of sweeps
separating them,
and it is seen
to drop to less than one half after about ten sweeps. Therefore, bins
containing far fewer than ten samples may give results tainted by
unacceptably large correlations, leading to artificially small
errors, whereas those containing far more than ten will lose
some information, giving errors which are too large. Thus, we bin our
raw data for the central contour into bins of size ten before
calculating bootstrap errors.

Illustrated in \IVFiii\ are errors from the non-studentised
bootstrap analysis, and from the bootstrap $t$, with more differences
apparent between them for the higher moments. The graphs show the effect of
rebinning the raw moment data into bins of different size. We take the
full 100k measurements for each moment, and bin the results into groups
of between one and ten thousand. Whereas a random variable with normal
distribution would have obey a relationship of the form $\sigma\sim
(\hbox{number of bins})^{-0.5}$, the moment errors flatten off for
bins containing more than a few hundred measurements. For bins with fewer
items than this, an estimated power law dependence of $\sigma$ on the
number of bins is shown, and this enables us to trivially adjust the errors
obtained from our bins of size one thousand to those that would be
obtained from bins of size ten.

\subsec{Statistical Problems Near Criticality}
Our results for $\beta\geq 8.35$ show reasonable statistical distributions
for the moments over the 100k sweeps. However, those for $\beta=8.25$
and small $L_x$ occasionally contain ``spikes'', observations for the
moments which are far larger than we would expect, sometimes by
several magnitudes. This can be seen by comparing the distributions in
the following two sets of figures: the first, where $L_x=54$ and no
spikes are apparent; and the second, where $L_x=18$ and
spikes have given each distributions an artificially long, flat
upper tail. The spikes are unlikely to be caused by
wild fluctuations passing through the twist, since similar spikes are
not seen for wider lattices where
fluctuations are larger. It is most
likely that they are an artefact of the greater energetic instability
of the smaller interfaces at very low temperatures: if parts of the
interface collapse during interaction with nearby bubbles of phase,
the interface contour may briefly undergo a drastic distortion or
partial collapse, even appearing to
pass through the twist because of the change in
Polyakov values there.

\ifigp\IIIFxix{Illustrated on the left are the statistical distributions of
unsubtracted moments for $(\beta=8.25, L_x=54)$. The distributions
have long upper tails, as expected for moments of a roughly normal
distribution. To the right are the corresponding distributions of the
{\it logarithm} of the moments, each resembling a normal distribution.
The dashed vertical lines represent a suggested upper cut-off, as
discussed in the text.}
{\epsfxsize\hsize \epsfbox{54o_dist.ps}}

\ifigp\IIIFxx{The partners to \IIIFxix, with $(\beta=8.25, L_x=54)$, show
unexpectedly long, flat upper tails in the right-hand plots. The
effects of these tails can be eliminated by the use of a cut-off
defined in the same way as that in \IIIFxix.}
{\epsfxsize\hsize \epsfbox{18o_dist.ps}}

It is difficult to prevent the spikes occurring, but
they have a massively disproportionate effect on the overall averages,
especially for the higher moments. Thus, we would like to be able to
examine the data with the spikes removed. To do this, we impose an
upper cut-off on the statistical distributions, as illustrated by the
dashed lines in
\IIIFxix\ and \IIIFxx. To ensure that only the spikes are removed, we
need to define the cut-off in a statistically sensible manner. We
take it, for each distribution, to be the median plus 2.5 times the
interquartile range of the distribution of {\it logarithmic} values of
data, where the interquartile range is defined to run between the 25th and 75th
percentiles of the distribution. This ensures that the cut-off
corresponds only to the
upper tip (to be precise, the top 0.04\%) of a normal distribution 
overlaid on the right-hand plots of \IIIFxix\ and \IIIFxx, ensuring
that only data sets containing spikes are affected by the procedure.
The exact multiplier ``2.5'' can, of course, be varied, but we find
that a lower number ({\it e.g.} 2.0, cutting off 0.3\% of the
distribution), has too great an effect on the normal contribution to
the distributions, whereas a higher number ({\it e.g.} 3.0, cutting
off only 0.002\% of the normal distribution) permits too much
influence from the spikes.

\vfill\supereject

\subsec{Revised Moment Averages (Without Spikes)}
In this section, we give revised results for moment averages after the
removal of spikes as discussed, and then some plots for
comparison with those of the previous chapter. We quote revised
results only for the middle (50\%) contour and raw Polyakov data:

\medskip\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTi\xdef\BTi{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^2>$ from Raw Data (Corrected), Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$5.44^{+0.05}_{-0.04}$&&$8.09^{+0.06}_{-0.06}$&&$11.9^{+0.1}_{-0.1}$&&$14.3^{+0.1}_{-0.1}$&&$17.8^{+0.1}_{-0.1}$&&$20.8^{+0.2}_{-0.2}$&&$23.1^{+0.2}_{-0.2}$&&${}_{ 1.33\pm 0.02}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$4.52^{+0.03}_{-0.03}$&&$6.69^{+0.05}_{-0.05}$&&$9.13^{+0.07}_{-0.06}$&&$11.4^{+0.1}_{-0.1}$&&$13.4^{+0.1}_{-0.1}$&&$16.5^{+0.1}_{-0.1}$&&$18.2^{+0.1}_{-0.1}$&&${}_{ 1.27\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$3.93^{+0.03}_{-0.03}$&&$5.19^{+0.03}_{-0.03}$&&$7.17^{+0.05}_{-0.05}$&&$8.89^{+0.07}_{-0.06}$&&$10.0^{+0.1}_{-0.1}$&&$11.9^{+0.1}_{-0.1}$&&$13.8^{+0.1}_{-0.1}$&&${}_{ 1.15\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$3.06^{+0.02}_{-0.02}$&&$4.21^{+0.03}_{-0.03}$&&$5.32^{+0.04}_{-0.03}$&&$6.34^{+0.04}_{-0.04}$&&$7.62^{+0.05}_{-0.05}$&&$8.85^{+0.06}_{-0.06}$&&$9.57^{+0.06}_{-0.06}$&&${}_{ 1.05\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$2.62^{+0.02}_{-0.02}$&&$3.44^{+0.02}_{-0.02}$&&$4.38^{+0.03}_{-0.03}$&&$5.27^{+0.03}_{-0.03}$&&$6.29^{+0.04}_{-0.04}$&&$7.37^{+0.05}_{-0.05}$&&$7.89^{+0.05}_{-0.05}$&&${}_{ 1.03\pm 0.01}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.31\pm 0.03}$&&${}_{-0.36\pm 0.03}$&&${}_{-0.42\pm 0.03}$&&${}_{-0.42\pm 0.03}$&&${}_{-0.44\pm 0.02}$&&${}_{-0.45\pm 0.03}$&&${}_{-0.46\pm 0.04}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\medskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTiv\xdef\BTiv{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^4>_{Ws}$ from Raw Data (Corrected), Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$63.2^{+3.7}_{-3.0}$&&$115^{+7}_{-5}$&&$273^{+14}_{-11}$&&$326^{+9}_{-9}$&&$425^{+15}_{-14}$&&$580^{+14}_{-13}$&&$658^{+15}_{-15}$&&${}_{ 2.12\pm 0.07}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$30.6^{+1.0}_{-1.1}$&&$61.7^{+2.1}_{-2.0}$&&$108^{+3}_{-3}$&&$166^{+6}_{-5}$&&$197^{+6}_{-6}$&&$322^{+1}_{-1}$&&$299^{+10}_{-9}$&&${}_{ 2.17\pm 0.06}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$19.2^{+0.6}_{-0.5}$&&$27.8^{+0.8}_{-0.8}$&&$59.0^{+2.0}_{-1.8}$&&$82.0^{+2.8}_{-2.5}$&&$87.8^{+2.8}_{-2.8}$&&$126^{+5}_{-4}$&&$163^{+6}_{-5}$&&${}_{ 1.97\pm 0.05}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$9.68^{+0.34}_{-0.31}$&&$16.3^{+0.6}_{-0.6}$&&$22.3^{+0.7}_{-0.6}$&&$30.3^{+1.1}_{-1.0}$&&$43.0^{+2.2}_{-2.0}$&&$48.2^{+1.9}_{-1.7}$&&$49.7^{+1.9}_{-1.8}$&&${}_{ 1.55\pm 0.04}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$5.84^{+0.17}_{-0.16}$&&$8.76^{+0.25}_{-0.25}$&&$13.0^{+0.4}_{-0.4}$&&$15.6^{+0.6}_{-0.5}$&&$23.3^{+0.8}_{-0.8}$&&$28.6^{+1.1}_{-1.0}$&&$28.5^{+1.3}_{-1.0}$&&${}_{ 1.54\pm 0.03}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-0.99\pm 0.06}$&&${}_{-1.10\pm 0.07}$&&${}_{-1.28\pm 0.07}$&&${}_{-1.25\pm 0.11}$&&${}_{-1.21\pm 0.06}$&&${}_{-1.27\pm 0.11}$&&${}_{-1.28\pm 0.12}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\medskip

\boxit{
\vbox{\tabskip=0pt \offinterlineskip
\def\tabletitles#1#2#3#4#5#6#7#8#9{\DefWarn\BTvii\xdef\BTvii{table
\secsym\the\tableno}&&\multispan{17}\hfil {Table
\secsym\the\tableno: Estimates of $<\phi^6>_{Ws}$ from Raw Data (Corrected), Middle (50\%) Contour}\hfil&\cr
\tableedge\tablerule\tablegap\tablerule\tablelines
&&#1&&#2&&#3&&#4&&#5&&#6&&#7&&#8&&#9&\cr}
\def\tablerule{\noalign{\hrule}}
\def\tablelines{\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt&\omit&height2pt\cr}
\def\tableedge{\omit&height2pt&\multispan{17}&\cr}
\def\tablegap{\omit&\omit\vbox to 3pt{}&\multispan{17}\cr}
\halign to\hsbox{\strut#& \vrule#\tabskip=0em plus 2em& \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule# & \hfil#\hfil & \vrule# & \hfil#\hfil &
\vrule#\tabskip=0pt\cr\tablerule\tableedge
\tabletitles{$\beta\ddots L_x$}{\it 18}{\it 24}{\it 30}{\it
36}{\it 42}{\it 48}{\it 54}{\it Slope}
\tablelines\tablerule\tablelines
&&{\it 8.25}&&$3530$&&$6330$&&$23500$&&$18500$&&$18500$&&$14500$&&$15200$&&${}_{ 1.46\pm 0.22}$&\cr
&& &&${}^{+490}_{-400}$&&${}^{+1080}_{-990}$&&${}^{+3500}_{-2800}$&&${}^{+1600}_{-1500}$&&${}^{+3400}_{-2600}$&&${}^{+2800}_{-2300}$&&${}^{+3400}_{-2900}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.35}&&$712$&&$1700$&&$2860$&&$5180$&&$4790$&&$10200$&&$2640$&&${}_{ 2.38\pm 0.29}$&\cr
&& &&${}^{+75}_{-55}$&&${}^{+210}_{-190}$&&${}^{+440}_{-390}$&&${}^{+670}_{-580}$&&${}^{+1050}_{-840}$&&${}^{+2100}_{-1700}$&&${}^{+2300}_{-1680}$&& &\cr
\tablelines\tablerule\tablelines
&&{\it 8.50}&&$259^{+29}_{-23}$&&$350^{+85}_{-73}$&&$1090^{+160}_{-150}$&&$1710^{+350}_{-280}$&&$912^{+316}_{-250}$&&$1580^{+430}_{-360}$&&$1020^{+670}_{-510}$&&${}_{ 1.84\pm 0.22}$&\cr
\tablelines\tablerule\tablelines
&&{\it 8.75}&&$82.5^{+9.9}_{-8.6}$&&$142^{+40}_{-35}$&&$102^{+30}_{-24}$&&$61.5^{+46.0}_{-43.4}$&&$244^{+116}_{-102}$&&$17.3^{+101.8}_{-78.0}$&&$-634^{+111}_{-91}$&&${}_{?\pm?}$&\cr
\tablelines\tablerule\tablelines
&&{\it 9.00}&&$24.7^{+3.6}_{-3.1}$&&$34.4^{+9.1}_{-9.5}$&&$27.3^{+15.8}_{-13.9}$&&$-35.7^{+19.5}_{-16.2}$&&$-65.2^{+34.2}_{-28.0}$&&$-214^{+47}_{-39}$&&$-139^{+61}_{-47}$&&${}_{ 0.49\pm 0.11}$&\cr
\tablelines\tablerule\tablelines
&&{\it Slope}&&${}_{-1.98\pm 0.11}$&&${}_{-2.10\pm 0.15}$&&${}_{-2.58\pm 0.25}$&&${}_{-1.94\pm 0.60}$&&${}_{-2.09\pm 0.12}$&&${}_{-2.79\pm 0.80}$&&${}_{-1.87\pm 0.07}$&&&\cr
\tablelines\tablerule}}\global\advance\tableno by1}\smallskip

\ifigp\IIIFxvc{Graphs of even moments against transverse size,
$L_x$, for $\beta=8.5$. Data are shown for corrected raw
 Polyakov configurations.}
{\epsfxsize\hsize \epsfbox{w2.ps}}

It can be seen by comparison with tables 4.6-8 that revision of
estimates beyond the original errors generally occurs only for low
$\beta$ and $L_x$. However, this can have an appreciable effect on the
calculated power-law dependence of moments on $L_x$ and
$(\beta-\beta_c)$. For comparison, figures corresponding to \IIIFxv,
\IIIFxvi, \IIIFxvii\ and \IIIFxviii\ conclude this chapter, showing
the effects of removing data spikes.

\ifig\IIIFxvic{Log plots corresponding to the Wick-subtracted data of
\IIIFxvc, with best fits to a power-law dependence on the lattice
width. The previous fits from \IIIFxvc\ are given for ease of
comparison.}
{\epsfxsize\hsize \epsfbox{w2l.ps}}

\ifigp\IIIFxviic{Graphs of even moments against $\beta$,
for $L_x=36$. Data are shown for corrected raw
 Polyakov configurations.}
{\epsfxsize\hsize \epsfbox{l2.ps}}

\ifig\IIIFxviiic{Log plots corresponding to the Wick-subtracted data of
\IIIFxviic, with best fits to a power-law dependence on the lattice
width. The previous fits from \IIIFxviic\ are given for ease of
comparison.}
{\epsfxsize\hsize \epsfbox{l2l.ps}}

For the data shown in the graphs of this chapter ($L_x=36$, middle
contour, raw data), the fitted slopes for the revised
second, fourth and sixth moments are:
$$<\phi^2>\sim(\beta-\beta_c)^{-0.42(3)},\quad
<\phi^4>_{Ws}\sim(\beta-\beta_c)^{-1.25(11)},\quad
<\phi^6>_{Ws}\sim(\beta-\beta_c)^{-1.94(60)}.$$
Referring back to our formulae for the moments, we see that the
first two imply the following for our unknown functions of $\beta$:
$$\gamma\sim (\beta-\beta_c)^{0.42(3)},\qquad \lambda\sim
(\beta-\beta_c)^{0.43(16)}.$$ 
These two together predict, from our previous formulae, that 
$$<\phi^6>_{Ws}\sim(\beta-\beta_c)^{-2.08(24)},$$ extremely close
to the observed behaviour. The other sets of revised data now give
very consistent results for $\gamma$ and $\lambda$.

\vfill\supereject

